Optimal Target Shape for LiDAR Pose Estimation

Targets are essential in problems such as object tracking in cluttered or textureless environments, camera (and multi-sensor) calibration tasks, and simultaneous localization and mapping (SLAM). Target shapes for these tasks typically are symmetric (square, rectangular, or circular) and work well for structured, dense sensor data such as pixel arrays (i.e., image). However, symmetric shapes lead to pose ambiguity when using sparse sensor data such as LiDAR point clouds and suffer from the quantization uncertainty of the LiDAR. This paper introduces the concept of optimizing target shape to remove pose ambiguity for LiDAR point clouds. A target is designed to induce large gradients at edge points under rotation and translation relative to the LiDAR to ameliorate the quantization uncertainty associated with point cloud sparseness. Moreover, given a target shape, we present a means that leverages the target's geometry to estimate the target's vertices while globally estimating the pose. Both the simulation and the experimental results (verified by a motion capture system) confirm that by using the optimal shape and the global solver, we achieve centimeter error in translation and a few degrees in rotation even when a partially illuminated target is placed 30 meters away. All the implementations and datasets are available at https://github.com/UMich-BipedLab/optimal_shape_global_pose_estimation.

==> Automatic-Calibration-System.tex <==
\section{Automatic Calibration System}
\label{sec:AutomaticExtrinsicCalibrationSystem}
% The best shape determined in Sec.~\ref{sec:ShapeSensitivity} are used as targets for
% both intrinsic calibration and extrinsic calibration. Target-based \lc extrinsic
% calibration methods often suffer from manual target extraction and feature
% association. In our previous work \cite{huang2019improvements}, we assumed points on
% a \lidar target were isolated from a full scan of point cloud, and corresponding
% camera corners had been given by manually clicking on an image, and concentrated on
% accurately estimating the vertices of a \lidar target and extrinsic calibration. The
% only manual process in the previous software release \cite{huang2019improvements},
% determining the image corners, was made automatic in
% \bh{cite:AutomaticCalibration}. Because comparing and validating the intrinsic
% calibration methods of Sec.~\ref{sec:ProposedIntrinsicModel}
% and~\ref{sec:BaselineIntrinsicCalibrationModels} would require significant data
% collection, we decided to create a fully automatic pipeline for both intrinsic and
% extrinsic calibration as shown in Fig~\ref{fig:AutomaticPipeline}. We demonstrate
% the capability of this pipeline by collecting a significant amount of data allowing
% us to check the quality of the calibration of our sensor suite (a \lc pair) at
% different distances; see~\bh{sec:ExtrinsicCalibration}.

The optimal shape determined in Sec.~\ref{sec:ShapeSensitivity} are used as targets
for both intrinsic calibration and extrinsic calibration. Target-based \lc extrinsic
calibration methods often suffer from manual target extraction and feature
association. Because comparing and validating the intrinsic calibration methods of
Sec.~\ref{sec:ProposedIntrinsicModel}
and~\ref{sec:BaselineIntrinsicCalibrationModels} would require significant data
collection, we decided to create a fully automatic pipeline for both intrinsic and
extrinsic calibration as shown in Fig~\ref{fig:AutomaticPipeline}. We demonstrate the
capability of this pipeline by collecting a significant amount of data allowing us to
check the quality of the calibration of our sensor suite (a \lc pair) at different
distances; see~\bh{sec:ExpExtrinsicCalibration}.


\begin{figure*}[t]
    \centering
    \includegraphics[width=1.9\columnwidth]{automatic-calibration-system/AutomaticPipeline.png}
    \caption{\bh{took from previous paper}A system diagram for
        automatic intrinsic and extrinsic calibration. The top shows the front-end of
        the pipeline. Its input is raw camera and \lidar data, which are subsequently
        synchronized. The \atag and \lidart packages are used to extract the target
        information, which is then examined to remove outliers and ensure that
        targets are still properly synchronized. Each run of the front-end saves all
        related information into a ROS bagfile, which can then be sent to the
        back-end for further processing. The back-end takes in (possibly many) ROS
        bagfiles and does the following: (i) refines the image corners; and (ii)
        extracts vertices of the \lidar targets. The correspondences are established
        between corners and vertices and an extrinsic transformation is determined
        PnP as in \cite{lepetit2009epnp}. For intrinsic calibration, the resulting vertices of
        the \lidar targets are used to extract normal vectors and a point on the
        plane. The calibration parameters are determined to minimize the P2P distance
        from the plane to the target points provided by the \lidart package.}
\label{fig:AutomaticPipeline}
\end{figure*}

\subsection{Front-End: Data Pre-processing}
\label{sec:FrontEnd}
Fiducial markers, such \atags\cite{olson2011apriltag, wang2016apriltag,
krogiusflexible}, are widely used in vision-based perception tasks because they can
be easily identified and automatically extracted from background.
In \cite{huang2019lidartag}, we introduced a similar concept for \lidar point clouds,
called a \lidartN. Inspired by \atagsN, they consist of a payload and a pattern that
makes each marker uniquely distinguishable and identifiable in real-time by both a
\lidar and a camera. An open-source package for processing \lidarts is available
\cite{githubFileLiDARTag} while both \atagN2 and \atagN3 are available as a Robot
Operating System (ROS) package \cite{githubFileAprilTagROS}.


\begin{remark}
    A payload is roughly\footnote{No measurement required for placing payloads}
    placed at the center of the optimal target, as shown in
    Fig.~\bh{fig:CalibrationTargets}. Another step will be performed to refine
    corners; see Sec.~\ref{sec:ImageCorners}.
\end{remark}

% As the \lidar and camera data streams arrive, they are synchronized, examined for
% fiducial markers, and checked for false positives.

Each step in the front-end of the Fig.~\ref{fig:AutomaticPipeline} is a node in ROS
\cite{quigley2009ros}. As the \lidar and camera data streams arrive at the
frame-synchronization node, they are synchronized by the approximate time policy.
Each synchronized frame is assigned a frame id, which is defined by the order of
arriving and published at the same frequency. The \lidart and \atag node will process
the synchronized data and publish arrays of detected fiducial markers separately. To
ensure the two streams remain synchronized, regardless if a fiducial marker is
detected, a message is published (i.e., an empty message will be published if no tag
is detected). 

% Also, the detection
% messages are labeled with a frame index from the synced
% image.

In the tag-paring node, types of messages\footnote{Each message of each type is
labeled with a frame id.} (\lidartsN, \atagsN, images) arrive at different frame
rates again at the tag-paring node due to different working frequency of each node.
However, the same synchronization policy cannot be used because working frequency for
each node is fluctuated. \bh{perhaps not clear enough?} A queue is created for each
type of messages to store its own messages. To further prevent from unexpected
dropping packets between communications in the pipeline, we create a master clock to
group the same frame id as shown in Fig.~\bh{fig:udpDropping}. \bh{say more maybe}

False positives and false negatives are examined after messages (\lidartsN, \atagsN,
images) with the same frame id are grouped together. For each grouped message, if the
number of the detected markers in the \lidart and the \atag message is not the same,
or if the detected ids in the \lidart and the \atag message are not the same, this
grouped message will be abandoned. Empty messages will also be dropped at this node.
The synchronized, examined data (images, \atag corners, points on \ltagsN) are saved
as ROS bagfiles for post-processing in MATLAB. 


\subsubsection{Extrinsic Calibration} 
For \lc extrinsic calibration, corresponding features from camera data and \lidar
data must be identified. We use target vertices as our correspondences in this
pipeline. The target's \lidar returns (\lidart points) are extracted from a full scan
of \lidar point cloud in the front end by the \lidart package. In the image plane,
the target vertices are typically called corners and are extracted in the front end
using the \atag ROS package. 


\subsubsection{Intrinsic Calibration} 
For a \slidar intrinsic calibration, points on a target are spitted based on rings and
points on the same ring but on different targets are gathered as a collection of
points to compute P2P cost \eqref{eq:OptSolution}. A target's normal vector and a
point on the target are computed by the estimated target vertices; see
Sec.~\ref{sec:TargetVertices}. 



\subsection{Back-End: \lidar Target Vertices Determination}
\label{sec:TargetVertices}
At this stage, extracted features (\atags corners and \lidart points) have been
properly synchronized and examined automatically for false positives. The next step
is to estimate the \lidart vertices, which, due to sparsity of the \lidar point
cloud, are not directly observable. We use the method developed in
\cite{huang2019lidartag} to determine the vertices. However, instead of a
diamond-shaped target stated in our previous paper \cite{huang2019lidartag}, we
change the shape to the optimal shape determined in Sec.~\ref{sec:ShapeSensitivity}.
From the vertices, the target normal $\N[t]$ and point on the target, $p_{0,t}$, can
be easily determined for evaluating the P2P cost function \eqref{eq:OptSolution} for
intrinsic calibration, while the vertices in combination with the camera corners are
used to determine the extrinsic calibration via a PnP problem or a IoU problem; see
Sec.~\bh{sec:ExtrisicProblem}.


The following is partially taken from \cite{huang2019improvements} and provided for
clarity. Let $\pc := \{\cal X_i\}_{i=1}^{M}$ be a collection of 3D points on a \lidar
target, where $M$ is the number of points. Given the target geometry (here is the
optimal shape determined in Sec.~\ref{sec:ShapeSensitivity}), we define an
ideal target with vertices $\{ \bar{X}_i \}_{i=1}^4$ located at the origin of the
\lidar as defined in Fig.~\bh{fig:IdealFrame}. We seek a rigid body transformation
from \lidar to the target, $H_L^T$, that ``best fits'' the ideal target onto the point
cloud.

\bh{Need to modify for the new shape}
In practice, it is actually easier to pull the $\pc$ back to the origin of the \lidar
through the inverse of the current estimate of transformation $H_T^L:=(H_L^T)^{-1}$
and measure the error there. For $a \ge 0$ and $\lambda \in \real$, an $L_1$-inspired
cost is defined as

\begin{equation}
    \label{eq:L1cost}
    c(\lambda,a):=\begin{cases}
    \min\{ |\lambda-a|, |\lambda + a| \} & \text{if}~|\lambda| >a \\
    0 & \text{otherwise}
    \end{cases}.
\end{equation}
Let $\{\tilde{\chi}_i\}_{i=1}^N:=H_T^L(\mathcal{PC}):=\{ H_T^L(\chi_i) \}_{i=1}^N$ denote
the pullback of the point cloud by $H_T^L$, and denote a point's $(x,y,z)$-entries by
$(\tilde{x}_i,\tilde{y}_i,\tilde{z}_i)$.
The total fitting error of the point cloud is defined as
\begin{equation}
	\label{eq:JKHcost}
    C(H_T^L(\pc)) :=\sum_{i=1}^{M} c(\tilde{x}_i,\epsilon) +
    c(\tilde{y}_i,d/2) +  c(\tilde{z}_i,d/2),
\end{equation}
where $\epsilon \ge 0$ is a tuning parameter to account for uncertainty in the depth
measurement of the planar target. For more detail about this method and target
placement for extrinsic calibration, see~\cite{huang2019improvements}.



\subsection{Back-End: Camera Corners Detection, Refinement and Correspondences Association}
\label{sec:ImageCorners}
The \atag package detects inner (black) corners of an \atagN, while correspondences
for extrinsic calibration are target vertices as shown in
Fig.~\bh{fig:CalibrationTargets}. Given the dimension of an \atagN, simple linear
interpolation is used to estimate the vertices in the \atag frame. The target
corners in the image coordinates are computed by projecting the vertices with a
homograph matrix.

The corners obtained from the \atag package are automatically refined as shown in
Fig.~\bh{refineImageCorners} using an process detailed in \cite{huang2019improvements}.
Given the camera corners ($\{ Y_i\}_{i=1}^4$) and \lidar vertices $\{ X_i\}_{i=1}^4$,
we use the vertical and horizontal positions in their own coordinates to sort them
and establish the correspondences.

\subsection{Optimizations}

\subsubsection{Extrinsic Calibration}
Once ``enough'' independent target vertices are estimated from both camera data and
\lidar point cloud, the optimization for the extrinsic transformation can be
formulated in a standard Perspective-n-Point (PnP) problem \cite{lepetit2009epnp}:
minimize Euclidean distance of the corresponding corners. In
\cite{huang2019improvements}, we also proposed maximizing the intersection over union
(IoU) of the corresponding projected polygons. More detail for both methods is provided in
\cite{huang2019improvements}.


Let $X_i$ be the (homogeneous) coordinates of the LiDAR features, $Y_i$ be the
coordinates of the camera features. We denote by $\Pi$ the often-called ``projection map''
\cite[(8)]{huang2019improvements} and let $H_{L}^{C}$ be the (homogeneous representation of)
the LiDAR-frame to camera-frame transformation with rotation matrix $R_{C}^{L}$ and
translation $T_{C}^{L}$.


\textbf{i) PnP Formulation} Given $n$ targets (i.e., $4n$ features), the PnP problem
is

\begin{equation}
    \label{eq:PnP}
        \left({R_L^C}^*, {T_L^C}^*\right) :=  \argmin_{R,
    T}\sum_{i=1}^{4n}\norm{\Pi\left(X_i; R, T\right)-\pre[C]Y_i}_2^2.
%\label{eq:ConceptualProblem}
%(R_{C}^{L*}, T_{C}^{L*})= \mathrm{arg} \min_{(R,T)}{\sum_i
%                    \mathrm{dist}(\Pi(H_{L}^{C}(X_i)),Y_i)},
\end{equation}

\textbf{ii) IoU Formulation} 
Let $\pre[L]\vx:=\{\pre[L]Y_i\}_{i=1}^{4n}$ be the vertices of the estimated target
polygons projected from the \lidar frame to the camera frame as in
\cite[(8)]{huang2019improvements}, and let $\pre[C]\vx:=\{\pre[C]Y_i\}_{i=1}^{4n}$ be
the vertices of the corresponding camera images of the targets. The corresponding
areas of the polygons are $\A(\pre[L]\vx), \A(\pre[C]\vx)$ and let $\A(\pre[I]\vx)$
denote the intersection of the two polygons. The IoU of the two polygons is then

\begin{equation}
    \label{eq:IoUCost}
    IoU(\pre[L]\vx,\pre[C]\vx,\pre[I]\vx) = \frac{\A(\pre[I]\vx)}{\A(\pre[L]\vx) +
    \A(\pre[C]\vx) - \A(\pre[I]\vx)}. 
\end{equation}

The resulting optimization problem is
\begin{align}
\label{eq:IoUOptimization}
    \left({R_L^C}^*, {T_L^C}^*\right) &:= \argmax_{R,T}IoU(\pre[L]\vx,\pre[C]\vx)\\
                                       &= \argmax_{R,T}IoU(\Pi\left(\{X_i\}_{i=1}^{4n}; R, T\right),\pre[C]\vx), \nonumber
\end{align}
where the projection map in \cite[(8)]{huang2019improvements} has been used to make
the dependence on the rigid-body transformation explicit. 


\subsubsection{Intrinsic Calibration}
With the method in Sec.~\ref{sec:TargetVertices} and \cite{huang2019lidartag}, the
target vertices are automatically co-planar and hence uniquely define a unit normal
vector and a point on the target. The target vertices are
used to compute a normal vector and a point on the target. The P2P distance is
minimized for each of the three calibration models, $\BL_1$, $\BL_2$, and $\Sim(3)$,
for a collection of targets, yielding $\alpha^*$ (for $\BL_1$ and $\BL_2$) and
$\Sigma^*$ for $\Sim(3)$.

The processes of intrinsic calibration involves iterating the estimation of the
target vertices and the parameters in the \lidar model until a given stopping
criterion is met\footnote{In simulation, no iteration is required as the target
information is known from ``ground truth''. }. Here, stopped when the maximum change
in a target vertex was less than $1e-5$.

\begin{algorithmic}
    \While{$\delta_m>10^{-5}$}
    \State \textbf{Step 1:} Re-estimate the target vertices $\{ X_i\}_{i=1}^4$ after
    applying the current intrinsic calibration parameters to the point cloud. This
    gives updated values for the target normals and points on the targets.

    \State \noindent \textbf{Step 2:} Using the updated target vertices, re-estimate
    the intrinsic calibration parameters for the three calibration models. \EndWhile
\end{algorithmic}


==> Baseline-LiDAR-Intrinsic-Model.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Baseline Intrinsic Calibration Models}
\label{sec:BaselineIntrinsicCalibrationModels}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
There are two standard calibration models for \slidarsN. They are inspired by
postulating \slidarsN' working mechanisms, which is based on spherical coordinates.
These types of calibration models is not applicable to other types of sensors that do
not function the same means as the models are designed. As shown in
Fig.~\bh{fig:spherical-coordinate}, the spherical coordinates $(\rho, \theta, \phi)$
refers to as range, elevation and azimuth,

\begin{equation}
	\label{eq:spherical2Cartesian}
	\begin{bmatrix}
		x\\y\\z
	\end{bmatrix} = f(\rho, \theta, \phi)
	=\begin{bmatrix}
		\rho\cos\theta\sin\phi\\
		\rho\cos\theta\cos\phi\\
		\rho\sin\theta
	\end{bmatrix},
\end{equation}
and the inverse function, 
\begin{equation}
	\label{eq:Cartesian2spherical2}
	\begin{bmatrix}
		\rho\\\theta\\\phi
	\end{bmatrix} 
	= f^{-1}(x,y,z) 
	=\begin{bmatrix}
		\sqrt{x^2+y^2+z^2}\\
		\asin[\frac{z}{\sqrt{x^2+y^2+z^2}}]\\
		{\rm atan2}(x,y)
	\end{bmatrix}.
\end{equation}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{3-Parameter Model}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The most basic model~\cite{pandey2010extrinsic} are shown in
Fig.~\bh{fig:basic-model}, and is denoted as $\BL_1$. The basic model assumes the
\lidar measurements are made in spherical coordinates, $(\rho, \theta,\phi)$.
Corrections to a measurement are given by a collection additive offsets
\mbox{$\alpha:=(\delta_\rho, \delta_\theta, \delta_\phi).$} Expressing the calibrated
measurement in Cartesian coordinates gives

\begin{equation}
\label{eq:SimpleCalibration}
        \Gamma_{\alpha}(\rho, \theta, \phi) := 
        \begin{bmatrix}
    (\rho+\drho)\cos(\dtheta)\sin(\phi-\dphi)\\
    (\rho+\drho)\cos(\dtheta)\cos(\phi-\dphi) \\
    (\rho+\drho)\sin(\dtheta)
        \end{bmatrix}
\end{equation}

\begin{remark} 
    \textbf{(a)} The nominal elevation for each ring is taken as zero;, i.e.,
    $\theta=0.$  \textbf{(b)} While it is not necessarily a drawback, most \lidar
    interfaces only return a Cartesian representation of a measured point. Hence, the
    user must assure the transformation to spherical coordinates, make the
    measurement correction coming from the calibration, and then transform back to
    Cartesian coordinates. 
\end{remark}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{6-Parameter Model}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \cite{pandey2010extrinsic, muhammad2010calibration, glennie2010static}
Fig.~\bh{fig:complex-model} shows a more complex model \cite{glennie2010static,
nouira2016point} for a \slidarN, and is denoted as $\BL_2$. This model also works in
spherical coordinates. In addition to the three offsets above, it includes $s$, a
scale factor of $\rho$, $h$, a horizontal offset of the origin, and $v$, a vertical
offset for the origin. The correction model becomes

\begin{equation}
\label{eq:ComplexCalibration}
         \bar{\Gamma}_{\alpha}:= 
\left[
\begin{array}{l}
    (s\rho+\delta_\rho)\cos\delta_\theta\sin(\phi-\delta_\phi) - h\cos(\phi-\delta_\phi)\\
    (s\rho+\delta_\rho)\cos\delta_\theta\cos(\phi-\delta_\phi) + h\sin(\phi-\delta_\phi)\\
    (s\rho+\delta_\rho)\sin\delta_\theta + v\\
\end{array}\right].
\end{equation}
and $\alpha:=(\delta_\rho, \delta_\theta,
\delta_\phi, s, h, v).$ 




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Can these be expressed as transformations by similar matrices?}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The short answer is no. This section decomposites the 6-parameter model
\eqref{eq:ComplexCalibration} viewed in Cartesian coordinates into cascaded
transformations. The  model is fundamentally nonlinear and can be expressed as
$\R[1](\R[2]\t[1] + \t[2])$,
% \begin{equation}
%     \label{eq:ComplexModelMatrixForm}
%     \calx_c = \R[1](\R[2]\t[1] + \t[2]),
% \end{equation}
where $\R[1], \R[2], \t[1] \text{ and } \t[2]$ depend on the measured point, 
$$\x[][\transpose] = [x,y,z] \xrightarrow[]{f^{-1}} (\rho, \theta, \phi),$$

\begin{align}
    \label{eq:ExpandComplexModelMatrixForm}
    \R[1]&=
             \begin{bmatrix}
                 \sin(\phi-\dphi) & -\cos(\phi-\dphi) & 0\\
                 \cos(\phi-\dphi) &  \sin(\phi-\dphi) & 0\\
                 0 &0 &1
             \end{bmatrix},\\ \nonumber
    \R[2]\t[1]+\t[2] &=
             \begin{bmatrix}
                 \cos(\dtheta) & 0 & -\sin(\dtheta)\\
                 0 &1 &0\\
                 \sin(\dtheta) & 0 & \cos(\dtheta)
             \end{bmatrix}
             \begin{bmatrix}
                 s\rho+\drho\\
                 0
                 \\0
             \end{bmatrix} +
             \begin{bmatrix}
                 0\\h\\
                 v
             \end{bmatrix}.
\end{align}

The 6-parameter model first applies a corrected elevation angle ($\R[2]$) to a range
value that has been offset and scaled ($\t[1]$). Next, the $(y,z)$ position of the
origin is offset ($\t[2]$), and lastly, a corrected rotation about the $z$-axis is
applied ($\R[1]$). Because the resulting cascading transformation cannot be written as a single
$\Sim(3)$ transformation, therefore, the proposed model is not the same as either the
3-parameter model or the 6-parameter model.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Cost function for baseline models}
\label{sec:BaselineCostFunctions}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
For a given collection of points $\pc_t = \{\x[i]\}_{i=1}^{M_t}$, possibly from
multiple targets $t\in\{1, \ldots, T\}$, we seek a set of calibration parameters
$\alpha$ that solve

% \begin{equation}
% \label{eq:OptSolutionBaseline}
%     \min_{\alpha}
%   \sum_{t=1}^T\sum_{i=1}^{M_t}
%     | \n[t][\transpose] \left(F({\cal X}_i, \alpha) - p_{0,t}\right) |,
% \end{equation}
\begin{equation}
\label{eq:OptSolutionBaseline}
    \min_{\alpha}
   \sum_{t=1}^T\sum_{i=1}^{M_t}
    | \n[t][\transpose] \left(F(\x[i], \alpha) - \p[0,t] \right) |,
\end{equation}
where
\begin{enumerate}
       \item for baseline model $\BL_1$~\cite{pandey2010extrinsic} in
           \eqref{eq:SimpleCalibration}, $\alpha =(\drho, \dtheta, \dphi)$ and
           $$F({\x}, \alpha):= \Gamma_{\alpha} \circ f^{-1}({\x});$$

      \item for baseline model $\BL_2$~\cite{glennie2010static, nouira2016point} in
          \eqref{eq:ComplexCalibration}, $\alpha =(\drho, \dtheta, \dphi, s, h, v)$
          and 
          $$F({\x}, \alpha):= \bar{\Gamma}_{\alpha} \circ f^{-1}({\x})$$
\end{enumerate}

\begin{remark}
    \bh{Do we need to include this? I am not sure how to say about $\BL_2$}
   For the 3-parameter model $\BL_1$, a single planar target is sufficient to
   uniquely determine a set of parameters $\alpha =(\drho, \dtheta, \dphi)$. For the
   6-parameter model $\BL_2$, non-uniqueness can occur as outlined in
   Proposition~\ref{thm:HopefullyTrue} and Fig.~\ref{fig:PropositionIllustration}.
\end{remark}


==> Extrinsic-Calibration.tex <==
\section{Extrinsic LiDAR-Camera Calibration}
\label{sec:ExtrinsicCalibration}
\bhw{}
In our previous work \cite{huang2019improvements}, we assumed each target is planar,
square, and has to be rotated in the frame of the LiDAR by roughly 45$^\circ$ to form
a diamond as. We also noted that placing the targets so that the rings of the LiDAR
run parallel to its edges leads to ambiguity in the vertical position due to the
spacing of the rings, as indicated in \cite{liao2018extrinsic, zhou2018automatic}.
However, by using the optimal shape in Sec.~\ref{sec:ShapeSensitivity}, we only need
to put the shape as it is, no further requirement above is needed. In this section,
we assume that standard methods have been used to automatically isolate the target's
point cloud \cite{huang2019lidartag}; see Sec.~\ref{sec:FrontEnd} and
Fig.~\ref{fig:AutomaticPipeline}.


points on a \lidar target were isolated from
a full scan of point cloud, and corresponding camera corners had been given by
manually clicking on an image, and concentrated on accurately estimating the vertices
of a \lidar target and extrinsic calibration. The only manual process in the previous
software release \cite{huang2019improvements}, determining the image corners, was
made automatic in \bh{cite:AutomaticCalibration}. 


==> Extrinsic-Refinement.tex <==
\section{Extrinsic Calibration and Refinement}
\label{sec:ExtrinsicCalibration}


==> Image-Projection.tex <==
\section{Image Corners and Correspondences with the \lidar Vertices}
\label{sec:ImageCorners}


==> Proposed-LiDAR-Intrinsic-Model.tex <==
% \section{3D \lidar Intrinsic Calibration}
% \label{sec:Intrinsic3DLiDARCalibration}
% something...

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Proposed \lidar Intrinsic Calibration Model}
\label{sec:ProposedIntrinsicModel}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The proposed calibration parameters are modeled as an element of the similarity Lie
group $\Sim(3).$ An element of the group is isometry composed with an additional
isotropic scaling, i.e., a rigid-body transformation with scaling. We note that this
is the most general form of transformation in 3D space while preserving the shape
(i.e. preserving ratio of lengths, and angles); and therefore, it is suitable for
intrinsic calibration of \lidarsN. The proposed calibration model works for both
\slidars and \sslidarsN. An element of the group is given by

\begin{equation}
\label{eq:sim3tf}
        \H = \begin{bmatrix}
         s \R & \t \\
         \zeros & 1
     \end{bmatrix} \in \Sim(3),
\end{equation}
where $\R \in \SO(3)$ is the 3D rotation matrix, $\t \in \mathbb{R}^3$ is the
translation vector, and $s \in \mathbb{R}^+$ is the scale parameter. In particular,
an element has seven degrees of freedom and the action of $\Sim(3)$ on $\mathbb{R}^3$
is $\H \cdot \x = s\R \x + \t$, where $\x \in \reals^3$. 


Let $\n[t]$ be a unit normal vector of a planar target and let $\p[0, t]$ be a fixed
point on the target. Let $\pc = \{ \x[i] | i=1,\dots,M~\text{and}~\x[i] \in
\mathbb{R}^3 \}$ denote a collection of \lidar returns on the target, and $M$ is the
number of points in the collection. Wherever convenient, we abuse notation by passing
to from regular coordinates to or homogeneous coordinates without noting the
distinction. Given the collection of \lidar returns $\pc$, the cost is defined by the
point-to-plane (P2P) distance: 

\begin{equation}
   J := \sum_{i=1}^M
   \lvert \n[t][\transpose] \left(\x[i] - \p[0,t] \right) \rvert,
\end{equation}
where $\n[t][\transpose] \left(\x[i] - \p[0,t] \right)$ is the orthogonal projection
of the measurement onto the normal vector and $\lvert\,\cdot\,\rvert$ is the absolute
value. Then the calibration problem can be formulated as follows

\begin{problem}
\label{prob:intrinsic_calibration}
For a given collection of points $\pc_t = \{\x[i]\}_{i=1}^{M_t}$, possibly
from multiple targets $t\in\{1, \ldots, T\}$, we seek a similarity transformation
$\H[][\star]$ that solves

\begin{equation}
\label{eq:OptSolution}
    \min_{\H \in \Sim(3)}
   \sum_{t=1}^T\sum_{i=1}^{M_t}
    \lvert \n[t][\transpose] \left( \H \cdot \x[i] - \p[0,t] \right) \rvert.
\end{equation}
\end{problem}

\begin{remark}
In practice each target's normal vector and a point on the target must be estimated
from data; see Sec.~\bh{sec:L1-optimization}. 
\end{remark}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \textbf{Parsing a target's point cloud to collections of points:}
\subsection{Parsing points on a target to collections of points}
\label{sec:CollectionOfPoints}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The specific method for parsing a target’s point cloud and the number of calibration
transformations depends on the nature of the sensor. For a \slidarN, the points $\pc$
on a target are typically separated by beam number so each beam has its own
optimization problem~\eqref{eq:OptSolution}. For example, for a $K$-beam \slidar,
the set of calibration parameters is $\{\H[k] | k=1,\dots,K~\text{and}~\H[k] \in
\Sim(3)\}$. 

For an OPA-based \sslidarN, we form an $m\times n$ grid over the planar target and
then parse the point cloud based on each point's projection onto the target along the
normal of each grid. This way, the set of calibration parameters becomes 
$\{\H[k] | k=1,\dots,m\times n~\text{and}~\H[k] \in \Sim(3)\}$.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Guideline for Target Placement for a Spinning \lidarN}
\subsection{Over parameterization analysis for a Spinning \lidarN}
\label{sec:TargetPlacementGuideline}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The proposed calibration model is over parameterized (i.e., the unique $\H[][*]$ does
not exist) when less than four targets are used to calibrate a \slidarN. In
particular, for a single planar target, the rotation about the target normal $\n[t]$,
two components of the translation vector $\t$ (translation in the plane of the
target) and the scale $s$ are unconstrained as shown in Fig.~\bh{fig:one-target}. For
two planar targets, the translation along the line orthogonal to the targets' normal
vectors and the scale are unconstrained as shown in Fig.~\bh{fig:two-targets}. 

% In our previous work \bh{cite:sec. II, AutomaticCalibration}, we provide a
% degenerated case:
% 
% \begin{proposition}
%     \label{thm:HopefullyTrue} 
%     Consider three targets with normals $\n[i]$, points
%     on target $\p[0,i]$, and point clouds $\pc_i$. Denote the orthogonal complement
%     of $\n[i]$ by $\n[i][\perp]$.  Assume the set of normal vectors, $\{\n[1],
%     \n[2], \n[3] \}$, is linearly independent.
%     \begin{enumerate}
%         \item[a)] The plane defined by the $i$-th target is $\mathcal{V}_i:= \p[0,i] + \n[i][\perp]$ and there exists a unique point $\q[0] \in \mathbb{R}^3$ defined by
%         \begin{equation}
%         \label{eq:PoleOfCalibration}
%             \q[0] :=\bigcap\limits_{i=1}^3 \mathcal{V}_i.
%         \end{equation}
%         % \item[b)] If at least one of the point clouds does not fall exactly on a line, then a minimizer of Problem~\ref{prob:intrinsic_calibration} is unique.
%         \item[b)] For $\H \in \SE(3)$ there exists a unique solution.
%         \item[c)] For $\H \in \Sim(3)$ the scale $s$ is unconstrained.
%         \item[d)] Suppose $\mathcal{L}_i$ is a line formed by a beam on the $i$-th target. If all of the lines $\mathcal{L}_i$, $1 \le i \le 3,$  pass through the point $\q[0]$, then the solution is not unique.
%     \end{enumerate}
% \end{proposition}
% If the condition in  parts (d) holds, then the scale factor, $s$, is not unique; see Fig.~\ref{fig:PropositionIllustration}.

For $\Scal\in\reals^3$, let $[\Scal] \text{ and } [\Scal]^\perp$ denote its span and
its orthogonal complement. Let $\{\e[1], \e[2], \e[3]\}$ be the canonical basis for
$\reals^3$. We also denote $\P\subset\reals^3$ a set traced out by a single ring of
a perfectly calibrated \slidarN. Without loss of generality, we assume
$\P=[\e[3]]^\perp$. 

Consider four targets with unit normal vectors $\n[i]$ and let $\p[0,i]$ be a point
on the $i$-th target. For $1\le i \le 4$, the plane defined by the $i$-th target is
$\V[i]:= \p[0,i] + [\n[i]]^\perp$. If the following two assumptions are satisfied,
Theorem~\ref{thm:uniqueness} states that there exists the unique answer to
Problem~\ref{prob:intrinsic_calibration} and is proved in
Appendix~\ref{sec:Uniqueness}.


% \subsubsection{Assumption N} All sets of three distinct vectors from $\{ \n[1],
% \n[2], \n[3], \n[4], \e[3]\}$ are linearly independent. Under this assumption, for
% each $i \neq j \in \{1, 2, 3, 4 \}$, $\p[ij]:=\P \cap \V[i] \cap \V[j]$ exists
% and is unique. 
% 
% \subsection{Assumptions}
\begin{assumption}[Assumption N]
    \label{asm:assumtionN}
    All sets of three distinct vectors from $\{ \n[1], \n[2], \n[3], \n[4], \e[3]\}$
    are \li.
\end{assumption}


\begin{assumption}[Assumption B]
    \label{asm:assumtionB}
    Given the six intersection points, any two form a set of basis for the ring
    plane. There are $\binom{6}{2}$ sets of basis. Subsets of the basis' are \li.
    \begin{enumerate}[(a)]
        \item $\{ \p[12], \p[13] \}$, $\{ \p[13], \p[14] \}$, $\{ \p[14], \p[12] \}$,
        \item $\{ \p[12], \p[23] \}$, $\{ \p[23], \p[24] \}$, $\{ \p[24], \p[12] \}$,
        \item $\{ \p[13], \p[23] \}$, $\{ \p[23], \p[34] \}$, $\{ \p[34], \p[13] \}$,
        \item $\{ \p[14], \p[24] \}$, $\{ \p[24], \p[34] \}$, $\{ \p[34], \p[14] \}$,
        \item $\{ \p[14], \p[23] \}$
    \end{enumerate}
\end{assumption}

\begin{remark}
    Assumption~\ref{asm:assumtionN} considers a set of condition numbers
    ($\binom{5}{3}=10$) for any three of 3D normal vectors.
    Assumption~\ref{asm:assumtionB} examines a set of condition numbers for
    the chosen 2D basis. If the two sets of condition numbers are well conditioned,
    there exists the unique answer to Problem~\ref{prob:intrinsic_calibration} as
    proved in Appendix~\ref{sec:Uniqueness}.
\end{remark}

\begin{theorem}
    \label{thm:uniqueness}
    Assume that Assumptions N (Assumption~\ref{eq:assumtionN}) and B
    (Assumption~\ref{eq:assumtionB}) hold and let $\H \in \Sim(3)$. If for each $i
    \neq j \in \{1, 2, 3, 4 \}$, $\H\cdot\p[ij] \in  \V[i] \cap
     \V[j]$, then
     \begin{equation}
         \H =
         \begin{bmatrix}
            \I & \zeros \\
            \zeros & 1
         \end{bmatrix}.
     \end{equation}
 \end{theorem}


The proof is given in Appendix~\ref{sec:Uniqueness}. The resulting target placement
for a \slidar is an oriented tetrahedron\footnote{Each of the four targets extends an
infinite plane. The extended infinite planes create a tetrahedron.} where the
normal vector of each face\footnote{Faces of the tetrahedron are extended planes
of targets. Therefore, normal vectors of faces are normal vectors of targets}
satisfies Assumption~\ref{asm:assumtionN} and the orientation of the
tetrahedron intersects with the ring plane fulfills
Assumptions~\ref{asm:assumtionB} as shown in Fig.~\ref{fig:oriented-tetrahedron} and
Fig.~\ref{fig:tetrahedron-Cassie}.

\begin{figure}[t]%
\centering
\subfloat[]{%
    \label{fig:oriented-tetrahedron}%
	\centering
	\includegraphics[width=1\columnwidth, trim={0.00cm 0cm 0cm 0.cm},clip]{tetrahedron-with-ring-plane.png}}
\hspace{5pt}%
\subfloat[]{%
    \label{fig:tetrahedron-Cassie}%
	\centering
    \includegraphics[width=1\columnwidth, trim={0.5cm 3.5cm 1.8cm 3.5cm},clip]{Cassie-with-targets.png}}
\caption[]{}%
% \label{fig:semantic}%
\end{figure}





==> Relaxed-Uniqueness.tex <==
\section{Proof on Uniqueness of Affine Transformation}
If we relax the problem to being an affine transformation, the problem becomes
linear and we only have to check the invertibility of a matrix. This also
allows us to calculate the conditioning number to get an instant measure on how robust
the setup is.

\begin{proposition}
 Assume that the matrix $A$ in \eqref{eq:18_matrix} has rank 15. If
 for each $i \neq j \in \{1, 2, 3, 4 \}$, $\H\cdot\p[ij] \in  \V[i] \cap \V[j]$, then

\begin{equation} 
    \H = \begin{bmatrix}
        \I & \zeros \\
        \zeros & 1
    \end{bmatrix}.
\end{equation}
\end{proposition}

\begin{proof}
    We reformulate \eqref{eq:NecssSuff}, 

\begin{equation}
\label{eq:rewrite-necssStuff}
\H\cdot\p[ij] \in  \V[i] \cap \V[j] \iff (s\R-\I) \p[ij] + \t = \alpha_{ij}(\n[i]\times \n[j]), 
\end{equation}
where the $\alpha_{ij}\in \reals$ are unknown coefficients. By relaxing to affine
transformation, rotations become arbitrary matrices. Let superscripts denote
components of vectors/matrices and let subscripts be indices. We further rewrite
\eqref{eq:rewrite-necssStuff}:

\begin{equation}
    \label{eq:linear_sys_part2}
    \M[3\times3]\p[ij] + \t = \alpha_{ij} \cdot v_{ij},
\end{equation}
where $\M[3\times3]$ is an arbitrary matrix and $v_{ij}=\n[i]\times \n[j]$. If we
write \eqref{eq:linear_sys_part2} as a summation: 
\begin{equation}
    \label{eq:linear_sys_part3}
     \sum_{\ell=1}^3 \, M^{k\ell}\cdot p_{ij}^\ell + t^k = \alpha_{ij}\cdot v_{ij}^k,
\end{equation}
this system clearly has $3n$ equations and $12+n$ unknowns where $n$ is the number of
$p_{ij}$. In our case, $n=6$ and \eqref{eq:linear_sys_part2} forms an $18$ by $15$
system. Therefore if its matrix \textcolor{green}{has maximal rank (it will always be singular as it is not square}, there exists a unique solution. The
matrix is given by
 \begin{equation}\label{eq:18_matrix}
     A = \begin{bmatrix}
     X & 0 & 0 & 1_{6\times 1} & 0 & 0 & -\Lambda_1 \\
     0 & X & 0 & 0 & 1_{6\times 1} & 0 & -\Lambda_2 \\
     0 & 0 & X & 0 & 0 & 1_{6\times 1} & -\Lambda_3
    \end{bmatrix},
 \end{equation}
 where
 \begin{equation*}
    \begin{split}
        X &= \left[ p_{12},p_{13},p_{14},p_{23},p_{24},p_{34}\right]^\intercal \\
        \Lambda_k &= \mathrm{diag}\left[ v_{12}^k, v_{13}^k, v_{14}^k, v_{23}^k, v_{24}^k, v_{34}^k \right].
    \end{split}
 \end{equation*}

The condition matrix $A$ is given in Appendix~\ref{sec:condition-matrix}.
\end{proof}

\begin{remark}
 \bh{need to be rephrased later on}
The matrix $A$ has three columns which are trivially zero. This leaves the last
column of $U$ free (so uniqueness fails). But! a (3 dimensional) rotation matrix is
uniquely determined by its first two columns (as the third is taken to be the third
ONB). Therefore, we obtain a unique rotation matrix and the result holds.
\end{remark}


% \pagebreak
\section{Condition Matrix}
\label{sec:condition-matrix}
The condition matrix in \eqref{eq:18_matrix} is an $18$ by $15$ matrix and is given by
\begin{figure*}[h]%% over both columns
\center
 \begin{equation*}
	% \resizebox{0.93\hsize}{!}{%
     A = \left(\begin{array}{ccccccccccccccc}
     p_{12}^1 & p_{12}^2 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & -v_{12}^1 & 0 & 0 & 0 & 0 & 0 \\
     p_{13}^1 & p_{13}^2 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & -v_{13}^1 & 0 & 0 & 0 & 0 \\
     p_{14}^1 & p_{14}^2 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & -v_{14}^1 & 0 & 0 & 0 \\
     p_{23}^1 & p_{23}^2 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & -v_{23}^1 & 0 & 0 \\
     p_{24}^1 & p_{24}^2 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & -v_{24}^1 & 0 \\
     p_{34}^1 & p_{34}^2 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & -v_{34}^1 \\ %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
     0 & 0 & p_{12}^1 & p_{12}^2 & 0 & 0 & 0 & 1 & 0 & -v_{12}^2 & 0 & 0 & 0 & 0 & 0 \\
     0 & 0 & p_{13}^1 & p_{13}^2 & 0 & 0 & 0 & 1 & 0 & 0 & -v_{13}^2 & 0 & 0 & 0 & 0 \\
     0 & 0 & p_{14}^1 & p_{14}^2 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & -v_{14}^2 & 0 & 0 & 0 \\
     0 & 0 & p_{23}^1 & p_{23}^2 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & -v_{23}^2 & 0 & 0 \\
     0 & 0 & p_{24}^1 & p_{24}^2 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & -v_{24}^2 & 0 \\
     0 & 0 & p_{34}^1 & p_{34}^2 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & -v_{34}^2 \\ %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
     0 & 0 & 0 & 0 & p_{12}^1 & p_{12}^2 & 0 & 0 & 1 & -v_{12}^3 & 0 & 0 & 0 & 0 & 0 \\
     0 & 0 & 0 & 0 & p_{13}^1 & p_{13}^2 & 0 & 0 & 1 & 0 & -v_{13}^3 & 0 & 0 & 0 & 0 \\
     0 & 0 & 0 & 0 & p_{14}^1 & p_{14}^2 & 0 & 0 & 1 & 0 & 0 & -v_{14}^3 & 0 & 0 & 0 \\
     0 & 0 & 0 & 0 & p_{23}^1 & p_{23}^2 & 0 & 0 & 1 & 0 & 0 & 0 & -v_{23}^3 & 0 & 0 \\
     0 & 0 & 0 & 0 & p_{24}^1 & p_{24}^2 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & -v_{24}^3 & 0 \\
     0 & 0 & 0 & 0 & p_{34}^1 & p_{34}^2 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & -v_{34}^3
    \end{array}\right)_{18\times 15}
% }
 \end{equation*}
\end{figure*}

% \begin{proof}
%      \bh{Taken from Will's proof}
%  Call $(u^{k\ell})=U:=sR-I$, which will be viewed as an element in $M_{3\times 3}$
%  (superscripts will denote components of vectors/matrices while subscripts will be
%  used for indexing). In order to have $H\cdot p_{ij}\in V_i\cap V_j$, we
%  need
% 
%  \begin{equation}\label{eq:linear_sys}
%     U\cdot p_{ij} + t = \alpha_{ij}\cdot v_{ij}, \quad v_{ij} = n_i\times n_j,
%  \end{equation}
% where the $\alpha_{ij}\in\mathbb{R}$ are unknown multipliers. By relaxing from
% rotations to arbitrary matrices, \eqref{eq:linear_sys} becomes a linear system of
% equations:
% 
%  \begin{equation}\label{eq:linear_sys_part2}
%      \sum_{\ell=1}^3 \, u^{k\ell}\cdot p_{ij}^\ell + t^k = \alpha_{ij}\cdot v_{ij}^k.
%  \end{equation}
% This system has $3n$ equations and $12+n$ unknowns where $n$ is the number of
% $p_{ij}$. In our case, $n=6$ and \eqref{eq:linear_sys_part2} forms an 18 by 18
% system. Therefore if its matrix is non-singular, there exists a unique solution. The
% matrix is given by
% 
%  \begin{equation}\label{eq:18_matrix}
%      A = \begin{bmatrix}
%      X & 0 & 0 & 1_{6\times 1} & 0 & 0 & -\Lambda_1 \\
%      0 & X & 0 & 0 & 1_{6\times 1} & 0 & -\Lambda_2 \\
%      0 & 0 & X & 0 & 0 & 1_{6\times 1} & -\Lambda_3
%     \end{bmatrix},
%  \end{equation}
%  where
%  \begin{equation*}
%     \begin{split}
%         X &= \left[ p_{12},p_{13},p_{14},p_{23},p_{24},p_{34}\right]^\intercal \\
%         \Lambda_k &= \mathrm{diag}\left[ v_{12}^k, v_{13}^k, v_{14}^k, v_{23}^k, v_{24}^k, v_{34}^k \right].
%     \end{split}
%  \end{equation*}
%  \end{proof}

% \begin{remark}
%     \bh{need to be rephrased later on}
%    The matrix $A$ has three columns which are trivially zero. This leaves the last
%    column of $U$ free (so uniqueness fails). But! a (3 dimensional) rotation matrix is
%    uniquely determined by its first two columns (as the third is taken to be the third
%    ONB). Therefore, we obtain a unique rotation matrix and the result holds.
% \end{remark}
 
% The matrix is an 18 by 15 matrix and is given by
% \begin{figure*}[b]%% over both columns
% \center
%  \begin{equation*}
% 	% \resizebox{0.93\hsize}{!}{%
%      A = \left(\begin{array}{ccccccccccccccc}
%      p_{12}^1 & p_{12}^2 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & -v_{12}^1 & 0 & 0 & 0 & 0 & 0 \\
%      p_{13}^1 & p_{13}^2 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & -v_{13}^1 & 0 & 0 & 0 & 0 \\
%      p_{14}^1 & p_{14}^2 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & -v_{14}^1 & 0 & 0 & 0 \\
%      p_{23}^1 & p_{23}^2 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & -v_{23}^1 & 0 & 0 \\
%      p_{24}^1 & p_{24}^2 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & -v_{24}^1 & 0 \\
%      p_{34}^1 & p_{34}^2 & 0 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & -v_{34}^1 \\ %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%      0 & 0 & p_{12}^1 & p_{12}^2 & 0 & 0 & 0 & 1 & 0 & -v_{12}^2 & 0 & 0 & 0 & 0 & 0 \\
%      0 & 0 & p_{13}^1 & p_{13}^2 & 0 & 0 & 0 & 1 & 0 & 0 & -v_{13}^2 & 0 & 0 & 0 & 0 \\
%      0 & 0 & p_{14}^1 & p_{14}^2 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & -v_{14}^2 & 0 & 0 & 0 \\
%      0 & 0 & p_{23}^1 & p_{23}^2 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & -v_{23}^2 & 0 & 0 \\
%      0 & 0 & p_{24}^1 & p_{24}^2 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & -v_{24}^2 & 0 \\
%      0 & 0 & p_{34}^1 & p_{34}^2 & 0 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & -v_{34}^2 \\ %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%      0 & 0 & 0 & 0 & p_{12}^1 & p_{12}^2 & 0 & 0 & 1 & -v_{12}^3 & 0 & 0 & 0 & 0 & 0 \\
%      0 & 0 & 0 & 0 & p_{13}^1 & p_{13}^2 & 0 & 0 & 1 & 0 & -v_{13}^3 & 0 & 0 & 0 & 0 \\
%      0 & 0 & 0 & 0 & p_{14}^1 & p_{14}^2 & 0 & 0 & 1 & 0 & 0 & -v_{14}^3 & 0 & 0 & 0 \\
%      0 & 0 & 0 & 0 & p_{23}^1 & p_{23}^2 & 0 & 0 & 1 & 0 & 0 & 0 & -v_{23}^3 & 0 & 0 \\
%      0 & 0 & 0 & 0 & p_{24}^1 & p_{24}^2 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & -v_{24}^3 & 0 \\
%      0 & 0 & 0 & 0 & p_{34}^1 & p_{34}^2 & 0 & 0 & 1 & 0 & 0 & 0 & 0 & 0 & -v_{34}^3
%     \end{array}\right)
% % }
%  \end{equation*}
% \end{figure*}





==> Target-Vertices-LiDAR-Frame.tex <==
\section{Finding the \lidar Vertices}
\label{sec:LiDARVertices}


==> Uniqueness.tex <==
\setcounter{theorem}{0}
\setcounter{assumption}{0}
\section{Proof on Uniqueness of Similarity Transformation}
\label{sec:Uniqueness}
This section completes the proof in \ref{sec:TargetPlacementGuideline} and
\bh{cite[Proposition 1]{AutomaticCalibration}}. It provides a guideline to place
targets such that an answer to the optimization problem is unique. In particular,
under Assumption~\ref{eq:assumtionN} and Assumption~\ref{eq:assumtionB}\bh{need to
fix numbers}, the optimization problem has only one unique answer. As stated in
Sec.~\ref{sec:ProposedIntrinsicModel}, the intrinsic calibration parameters are
modeled as an element of the similarity Lie group ($\Sim(3)$). An element of this
group in matrix from is
\begin{equation}
    \H = 
    \begin{bmatrix}
        s\R & \t \\
        \zeros & 1
    \end{bmatrix} \in \Sim(3),
\end{equation}
where $\R\in\SO(3), \t \in \reals^3$ and $s \in \reals^+$.


\subsection{Mathematical Definitions and Preliminaries}
Let $[\Scal]$ and $[\Scal]^\perp$ be the span and its orthogonal complement of
$\Scal\subset \realnumbers^3$, respectively\footnote{$\because \Scal \subset
\real^3$, $[\Scal]=\real^3 \iff [\Scal]^\perp =0$}. We denote the union of
intersection of $K$ spans as $\left( [\Scal_1] + [\Scal_2] + \cdots +
[\Scal_K]\right) = \cap_{i=1}^K[\Scal_i]$. Let $\P \subset \real^3$ be a plane.
$\P$ modeled the set traced out by a single ring of a perfectly calibrated
spinning \lidarN. Let $\{\e[1], \e[2], \e[3] \}$ denote the canonical basis for
$\real^3$. Without loss of generality, we assume $\P=[\e[3]]^\perp = \{\e[1],
\e[2]\}$. Therefore, $\forall s>0, \R\in\SO(3)$, 
$$ (s\R -\I)(\P)=0 \iff s=1, \R=\I.\footnote{$(s\R-\I)(\P) = [(s\R-\I)\e[1]] +
[(s\R-\I)\e[2])]$}$$


\subsection{Assumptions}
Consider four targets with unit normal vectors $\n[i]$ and let $\p[0, i]$ be a points
on the $i$-th target. 

\begin{assumption}[Assumption N]
    \label{eq:assumtionN}
    All sets of three distinct vectors from $\{ \n[1], \n[2], \n[3], \n[4], \e[3]\}$
    are \li.
\end{assumption}

For $1\le i \le 4$, the plane defined by the $i$-th target is $\V[i]:= \p[0,i] +
[\n[i]]^\perp.$ Under Assumption~\ref{eq:assumtionN}, some facts are listed below
without proofs:

\begin{enumerate}[(a)]
    \item $\V[i] \cap \V[j]=\p[ij] + [\n[i], \n[j]]^\perp$.

    \item For each $i \neq j \in \{1, 2, 3, 4 \}$, $\p[ij]:=\P \cap \V[i] \cap \V[j]$
        exists and is unique. There are $\binom{4}{2}$ intersection points.

    \item  $\H\cdot \p[ij] \in \V[i] \cap \V[j]$ if, and only if, $$(s \R-\I)\p[ij]
        +\t \in [\n[i], \n[j]]^\perp. $$

    \item Because $\dim [\n[i], \n[j]]^\perp=1$,  $(s \R-\I)\p[ij] +\t  \neq 0$ if,
        and only if, $ [(s \R-\I)\p[ij] +\t] = [\n[i], \n[j]]^\perp. $

    \item Let $\{\p[a], \p[b] \}$ be a basis for $\P$. Then $(s \R-\I)(\P)=0$ if,
        and only if, $(s \R-\I)(\p[a])=0$ and $(s \R-\I)(\p[b])=0$.
\end{enumerate}


\begin{assumption}[Assumption B]
    \label{eq:assumtionB}
    Given the six intersection points, any two form a set of basis for the ring
    plane. There are $\binom{6}{2}$ sets of basis. Subsets of the basis' are \li.
    \begin{enumerate}[(a)]
        \item $\{ \p[12], \p[13] \}$, $\{ \p[13], \p[14] \}$, $\{ \p[14], \p[12] \}$,
        \item $\{ \p[12], \p[23] \}$, $\{ \p[23], \p[24] \}$, $\{ \p[24], \p[12] \}$,
        \item $\{ \p[13], \p[23] \}$, $\{ \p[23], \p[34] \}$, $\{ \p[34], \p[13] \}$,
        \item $\{ \p[14], \p[24] \}$, $\{ \p[24], \p[34] \}$, $\{ \p[34], \p[14] \}$,
        \item $\{ \p[14], \p[23] \}$
    \end{enumerate}
\end{assumption}

\subsection{A Complete Proof}
\begin{theorem} 
    Assume that Assumptions N (Assumption~\ref{eq:assumtionN}) and B
    (Assumption~\ref{eq:assumtionB}) hold and let $\H \in \Sim(3)$. If for each $i
    \neq j \in \{1, 2, 3, 4 \}$, $\H\cdot\p[ij] \in  \V[i] \cap
     \V[j]$, then 
     \begin{equation} 
         \H = 
         \begin{bmatrix}
            \I & \zeros \\
            \zeros & 1
         \end{bmatrix}.
     \end{equation}
 \end{theorem}


\begin{proof} 
The proof is by exhaustion on the dimension of $(s\R-\I)(\P)$. We have that
$\H\cdot\p[ij] = s\R \p[ij] + \t$, and therefore 
\begin{equation}
\label{eq:NecssSuff}
   \H\cdot\p[ij] \in  \V[i] \cap \V[j] \iff (s\R-\I) \p[ij] + \t \in [\n[i], \n[j]]^\perp. 
\end{equation}
 
\begin{itemize}

\item \textbf{Case 1:} $\dim (s\R-\I)(\P) =0$. \par
    Then $\t \in [\n[i],
\n[j]]^\perp$ for all $i\neq j$. Hence, $\t \in [\n[1], \n[2]]^\perp \cap
[\n[2], \n[3]]^\perp =0$, which implies that $\t=0$. Therefore, by
\textbf{Simple Fact 1}, we are done. We next show that $\dim (s\R-\I)(\P) > 0$
and $\H\cdot\p[ij] \in  \V[i] \cap \V[j]$ for all $i \ne j$ lead to
contradictions.
 
 
\item  \textbf{Case 2:} $\dim (s\R-\I)(\P) =1$ \par
    (a) Suppose $\t \not \in (s\R-\I)(\P)$. Then, for any $\p[ij]$, $(s\R-\I)\p[ij] +
    \t \neq 0$. Hence, 
    \begin{align*}
     [\n[1], \n[2]]^\perp &= [(s\R-\I)(\p[12]) + \t] \\
     [\n[2], \n[3]]^\perp &= [(s\R-\I)(\p[23]) +\t] \\
      [\n[3], \n[4]]^\perp &= [(s\R-\I)(\p[34]) +\t].
    \end{align*}
Because $[\n[1], \n[2]] \cap [\n[2], \n[3]]\cap [\n[3], \n[4]] =0$, we have
that $[\n[1], \n[2]]^\perp + [\n[2], \n[3]]^\perp +  [\n[3], \n[4]]^\perp =
\real^3$. We deduce that $\dim (s\R-\I)(\P) =2$, which is a contradiction. \\

(b) Suppose $\t \in (s\R-\I)(\P)$ and thus there exists $\p[t]\in \P$ such that
$\t=(s\R-\I)(\p[t])$. The condition \eqref{eq:NecssSuff} can therefore be written as
\begin{equation}
\label{eq:NecssSuffWithT}
   \H\cdot\p[ij] \in  \V[i] \cap \V[j] \iff (s\R-\I)( \p[ij] + \p[t]) \perp \{\n[i],\n[j] \}. 
\end{equation}

  Because  $\{ \p[12], \p[13] \}$,  $\{ \p[13], \p[14] \}$,  $\{ \p[14], \p[12] \}$
  are bases for $\P$, we conclude that 
  \begin{equation}
      [\p[12]+\p[t], \p[13]+\p[t], \p[14]+\p[t] ]=\P.
  \end{equation}
  Applying \eqref{eq:NecssSuffWithT} to this set of vectors, we deduce that
  $$(s\R-\I)(\P) \perp \n[1].$$ 
  Applying the same reasoning to $\{ \p[12], \p[23] \}$,
  $\{ \p[23], \p[24] \}$, $\{ \p[24], \p[12] \}$ , we deduce that $(s\R-\I)(\P) \perp
  \n[2]$. Repeating again, we have $(s\R-\I)(\P) \perp \n[3]$ and thus $\dim
  (s\R-\I)(\P)=0$. 
 

\item  \textbf{Case 3:} $\dim (s\R-\I)(\P) =2$ \par
    We rewrite \eqref{eq:NecssSuff} as
    \begin{equation}
    \label{eq:NecssSuffv02}
       \H\cdot\p[ij] \in  \V[i] \cap \V[j] \iff -\t \in  (s\R-\I) \p[ij] +[\n[i], \n[j]]^\perp. 
    \end{equation}
Hence, if for all  $i \neq j \in \{1, 2, 3, 4 \}$, $\H\cdot\p[ij] \in  \V[i] \cap
\V[j]$, then the lines $(s\R-\I) \p[ij] +[\n[i], \n[j]]^\perp$ in $\real^3$ must have
a common point of intersection, namely $-\t$ and hence
\begin{equation} 
\label{eq:MasternIntersection}
\bigcap \limits_{i \neq j \in \{1, 2, 3, 4 \}} \{ (s\R-\I) \p[ij] + [\n[i], \n[j]]^\perp \} \neq \emptyset.
\end{equation}

\begin{remark}  
    When $(s\R-\I)(\P)=0$, the intersections in \eqref{eq:MasternIntersection} are
    non-empty; indeed, the equation reduces to 
    $$\bigcap \limits_{i \neq j \in \{1,
    2, 3, 4 \}} [\n[i], \n[j]]^\perp = \left(~ \sum \limits_{i \neq j} [\n[i], \n[j]]
    ~\right)^\perp = (\real^3)^\perp =0,$$
and hence $\t=0$.
\end{remark}

In the remainder of the proof, we show the intersection being non-empty
contradicts ${\rm dim}~(s\R-\I)(\P) = 2$. We do this by examining the
intersections in \eqref{eq:MasternIntersection} pairwise to arrive at a set of
necessary conditions for $\H \cdot \p[ij] \in  \V[i] \cap \V[j]$ for $i \neq
j$, and then use the necessary conditions to complete the proof. We note that for $ij
\neq kl$, 
  
\begin{align*}
 &\{ (s\R-\I) \p[ij] + [\n[i], \n[j]]^\perp \} \cap \{ (s\R-\I) \p[kl] +
[\n[k], \n[l]]^\perp \} \neq \emptyset \\
 &\iff (s\R-\I)(\p[ij] -  \p[kl]) \in
[\n[i], \n[j]]^\perp  + [\n[k], \n[l]]^\perp.
\end{align*}
 
 The indices are a bit easier to keep track of if we set 
 \begin{align}
 &\q[1]:=(s\R-\I)(\p[12]), ~\U[1]:=[\n[1], \n[2]]^\perp \nonumber\\
 &\q[2]:=(s\R-\I)(\p[13]), ~\U[2]:=[\n[1], \n[3]]^\perp \nonumber\\
 &\q[3]:=(s\R-\I)(\p[23]), ~\U[3]:=[\n[1], \n[4]]^\perp \nonumber\\
 &\q[4]:=(s\R-\I)(\p[14]), ~\U[4]:=[\n[2], \n[3]]^\perp \nonumber,
 \end{align}
 where $\{\U[k]|k=1,\cdots,4\}$ denote the indicated one-dimensional subspaces. Then,
 for each $i \neq j \in \{1, 2, 3, 4 \}$, $\U[i] \cap \U[j] =0$, and we have $\U[1]
 \oplus \U[2] \oplus \U[3]=\real^3$. Let $\u[i]$ be a basis for $\U[i]$, so that
 $\U[i] = [\u[i]]$, and write $$\u[4] =\alpha \u[1] + \beta \u[2] + \gamma \u[3].$$


\begin{claim} 
\label{claim:abg}
Each of the coefficients $\alpha, \beta, \gamma$ is non-zero.
\end{claim}
\begin{proof}  Suppose $\alpha=0$. Then $\U[4] \subset \U[2] + \U[3]$, that is,
$$[\n[2], \n[3]]^\perp  \subset [\n[1], \n[3]]^\perp +[\n[1], \n[4]]^\perp $$ But this is equivalent to
$$ [\n[1]] = [\n[1], \n[3]] \cap [\n[1], \n[4]]  \subset [\n[2], \n[3]], $$ and hence $\{
\n[1], \n[2], \n[3]\}$ is not linearly independent, contradicting Assumption N. The same argument holds for the other coefficients. 
 \end{proof}
 
 \begin{claim}  A necessary condition for 
\begin{equation} 
\label{eq:MasternIntersection}
\bigcap \limits_{i=1}^{4}  \{\q[i] + \U[i] \} \neq \emptyset
\end{equation}
is that there exist real numbers $c_1, c_2, c_3, c_4$ such that
\begin{equation}
\label{eq:SimulEqns}
\begin{aligned}
    \Delta \q[12]:=\q[1]-\q[2]&=c_1 \u[1] + c_2\u[2] \\
    \Delta \q[13]:=\q[1]-\q[3]&=c_1 \u[1] + c_3\u[3] \\
    \Delta \q[14]:=\q[1]-\q[4]&=c_1 \u[1] + c_4 \u[4] \\
    \Delta \q[23]:=\q[2]-\q[3]&=c_3 \u[3] - c_2\u[2] \\
    \Delta \q[24]:=\q[2]-\q[4]&=c_4 \u[4] - c_2\u[2] \\
    \Delta \q[34]:=\q[3]-\q[4]&=c_3 \u[3] - c_4\u[4] \\
\end{aligned}
\end{equation}
\end{claim}

\begin{proof}
Each row of \eqref{eq:SimulEqns} corresponds to a condition of the form $\q[i]-\q[j] \in \U[i] \oplus \U[j]$. 
The proof proceeds by expressing each of the six rows in \eqref{eq:SimulEqns} with distinct coefficients (12 in total), and then writing down three necessary compatibility conditions, 
\begin{equation}
\label{eq:CompatibilityEqns}
\begin{aligned}
\Delta \q[12]-\Delta \q[13]+\Delta \q[23]&=0 \\
\Delta \q[12]-\Delta \q[14]+\Delta \q[24]&=0\\
\Delta \q[14]-\Delta \q[13]+\Delta \q[34]&=0.
\end{aligned}
\end{equation}
Because $-\t$ is in the intersection of the lines in \eqref{eq:MasternIntersection},
the resulting linear equations must have a solution, and indeed direct computation
shows that the set of solutions can be parameterized as given in the claim.
\end{proof}

The next step is to note that $[\Delta \q[12], \cdots, \Delta \q[34] ] \subset
(s\R-\I)(\P)$, and hence its dimension must be less than three. Additional
straightforward calculations show that
$$\dim ~[\Delta \q[12], \Delta \q[13], \Delta \q[34] ] =  {\rm rank~} 
\begin{bmatrix}
    c_1 & c_1 & -\alpha c_4 \\ c_2 & 0 & c_2 - \beta c_4 \\ 0 & c_3 &-\gamma c_4
\end{bmatrix}.
$$

In light of Claim~\ref{claim:abg}, the rank is less than three if, and only if, any
two coefficients of $\{ c_1, c_2, c_3, c_4\}$ are zero. But if this is the case, then
at least one row of \eqref{eq:SimulEqns} must be zero. Each row of
\eqref{eq:SimulEqns}, however, has the form $(s\R-\I)(\p[a] - \p[b])$, where
$\{\p[a], \p[b] \}$ is a basis for $\P$, and thus it cannot be the case that $\dim
(s\R-\I)(\P) = 2.$ This completes the proof. 
\end{itemize}
\end{proof}


==> Vertices_.tex <==
\section{Vertices Determination From \lidar  Measurement}
Vertices of a target is important feature for target-based extrinsic calibration,
target plane estimation, target pose estimation, etc. However, vertices are not
directly observable due to sparse \lidar point clouds. We proposed a concept of
$L_1$-inspired norm to estimate vertices in \cite[(2)]{huang2019improvements}. In the
paper, We seek a rigid body transformation from \lidar to the target, $H_L^T$, that
``best fits'' the ideal target onto the point cloud. In practice, it is actually
easier to pull the $\pc$ back to the origin of the \lidar through the inverse of the
current estimate of transformation $H_T^L:=(H_L^T)^{-1}$ and measure the error there.
For more details about this method, see \cite[Sec.~II]{huang2019improvements}.

However, instead of a diamond-shaped target stated in \cite{huang2019improvements},
we use the optimal shape in Sec.~\ref{sec:ShapeSensitivity}. The cost function
\cite[(3)]{huang2019improvements} has to be modified because the target is no longer
a square. This section will provide a generic cost function to the any polygonal
shape, the gradient, and the convexity analysis of the cost function.


\subsection{$L_1$-inspired cost function for a polygonal shape}
%The following is partially taken from \cite{huang2019improvements} to provide for
%clarity. 
Let $\pc := \{\calx_i\}_{i=1}^{M}$ be a collection of 3D points on a \lidar target,
where $M$ is the number of points. Given the target geometry (here is the optimal
shape determined in Sec.~\ref{sec:ShapeSensitivity}), we define an ideal target with
$m$ vertices $\bar{\Vcal} := \{ \bar{X}_i| \bar{X}_i=(y_i, z_i)\}_{i=1}^m$ located at
the origin of the \lidar with thickness $\epsilon$ as defined in
Fig.~\bh{fig:IdealFrame}. Without loss of generality, we assume the centroid of the
ideal target is at the origin of the \lidarN\footnote{the ideal target is a 2D shape
placed on $y$-$z$ plane with thickness $\epsilon$ on $x$-axis.}. 



\subsubsection{Region of interest}
Let $\Lcal :=\{l_i\}_{i=1}^m$ be the line equations\footnote{All the lines lie on
$y$-$z$ plane.} for the edges of the ideal target and are computed as 
\begin{align}
    l_i(\bar{X}_i, \bar{X}_{i+1}) := &(y_{i+1} - y_i)z + (z_i-z_{i+1})y \nonumber\\
                                     &-z_iy_{i+1} + z_{i+1}y_1 = 0,
    % l_i := \begin{cases}
    %     y = \frac{y_{i+1}-y_i}{x_{i+1}-x_i}(x-x_i)+y_i& \mbox{if } x_i \neq x_{i+1}\\
    %     x = x_i &\mbox{otherwise}
    % \end{cases}.
\end{align}
where $X_{m+1} = X_1$, $l_i$ is the line equation for the $i$-th edge of the ideal
target, and the $i$-th edge connects $\bar{X}_i$ and $\bar{X}_{i+1}$. 

Given a line $l_i$, the $y$-$z$ plane is split into two areas: $l_i>0$ and
$l_i<0$\footnote{$l_i=0$ is the line itself.}. We denote $\RI[i][+]$ and $\RI[i][-]$
as the area of $l_i>0$ and the area of $l_i<0$, respectively. Therefore, the ideal
target located the origin can be represented as a union of $\{RI_i\}_{i=1}^m$, called
``region of interest'' (\roiN):
\begin{equation}
    \RI[yz][*] = \bigcap_{i=1}^m \RI[i][*]
\end{equation}
where $\RI[i][*]$ is the region containing the ideal target. Specifically,
$\RI[yz][*]$ for the optimal shape in Fig.~\bh{fig:regionOfInterest} is 
\begin{equation}
    \RI[yz][*] = \RI[1][+] \cap \RI[2][-] \cap \RI[3][-]\cap \RI[4][+].
\end{equation}

Similarly, $\RI[xz][*]$ can be expressed as:
\begin{equation}
    \RI[xz][*] = \bigcap_{i=1}^2 \RI[i][*] = \RI[1][-]  \cap \RI[2][+],
\end{equation}
where again $\RI[i][*]$ is the region containing the
\begin{remark}
    $\RI[yz][*]$ is a polygonal shape with $m$ vertices and $\RI[xz][*]$ is two
    vertical lines separated $\epsilon$ away from each other. Thus, $\RI[yz][*]$ has
    $m$ unions and $\RI[xz][*]$ has $2$ unions.
\end{remark}


% Let $\RI[yz][*]$ be the \rio of the ideal target as shown
% in Fig.~\bh{fig:regionOfInterest} and is expressed as
% \begin{equation}
%     \RI[yz][*] = \bigcap_{i=1}^m \RI[i][*] = \RI[1][+] \cap \RI[2][-] \cap \RI[3][-]\cap \RI[4][+],
% \end{equation}


\subsubsection{Cost function of a polygonal shape}
Let $\{\tilde{\Xcal}_i\}_{i=1}^M:=H_T^L(\pc):=\{
H_T^L(\Xcal_i) \}_{i=1}^M$ denote the pullback of the point cloud by $H_T^L$, and
denote a point's Cartesian coordinates by $(\td[x]_i,\td[y]_i,\td[z]_i)$. Let
$\td[p]_{ixz}$ and $\td[p]_{iyz}$ be the orthogonal projection of $\td[\Xcal_i]$
onto $x$-$z$ plane and $y$-$z$ plane, respectively, as shown in
Fig.~\bh{fig:costFunction}. Because the 2D optimal shape is placed on $y$-$z$ plane with thickness $\epsilon$ ,
the cost function is computed from $y$-$z$ plane and $x$-$z$ plane. 


Let $\indicator(\td[p]_i, l_i)$ be the indicator function determining if $\td[p]_i$ is within
the $\RI[i][*]$ of $l_i$ and let $\Mcal(\td[p]_i, l_i)$ denote the Manhattan distance between
$\td[p]_i$ and $l_i$. The cost for a pullback point $\td[\Xcal_i]$ is defined as
\begin{align}
    f(\td[\Xcal_i]; \epsilon, \Lcal) &= f(H_T^L\Xcal_i; \epsilon, \Lcal) \nonumber\\
                                     &:= \Mcal_{xz}\indicator_{xz}(\td[p]_i, x=\epsilon) +
    \Mcal_{yz}\indicator_{yz}(\td[y]_i,\td[z]_i, \Lcal),
\end{align}
where $\indicator_x(\td[x]_i, \epsilon)$ and $\Mcal_x\indicator_x(\td[x]_i, \epsilon)$ are defined 
\begin{align}
    \indicator_{x}(\td[x]_i, \epsilon) &= 
    \begin{cases}
        1 & \text{if } \td[x]_i \notin \RI[x][*]\\
        0 & \text{if } \td[x]_i \in    \RI[x][*]\\
    \end{cases}, \\
    \Mcal_x\indicator_x(\td[x]_i, \epsilon) &= 
    \begin{cases}
        ~~(\td[x]_i - \frac{\epsilon}{2}) \cdot \indicator_x(\td[x]_i, \epsilon) & \text{if } \td[x]_i>0\\
        - (\td[x]_i + \frac{\epsilon}{2}) \cdot \indicator_x(\td[x]_i, \epsilon) & \text{if } \td[x]_i\leq0\\
    \end{cases}
\end{align}
and $\indicator_{yz}(\td[y]_i,\td[z]_i, l_i)$ and $\Mcal_{yz}\indicator_{yz}(\td[y]_i,\td[z]_i \Lcal)$ is defined 
\begin{align}
    \indicator_{yz}(\td[y]_i,\td[z]_i, l_i) &= 
    \begin{cases}
        1 & \text{if } (\td[y]_i,\td[z]_i) \notin \RI[i][*]\\
        0 & \text{if } (\td[y]_i,\td[z]_i) \in    \RI[i][*]\\
    \end{cases},\\
    \Mcal_{yz}\indicator_{yz}(\td[y]_i,\td[z]_i, \Lcal) &=
    \sum_{i=1}^m \frac{|a_i\td[y]_i + b_i\td[z]_i + c_i|}{\sqrt{a_i^2+b_i^2}} \indicator_{yz}(\td[y]_i,\td[z]_i, \Lcal)
\end{align}
and


% where $\Mcal_x\indicator_x(\td[x]_i, \epsilon)$ is defined 
% \begin{equation}
%     \Mcal_x\indicator_x(\td[x]_i, \epsilon) = 
%     \begin{cases}
%         ~~(\td[x]_i - \frac{\epsilon}{2}) \cdot \indicator_x(\td[x]_i, \epsilon) & \text{if } \td[x]_i>0\\
%         - (\td[x]_i + \frac{\epsilon}{2}) \cdot \indicator_x(\td[x]_i, \epsilon) & \text{if } \td[x]_i\leq0\\
%     \end{cases}
% \end{equation}


% Let $\RI_{yz}^*$ be the region of interest (\roiN) on $y$-$z$ plane and let $\RI_x^*$ be the
% \roi on $x$-$z$ plane as shown in Fig.~\bh{fig:regionOfInterest}.


% An edge is defined by two vertices of the shape. The 2D line equation for an edge
% given two vertices of the ideal target can be easily computed by

\subsubsection{Gradient of the cost function}


\subsection{Convexity Analysis}










==> Vertices_pre.tex <==
\section{Vertices Determination From $L_1-$ inspired cost}
\label{sec:VertexFromL1}
% Vertices of a target are important features for target-based extrinsic calibration,
% target plane estimation, target pose estimation, etc. However, vertices are not
% directly observable due to sparse \lidar point clouds. We proposed a concept of
% $L_1$-inspired norm to estimate vertices in \cite[(2)]{huang2020improvements}. In the
% paper, We seek a rigid body transformation from \lidar to the target, $H_L^T$, that
% ``best fits'' the ideal target onto the point cloud. In practice, it is actually
% easier to pull the $\pc$ back to the origin of the \lidar through the inverse of the
% current estimate of transformation $H_T^L:=(H_L^T)^{-1}$ and measure the error there.
% For more details about this method, see \cite[Sec.~II]{huang2020improvements}.
% 
% However, instead of a diamond-shaped target stated in \cite{huang2020improvements},
% the optimal shape in Sec.~\ref{sec:ShapeSensitivity} is used. The cost function
% \cite[(3)]{huang2020improvements} has to be modified because the target is no longer
% a square. Additionally, we use $L_2$ distance so that other convex relaxation
% techniques can be easily applied.
% %  and a method to determine if a
% % point is inside the polygon needs to be established 
% 
% This section will provide a method to determine if a point is inside an arbitrary
% planar polygon, a generic cost function to the polygon, the
% convexity analysis and the gradient of the cost function.
% 
% \subsection{Determine If a Point Is Inside an arbitrary planar polygon}
% \label{sec:InNOutPoints}
% Given an $m$ vertices planar polygon, we define an ideal target $\bar{\Vcal} := \{
% \bar{X}_i| \bar{X}_i=(y_i, z_i)\}_{i=1}^m$ located at the origin of the \lidar with
% thickness $\epsilon$. Specifically, the ideal target is a planar polygon placed on
% $y$-$z$ plane with thickness $\epsilon$ on $x$-axis as shown in
% Fig.~\bh{fig:IdealFrame}. Without loss of generality, we assume the centroid of the
% ideal target is at the origin of the \lidarN. To determine if a point is within the
% ideal target, the ideal target is represented as ``intersections of interest'' (see
% Sec.~\ref{sec:IoA}).
% 
% \subsubsection{Line equations for edges}
% \label{sec:IoE}
% An edge connects two vertices of the ideal target. Let $\Lcal :=\{l_i\}_{i=1}^m$ be
% the line equations\footnote{All the lines lie on $y$-$z$ plane.} for the edges of the
% ideal target and are computed as 
% \begin{align}
%     l_i(\bar{X}_i, \bar{X}_{i+1}) := &(y_{i+1} - y_i)z + (z_i-z_{i+1})y \nonumber\\
%                                      &-z_iy_{i+1} + z_{i+1}y_1 = 0,
%     % l_i := \begin{cases}
%     %     y = \frac{y_{i+1}-y_i}{x_{i+1}-x_i}(x-x_i)+y_i& \mbox{if } x_i \neq x_{i+1}\\
%     %     x = x_i &\mbox{otherwise}
%     % \end{cases}.
% \end{align}
% where $X_{m+1} = X_1$, $l_i$ is the line equation for the $i$-th edge of the ideal
% target, and the $i$-th edge connects $\bar{X}_i$ and $\bar{X}_{i+1}$ vertices. 
% 
% \subsubsection{Properties of 2D lines}
% \label{sec:PropertiesOf2DLines}
% Let $l_i$ be a 2D line lying on a plane. The 2D line splits the plane into two areas:
% $l_i>0$ and $l_i<0$\footnote{$l_i=0$ is the line itself.}. Let $\RI[i][+]$ and
% $\RI[i][-]$ be the area of $l_i>0$ and the area of $l_i<0$, respectively. We further
% denote the area containing the ideal target as $\RI[i][*]$.
% 
% 
% \subsubsection{Intersections of interest}
% \label{sec:IoA}
% Therefore, from Sec.~\ref{sec:IoE} and Sec.~\ref{sec:PropertiesOf2DLines}, the ideal
% target located the origin can be represented as intersections of areas
% ($\{RI_i^{*}\}_{i=1}^m$). We call the resulting intersection area ``region of
% interest'' (\roiN): 
% \begin{equation}
%     \RI[yz][*] = \bigcap_{i=1}^m \RI[i][*]
% \end{equation}
% where $\RI[i][*]$ is the region containing the ideal target. Specifically,
% $\RI[yz][*]$ for the optimal shape in Fig.~\bh{fig:regionOfInterest} is 
% \begin{equation}
%     \RI[yz][*] = \RI[1][+] \cap \RI[2][-] \cap \RI[3][-]\cap \RI[4][+].
% \end{equation}
% Similarly, $\RI[xz][*]$ can be expressed as:
% \begin{equation}
%     \RI[xz][*] = \bigcap_{i=1}^2 \RI[i][*] = \RI[1][-]  \cap \RI[2][+],
% \end{equation}
% where again $\RI[i][*]$ is the region containing the ideal target.
% \begin{remark}
%     $\RI[yz][*]$ results in the $m$-vertices polygon and $\RI[xz][*]$ is a stripe-area
%     between two vertical lines separated $\epsilon$ away from each other. Thus,
%     $\RI[yz][*]$ has $m$ intersections and $\RI[xz][*]$ has $2$ intersections.
% \end{remark}
% 
% 
% % Let $\RI[yz][*]$ be the \rio of the ideal target as shown
% % in Fig.~\bh{fig:regionOfInterest} and is expressed as
% % \begin{equation}
% %     \RI[yz][*] = \bigcap_{i=1}^m \RI[i][*] = \RI[1][+] \cap \RI[2][-] \cap \RI[3][-]\cap \RI[4][+],
% % \end{equation}
% 
% 
% \subsection{Cost Function of a Planar Polygon and Convexity Analysis}
% Let $\{\tilde{\Xcal}_k\}_{k=1}^M:=H_T^L(\pc):=\{ H_T^L(\Xcal_k) \}_{k=1}^M$ denote
% the pullback of the point cloud by $H_T^L$, and denote a point's Cartesian
% coordinates by $(\td[x]_k,\td[y]_k,\td[z]_k)$. Let $\td[p]_{k}$ be the orthogonal
% projection of $\td[\Xcal_k]$ onto $x$-$z$ plane ($\td[p]_{kxz}=(\td[x]_k,
% 0,\td[z]_k)$) or $y$-$z$ plane ($\td[p]_{kyz} = (0,\td[y]_k,\td[z]_k)$), as shown in
% Fig.~\bh{fig:costFunction}. 
% % Let $\td[p]_{kxz}$ and $\td[p]_{kyz}$
% % be the orthogonal projection of $\td[\Xcal_k]$ onto $x$-$z$ plane and $y$-$z$ plane,
% % respectively, as shown in Fig.~\bh{fig:costFunction}. 
% % Because the planar polygon is
% % placed on the $y$-$z$ plane with thickness $\epsilon$ on the $x$-$z$ plane, the cost
% % function is computed from $y$-$z$ plane and $x$-$z$ plane. 
% 
% 
% Let $\indicator(\td[p]_k, l_i)$ be the indicator function determining if $\td[p]_k$ is within
% the $\RI[i][*]$ of $l_i$ and is defined as
% \begin{equation}
%     \indicator(\td[p]_{k}, l_i) = 
%     \begin{cases}
%         1 & \text{if } \td[p]_{k} \notin \RI[][*]\\
%         0 & \text{if } \td[p]_{k} \in    \RI[][*]\\
%     \end{cases}.
% \end{equation}
% 
% Let $\EDis(\td[p]_{kxz}, l_i), \EDis(\td[p]_{kyz}, l_i)$ denote the Euclidean distance between
% $\td[p]_{kxz}$ and $l_i$, and $\td[p]_{kyz}$ and $l_i$, and are computed by
% \begin{align}
%     \label{eq:Mxz}
%     \EDis(\td[p]_{kxz}, l_i) &= \frac{|a_i\td[x]_{kxz} + b_i\td[z]_{kxz} + c_i|}{\sqrt{a_i^2+b_i^2}},\\
%     \label{eq:Myz}
%     \EDis(\td[p]_{kyz}, l_i) &= \frac{|a_i\td[y]_{kyz} + b_i\td[z]_{kyz} + c_i|}{\sqrt{a_i^2+b_i^2}}, 
% \end{align}
% where $a_i, b_i, c_i$ are line coefficients. 
% % Similarly, $\EDis(\td[p]_{kyz}, l_i)$ is
% % computed by
% % \begin{equation}
% %     \label{eq:Myz}
% %     \EDis(\td[p]_{kyz}, l_i)= \frac{|a_i\td[y]_{kyz} + b_i\td[z]_{kyz} + c_i|}{\sqrt{a_i^2+b_i^2}}, 
% % \end{equation}
% % where $a_i, b_i, c_i$ are line coefficients.
% 
% \subsubsection{Cost function}
% The cost for a pullback point $\td[\Xcal_k]$ is defined as
% \begin{align}
%     \label{eq:L1Cost}
%     f(\td[\Xcal_k]; \epsilon, \Lcal) &= f(H_T^L\Xcal_k; \epsilon, \Lcal) \nonumber\\
%                                      &:= \sum_{i=1}^2 \EDis_{xz}(\td[p]_{kxz}, l_i) \indicator_{xz}(\td[p]_{kxz}, l_i)\nonumber\\
%                                      &+ \sum_{i=1}^m \EDis_{yz}(\td[p]_{kyz}, l_i) \indicator_{yz}(\td[p]_{kyz}, l_i)
% %    \EDis_{yz}\indicator_{yz}(\td[p]_{kyz}, \Lcal),
% \end{align}
% \begin{remark}
%     Line equations on the $x$-$z$ plane are simply $x= \frac{\epsilon}{2}$ and $x=\frac{-\epsilon}{2}$.
% \end{remark}
% % where $\EDis_{xz}\indicator_{xz}(\td[p]_{kxz}, \epsilon)$ is defined 
% % \begin{align}
% %     \EDis_{xz}\indicator_{xz}(\td[p]_{kxz}, \epsilon) = 
% %     \begin{cases}
% %         ~~(\td[x]_k - \frac{\epsilon}{2})\indicator_{xz}(\td[p]_{kxz}, \epsilon) & \text{if } \td[x]_k>0\\
% %         - (\td[x]_k + \frac{\epsilon}{2})\indicator_{xz}(\td[p]_{kxz}, \epsilon) & \text{if } \td[x]_k\leq0\\
% %     \end{cases}
% % \end{align}
% % and $\EDis_{yz}\indicator_{yz}(\td[p]_{kyz}, \Lcal)$ is defined 
% % \begin{align}
% %     \EDis_{yz}\indicator_{yz}(\td[p]_{kyz}, \Lcal) &= \EDis_{yz}(\td[p]_{kyz}, l_1) + \cdots +\EDis_{yz}(\td[p]_{kyz}, l_m)\nonumber\\
% %                                                    &=\sum_{i=1}^m \frac{|a_i\td[y]_k + b_i\td[z]_k + c_i|}{\sqrt{a_i^2+b_i^2}} \indicator_{yz}(\td[p]_{kyz}, l_i)
% % \end{align}
% 
% 
% 
% 
% % The cost for a pullback point $\td[\Xcal_k]$ is defined as
% % \begin{align}
% %     f(\td[\Xcal_k]; \epsilon, \Lcal) &= f(H_T^L\Xcal_k; \epsilon, \Lcal) \nonumber\\
% %                                      &:= \EDis_{xz}\indicator_{xz}(\td[p]_{kxz}, \epsilon) +
% %     \EDis_{yz}\indicator_{yz}(\td[p]_{kyz}, \Lcal),
% % \end{align}
% % where $\indicator_x(\td[p]_{kxz}, \epsilon)$ and $\EDis_x\indicator_x(\td[p]_{kxz}, \epsilon)$ are defined 
% % \begin{align}
% %     \indicator_{x}(\td[p]_{kxz}, \epsilon) &= 
% %     \begin{cases}
% %         1 & \text{if } \td[p]_{kxz} \notin \RI[xz][*]\\
% %         0 & \text{if } \td[p]_{kxz} \in    \RI[xz][*]\\
% %     \end{cases}, \\
% %     \EDis_x\indicator_x(\td[p]_{kxz}, \epsilon) &= 
% %     \begin{cases}
% %         ~~(\td[x]_k - \frac{\epsilon}{2})\indicator_x(\td[p]_{kxz}, \epsilon) & \text{if } \td[x]_k>0\\
% %         - (\td[x]_k + \frac{\epsilon}{2})\indicator_x(\td[p]_{kxz}, \epsilon) & \text{if } \td[x]_k\leq0\\
% %     \end{cases}
% % \end{align}
% % and $\indicator_{yz}(\td[p]_{kyz}, l_i)$ and $\EDis_{yz}\indicator_{yz}(\td[p]_{kyz}, \Lcal)$ are defined 
% % \begin{align}
% %     \indicator_{yz}(\td[p]_{kyz}, l_i) &= 
% %     \begin{cases}
% %         1 & \text{if } \td[p]_{kyz} \notin \RI[yz][*]\\
% %         0 & \text{if } \td[p]_{kyz} \in    \RI[yz][*]\\
% %     \end{cases},\\
% %     \EDis_{yz}\indicator_{yz}(\td[p]_{kyz}, \Lcal) &= \EDis_{yz}(\td[p]_{kyz}, l_1) + \cdots +\EDis_{yz}(\td[p]_{kyz}, l_m)\nonumber\\
% %                                                    &=\sum_{i=1}^m \EDis_{yz}(\td[p]_{kyz}, l_i) \indicator_{yz}(\td[p]_{kyz}, l_i)\nonumber\\
% %                                                    &=\sum_{i=1}^m \frac{|a_i\td[y]_k + b_i\td[z]_k + c_i|}{\sqrt{a_i^2+b_i^2}} \indicator_{yz}(\td[p]_{kyz}, l_i)
% %     % \EDis_{yz}\indicator_{yz}(\td[p]_{kyz}, \Lcal) &= \EDis_{yz}(\td[p]_{kyz}, l_1) + \EDis_{yz}(\td[p]_{kyz}, l_2)\\
% %     %                                                & +\EDis_{yz}(\td[p]_{kyz}, l_3) + \EDis_{yz}(\td[p]_{kyz}, l_4)\\
% %     %                                                &=\sum_{i=1}^m \EDis_{yz}(\td[p]_{kyz}, l_i) \indicator_{yz}(\td[p]_{kyz}, l_i)\\
% %     %                                                &=\sum_{i=1}^m \frac{|a_i\td[y]_k + b_i\td[z]_k + c_i|}{\sqrt{a_i^2+b_i^2}} \indicator_{yz}(\td[p]_{kyz}, l_i)
% % \end{align}
% % where $\indicator_x(\td[p]_{kxz}, \epsilon)$ and $\EDis_x\indicator_x(\td[p]_{kxz}, \epsilon)$ are defined 
% % \begin{align}
% %     \indicator_{x}(\td[p]_{kxz}, \epsilon) &= 
% %     \begin{cases}
% %         1 & \text{if } \td[p]_{kxz} \notin \RI[xz][*]\\
% %         0 & \text{if } \td[p]_{kxz} \in    \RI[xz][*]\\
% %     \end{cases}, \\
% %     \EDis_x\indicator_x(\td[p]_{kxz}, \epsilon) &= 
% %     \begin{cases}
% %         ~~(\td[x]_k - \frac{\epsilon}{2})\indicator_x(\td[p]_{kxz}, \epsilon) & \text{if } \td[x]_k>0\\
% %         - (\td[x]_k + \frac{\epsilon}{2})\indicator_x(\td[p]_{kxz}, \epsilon) & \text{if } \td[x]_k\leq0\\
% %     \end{cases}
% % \end{align}
% % and $\indicator_{yz}(\td[p]_{kyz}, l_i)$ and $\EDis_{yz}\indicator_{yz}(\td[p]_{kyz}, \Lcal)$ are defined 
% % \begin{align}
% %     \indicator_{yz}(\td[p]_{kyz}, l_i) &= 
% %     \begin{cases}
% %         1 & \text{if } \td[p]_{kyz} \notin \RI[yz][*]\\
% %         0 & \text{if } \td[p]_{kyz} \in    \RI[yz][*]\\
% %     \end{cases},\\
% %     \EDis_{yz}\indicator_{yz}(\td[p]_{kyz}, \Lcal) &= \EDis_{yz}(\td[p]_{kyz}, l_1) + \cdots +\EDis_{yz}(\td[p]_{kyz}, l_m)\nonumber\\
% %                                                    &=\sum_{i=1}^m \EDis_{yz}(\td[p]_{kyz}, l_i) \indicator_{yz}(\td[p]_{kyz}, l_i)\nonumber\\
% %                                                    &=\sum_{i=1}^m \frac{|a_i\td[y]_k + b_i\td[z]_k + c_i|}{\sqrt{a_i^2+b_i^2}} \indicator_{yz}(\td[p]_{kyz}, l_i)
% %     % \EDis_{yz}\indicator_{yz}(\td[p]_{kyz}, \Lcal) &= \EDis_{yz}(\td[p]_{kyz}, l_1) + \EDis_{yz}(\td[p]_{kyz}, l_2)\\
% %     %                                                & +\EDis_{yz}(\td[p]_{kyz}, l_3) + \EDis_{yz}(\td[p]_{kyz}, l_4)\\
% %     %                                                &=\sum_{i=1}^m \EDis_{yz}(\td[p]_{kyz}, l_i) \indicator_{yz}(\td[p]_{kyz}, l_i)\\
% %     %                                                &=\sum_{i=1}^m \frac{|a_i\td[y]_k + b_i\td[z]_k + c_i|}{\sqrt{a_i^2+b_i^2}} \indicator_{yz}(\td[p]_{kyz}, l_i)
% % \end{align}
% 
% 
% % where $\EDis_x\indicator_x(\td[x]_i, \epsilon)$ is defined 
% % \begin{equation}
% %     \EDis_x\indicator_x(\td[x]_i, \epsilon) = 
% %     \begin{cases}
% %         ~~(\td[x]_i - \frac{\epsilon}{2}) \cdot \indicator_x(\td[x]_i, \epsilon) & \text{if } \td[x]_i>0\\
% %         - (\td[x]_i + \frac{\epsilon}{2}) \cdot \indicator_x(\td[x]_i, \epsilon) & \text{if } \td[x]_i\leq0\\
% %     \end{cases}
% % \end{equation}
% 
% 
% % Let $\RI_{yz}^*$ be the region of interest (\roiN) on $y$-$z$ plane and let $\RI_x^*$ be the
% % \roi on $x$-$z$ plane as shown in Fig.~\bh{fig:regionOfInterest}.
% 
% 
% % An edge is defined by two vertices of the shape. The 2D line equation for an edge
% % given two vertices of the ideal target can be easily computed by
% 
% 
% \subsubsection{Convexity Analysis}
% \bh{NEED TO CHECK AGAIN AT THE END}
% From \cite[3.1.2]{boyd2004convex}, if set $C$ is convex, then its indicator function
% is convex. Therefore, $\indicator_{xz}$ and $\indicator_{yz}$ are convex because
% $\RI[xz][*]$ and $\RI[yz][*]$ are convex. From \cite[3.1.1, 3.1.5]{boyd2004convex}, all
% affine functions are convex (and concave), and powers of absolute value is convex on
% $\reals$. Therefore, \eqref{eq:Mxz} and \eqref{eq:Myz} are both convex. This concludes  
% \eqref{eq:L1Cost} is convex. However, the domain ($\SE(3)$) is not convex. Further
% convex relaxation \cite{Rosen2019SESync, horowitz2014convex, yang2020graduated} could be applied.
% 
% \subsection{Gradient of the cost function}
% The gradient of the cost function is essential when one utilizes gradient decent
% solvers to solve an optimization problem. It is not only critical in our case to
% solve the $H_L^T$ transformation but also to include the gradient of the cost
% function to find the optimal shape in Sec.~\ref{sec:ShapeSensitivity} so that the
% resulting shape is also sensitive to the gradient, and thus further improves vertices
% estimation.
% 
% 
% Let $H$ be a rigid-body transform:
% \begin{equation}
%    H := 
%    \begin{bmatrix}
%        R & T \\
%        \zeros &1
%    \end{bmatrix} = 
%    \begin{bmatrix}
%        r_{11} & r_{12} & r_{13} & t_{1} \\
%        r_{21} & r_{22} & r_{23} & t_{2} \\
%        r_{31} & r_{32} & r_{33} & t_{3} \\
%        0 & 0 & 0 & 1
%    \end{bmatrix}\nonumber.
% \end{equation}
% 
% Let $\nabla_Hf$ be the gradient of \eqref{eq:L1Cost} with respect to $H$ and is computed 
% \begin{equation}
%    \nabla_Hf := 
%    \begin{bmatrix}
%        \pdv{f}{r_{11}} & \pdv{f}{r_{12}} & \pdv{f}{r_{13}} & \pdv{f}{t_{1}} \\
%        \pdv{f}{r_{21}} & \pdv{f}{r_{22}} & \pdv{f}{r_{23}} & \pdv{f}{t_{2}} \\
%        \pdv{f}{r_{31}} & \pdv{f}{r_{32}} & \pdv{f}{r_{33}} & \pdv{f}{t_{3}}
%    \end{bmatrix}=
%    \begin{bmatrix}
%        \pdv{f}{\td[x]}x & \pdv{f}{\td[x]}y &  \pdv{f}{\td[x]}z & \pdv{f}{\td[x]} \\
%        \pdv{f}{\td[y]}x & \pdv{f}{\td[y]}y &  \pdv{f}{\td[y]}z & \pdv{f}{\td[y]} \\
%        \pdv{f}{\td[z]}x & \pdv{f}{\td[z]}y &  \pdv{f}{\td[z]}z & \pdv{f}{\td[z]}
%    \end{bmatrix},
% \end{equation}
% where $\pdv{f}{\td[x]}, \pdv{f}{\td[y]}, \pdv{f}{\td[z]}$ are
% \begin{align}
%     % \pdv{f}{\td[x]} &= 
%     % \begin{cases}
%     %      1 & \td[x] > \frac{\epsilon}{2} \\
%     %     -1 & \td[x] < \frac{-\epsilon}{2} \\
%     %      0 & \text{otherwise} 
%     % \end{cases}\\
%     \pdv{f}{\td[x]} &= \sum_{i=1}^2\pdv{\EDis_{xz}}{\td[x]}\indicator_{xz}(\td[p]_{xz}, l_i)\\ 
%     \pdv{f}{\td[y]} &= \sum_{i=1}^m\pdv{\EDis_{yz}}{\td[y]}\indicator_{yz}(\td[p]_{yz}, l_i)\\ 
%     \pdv{f}{\td[z]} &= \sum_{i=1}^m\pdv{\EDis_{yz}}{\td[z]}\indicator_{yz}(\td[p]_{yz}, l_i),
% \end{align}
% where $l_i$ is the line equation with coefficients $a_i, b_i, c_i$ and
% $\pdv{\EDis_{xz}}{\td[x]}, \pdv{\EDis_{yz}}{\td[y]}, \pdv{\EDis_{yz}}{\td[z]}$ are
% \begin{align}
%     \pdv{\EDis_{xz}}{\td[x]} &= 
%     \begin{cases}
%          1 & \td[x] > \frac{\epsilon}{2} \\
%         -1 & \td[x] < \frac{-\epsilon}{2} \\
%          0 & \text{otherwise} 
%     \end{cases}, \\
%     \pdv{\EDis_{yz}}{\td[y]} &= 
%     \begin{cases}
%         \frac{a_i}{\sqrt{a_i^2+b_i^2}}  & a_i\td[y]+b_i\td[z]+c_i > 0\\
%         \frac{-a_i}{\sqrt{a_i^2+b_i^2}} & a_i\td[y]+b_i\td[z]+c_i < 0 \\
%          0 & \text{otherwise} 
%     \end{cases}, \\
%     \pdv{\EDis_{yz}}{\td[z]} &=
%     \begin{cases}
%         \frac{b_i}{\sqrt{a_i^2+b_i^2}}  & a_i\td[y]+b_i\td[z]+c_i > 0\\
%         \frac{-b_i}{\sqrt{a_i^2+b_i^2}} & a_i\td[y]+b_i\td[z]+c_i < 0 \\
%          0 & \text{otherwise} 
%     \end{cases}.
% \end{align}



% Apply the chain role, we have
% \begin{align}
%     \pdv{f}{r_{11}} =  \pdv{f}{\td[x]}\pdv{\td[x]}{r_{11}} &= \pdv{f}{\td[x]}x,~~\pdv{f}{r_{12}} =  \pdv{f}{\td[x]}y,~~\pdv{f}{r_{13}} =  \pdv{f}{\td[x]}z\nonumber\\
%     \pdv{f}{r_{21}} =  \pdv{f}{\td[y]}\pdv{\td[y]}{r_{21}} &= \pdv{f}{\td[y]}x,~~\pdv{f}{r_{22}} =  \pdv{f}{\td[y]}y,~~\pdv{f}{r_{23}} =  \pdv{f}{\td[y]}z\nonumber\\
%     \pdv{f}{r_{31}} =  \pdv{f}{\td[z]}\pdv{\td[z]}{r_{31}} &= \pdv{f}{\td[z]}x,~~\pdv{f}{r_{32}} =  \pdv{f}{\td[z]}y,~~\pdv{f}{r_{33}} =  \pdv{f}{\td[z]}z\nonumber\\
%     \pdv{f}{t_{1}} &= \pdv{f}{\td[x]},~~~~~\pdv{f}{t_{2}} = \pdv{f}{\td[y]},~~~~~\pdv{f}{t_{3}} = \pdv{f}{\td[z]}
% \end{align}




==> defines.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Packages
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% normal packages
\usepackage{bmpsize}
\usepackage{amsthm}
\usepackage{algorithm, algorithmicx, algpseudocode}
\usepackage{amsmath,amssymb,enumerate}
\usepackage{mathrsfs}
\usepackage{times}
\usepackage{multicol}
\usepackage{amsfonts}
\usepackage{textcomp}
\usepackage{balance}
\usepackage{multirow}
\usepackage{booktabs}
\usepackage{dblfloatfix} 

\usepackage{bbold}
\usepackage{makecell}
\usepackage{hhline} % double-line in a table

\usepackage{comment}
\usepackage{xparse}
\usepackage{lipsum}
\usepackage{soul} 
\usepackage{times}
\usepackage{balance}
\usepackage{dsfont} % indicator function
\usepackage{physics} % partial differential equation

% \usepackage{graphicx}
% \usepackage{fixltx2e}


% packages with options
\usepackage[dvipdfmx]{graphicx} 
\usepackage[T1]{fontenc}
\usepackage[usenames,dvipsnames,svgnames,table, xcdraw]{xcolor}
\usepackage[caption=false,font=footnotesize]{subfig}
\usepackage[utf8]{inputenc}
% \usepackage[title]{appendix}


% packages with setups
\usepackage{hyperref}
\hypersetup{
  colorlinks=true,pdfpagemode=UseNone,citecolor=black,linkcolor=black,urlcolor=BrickRed
}

\usepackage{caption}
\captionsetup{size=footnotesize,
    %justification=centering, %% not needed
    skip=5pt, position = bottom}
% \let\proof\relax 
% \let\endproof\relax



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Graphics path
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\graphicspath{
    {graphics/}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Theorem style
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newtheoremstyle{break}
  {\topsep}{\topsep}%
  {\itshape}{}%
  {\bfseries}{}%
  {\newline}{}%



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Environments
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newtheorem{problem}{Problem}
\newtheorem{theorem}{Theorem}
% \newtheorem{corollary}[theorem]{Corollary}
% \newtheorem{proposition}[theorem]{Proposition}
% \newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}{Proposition}
\newtheorem{remark}{Remark}
\newtheorem{fact}{Fact}
\newtheorem{definition}{Definition}
\newtheorem{example}{Example}

\theoremstyle{break}
% \newcounter{exercises}
\newtheorem{assumption}{Assumption}
% \setcounter{assumption}{0}

% \newtheorem{claim}[theorem]{Claim}
\newtheorem{claim}{Claim}

% proof style
\renewcommand\qedsymbol{$\blacksquare$}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Algorithm inputs
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \SetKwInput{KwInput}{Input}                % Set the Input
% \SetKwInput{KwOutput}{Output}              % set the Output


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Comments
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\hilight}[1]{\colorbox{yellow}{#1}} % to use: \hl{this is some highlighted text}
\newcommand{\red}[1]{{\textcolor{red}{#1}}}
\newcommand{\blue}[1]{{\textcolor{blue}{#1}}}
\newcommand{\rha}[1]{[{\textbf{\textcolor{orange}{Ross: #1}}}]}
\newcommand{\jwg}[1]{[{\textbf{\textcolor{red}{JWG: #1}}}]}
\newcommand{\mgj}[1]{[{\textbf{\textcolor{teal}{Maani: #1}}}]}
\newcommand{\jkh}[1]{[{\textbf{\textcolor{blue}{Bruce: #1}}}]}
\newcommand{\bh}[1]{[{\textbf{\textcolor{blue}{Bruce: #1}}}]}
\newcommand{\bht}[1]{[{\textbf{\textcolor{note}{Bruce: (TODO) #1}}}]}
\newcommand{\bhw}[1]{[{\textbf{\textcolor{note}{Bruce: working in progress #1}}}]}
\newcommand{\bhd}[1]{[{\textbf{\textcolor{blue}{Bruce: Done, please check#1}}}]}
\definecolor{note}{rgb}{0.3,0.7,0.25}
\definecolor{rephase}{rgb}{0.15,0.7,0.15}
\definecolor{bag}{rgb}{0.6,0.6,0.2}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Text Shortcuts
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\lc}{LiDAR-camera~}
\newcommand{\LC}{LiDAR-Camera~}
\newcommand{\lidar}{LiDAR~}
\newcommand{\lidarNoSpace}{LiDAR}
\newcommand{\lidarN}{LiDAR}
\newcommand{\lidars}{LiDARs~}
\newcommand{\lidarsN}{LiDARs}
\newcommand{\velodyne}{\textit{32-Beam Velodyne ULTRA Puck LiDAR~}}
\newcommand{\velodyneN}{\textit{32-Beam Velodyne ULTRA Puck LiDAR}}

\newcommand{\sslidar}{solid-state LiDAR~}
\newcommand{\sslidarN}{solid-state LiDAR}
\newcommand{\sslidars}{solid-state LiDARs~}
\newcommand{\sslidarsN}{solid-state LiDARs}

\newcommand{\slidar}{spining LiDAR~}
\newcommand{\slidarN}{spining LiDAR}
\newcommand{\slidars}{spining LiDARs~}
\newcommand{\slidarsN}{spining LiDARs}

\newcommand{\lidart}{LiDARTag~}
\newcommand{\lidarts}{LiDARTags~}
\newcommand{\lidartN}{LiDARTag}
\newcommand{\lidartsN}{LiDARTags}

\newcommand{\ltag}{LiDARTag~}
\newcommand{\ltagN}{LiDARTag}
\newcommand{\ltags}{LiDARTags~}
\newcommand{\ltagsN}{LiDARTags}

\newcommand{\atag}{AprilTag~}
\newcommand{\atags}{AprilTags~}
\newcommand{\atagN}{AprilTag}
\newcommand{\atagsN}{AprilTags}

\newcommand{\lind}{linearly independent}
\newcommand{\li}{linearly independent}
\newcommand{\ld}{linearly dependent}

\newcommand{\dom}{\mathrm{dom}}
\newcommand{\BL}{\textbf{BL}}
\newcommand{\bl}{\textbf{BL}}

% region of interest
\newcommand{\roi}{RoI~}
\newcommand{\rio}{RoI~}
\newcommand{\roiN}{RoI}
\newcommand{\rioN}{RoI}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% functionalities
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\squeezeup}{\vspace{-4mm}} % save space
% \long\def\/*#1*/{} % block comments: \/* */



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Mathematics Shortcuts
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\realnumbers{\mathbb{R}}
\def\real{\mathbb{R}}
\def\reals{\mathbb{R}}

\newcommand{\pc}{\mathcal{PC}}
\newcommand{\GPcal}{\mathcal{GP}}
\newcommand{\calx}{\mathcal{X}}
\newcommand{\dtheta}{\delta_\theta}
\newcommand{\dphi}{\delta_\phi}
\newcommand{\drho}{\delta_\rho}
\newcommand{\ep}{\mathcal{EP}}
\newcommand{\Pring}{\mathcal{P}}
\newcommand{\vx}{\mathcal{V}}
\newcommand{\lring}{\Lcal{\cal R}}


\newcommand{\indicator}{\mathds{1}}
\newcommand{\EDis}{\mathcal{ED}}
\DeclareDocumentCommand{\RI}{ O{} O{} }{\mathcal{RI}_{#1}^{#2}}
% \newcommand{\RI}{\mathcal{RI}} % region of interest

% operations
\newcommand{\floor}[1]{\lfloor #1 \rfloor}
\newcommand\inv[1]{#1\raisebox{1.15ex}{$\scriptscriptstyle-\!1$}}
%\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\DeclareDocumentCommand{\td}{ O{} }{\tilde{#1}}
\newcommand{\transpose}{\mathsf{T}}
% \newcommand{\span}[1]{\left{#1\right}}


% Groups and Algebra
\newcommand{\SO}{\mathrm{SO}}
\newcommand{\se}{\mathfrak{se}}
\newcommand{\SE}{\mathrm{SE}}
\newcommand{\Sim}{\mathrm{Sim}}
\newcommand{\Exp}{\mathrm{Exp}}
% \newcommand{\Log}{\mathrm{Log}}
% \newcommand{\Jr}{\mathrm{J_r}}

% Trigonometry
\DeclareDocumentCommand{\asin}{ O{} }{\sin^{-1}(#1)}
\DeclareDocumentCommand{\acos}{ O{} }{\cos^{-1}(#1)}
\DeclareDocumentCommand{\atan}{ O{} }{\tan^{-1}(#1)}


\DeclareDocumentCommand{\vector}{ O{} }{\mathrm{vec}(#1)}
\DeclareDocumentCommand{\zeros}{ O{} }{\textbf{0}_{#1}}
\DeclareDocumentCommand{\pre}{ O{} O{} }{{}_{#1}^{#2}}


% \newcommand{\GL}{\mathrm{GL}}

% \newcommand{\vecToSkew}{\wedge}
% \newcommand{\skewToVec}{\hat}
% \DeclareDocumentCommand{\vectorToSkew}{ O{} }{\left(#1\right)_\times}

% \newcommand{\bigO}[1]{\Ocal(#1)} % Big O
% \newcommand{\EV}[1]{\mathbb{E}[#1]} % Expected Value
% \newcommand{\Var}[1]{\mathbb{V}[#1]} % Variance
% \newcommand{\Covariance}[1]{\mathbf{Cov}[#1]} % Covariance

% \newcommand{\diag}{\mathop{\mathrm{diag}}}
% \newcommand{\m}{\mathop{\mathrm{m}}}
% \newcommand{\rad}{\mathop{\mathrm{rad}}}
% \newcommand{\dBm}{\mathop{\mathrm{dBm}}}
% \newcommand{\Hz}{\mathop{\mathrm{Hz}}}
% \newcommand{\GHz}{\mathop{\mathrm{GHz}}}
% \newcommand{\MHz}{\mathop{\mathrm{MHz}}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% New Operators
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
% \DeclareMathOperator*{\minimize}{minimize}
% \newcommand\scalemath[2]{\scalebox{#1}{\mbox{\ensuremath{\displaystyle #2}}}}
% \renewcommand{\thefigure}{\arabic{figure}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% -- Cal
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% uppers
% \newcommand{\Acal}{\mathcal{A}}
% \newcommand{\Bcal}{\mathcal{B}}
% \newcommand{\Ccal}{\mathcal{C}}
% \newcommand{\Dcal}{\mathcal{D}}
\newcommand{\Ecal}{\mathcal{E}}
% \newcommand{\Fcal}{\mathcal{F}}
% \newcommand{\Hcal}{\mathcal{H}}
% \newcommand{\Ical}{\mathcal{I}}
% \newcommand{\Kcal}{\mathcal{K}}
\newcommand{\Lcal}{\mathcal{L}}
\newcommand{\Mcal}{\mathcal{M}}
\newcommand{\Ncal}{\mathcal{N}}
% \newcommand{\Ocal}{\mathcal{O}}
\newcommand{\Rcal}{\mathcal{R}}
\newcommand{\Scal}{\mathcal{S}}
% \newcommand{\Tcal}{\mathcal{T}}
\newcommand{\Vcal}{\mathcal{V}}
\newcommand{\Xcal}{\mathcal{X}}
% \newcommand{\Ycal}{\mathcal{Y}}
% \newcommand{\Zcal}{\mathcal{Z}}


% lowers
% \newcommand{\dcal}{\text{\calligra d }}
% \newcommand{\ccal}{\text{\calligra c }}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% New commands for letters
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% uppers
\DeclareDocumentCommand{\A}{ O{} O{} }{\textbf{A}_{#1}^{#2}}
\DeclareDocumentCommand{\H}{ O{} O{} }{\textbf{H}_{#1}^{#2}}
\DeclareDocumentCommand{\I}{ O{} O{} }{\textbf{I}_{#1}^{#2}}
% \DeclareDocumentCommand{\J}{ O{} O{} }{\textbf{J}_{#1}^{#2}}
\DeclareDocumentCommand{\L}{ O{} O{} }{\textbf{L}_{#1}^{#2}}
\DeclareDocumentCommand{\M}{ O{} O{} }{\textbf{M}_{#1}^{#2}}
\DeclareDocumentCommand{\N}{ O{} O{} }{\textbf{N}_{#1}^{#2}}
\DeclareDocumentCommand{\P}{ O{} O{} }{\textbf{P}_{#1}^{#2}}
% \DeclareDocumentCommand{\Q}{ O{} O{} }{\textbf{Q}_{#1}^{#2}}
\DeclareDocumentCommand{\R}{ O{} O{} }{\textbf{R}_{#1}^{#2}}
% \DeclareDocumentCommand{\S}{ O{} O{} }{\textbf{S}_{#1}^{#2}}
\DeclareDocumentCommand{\T}{ O{} O{} }{\textbf{T}_{#1}^{#2}}
\DeclareDocumentCommand{\U}{ O{} O{} }{\textbf{U}_{#1}^{#2}}
\DeclareDocumentCommand{\V}{ O{} O{} }{\textbf{V}_{#1}^{#2}}
\DeclareDocumentCommand{\X}{ O{} O{} }{\textbf{X}_{#1}^{#2}}
\DeclareDocumentCommand{\Y}{ O{} O{} }{\textbf{Y}_{#1}^{#2}}
% \DeclareDocumentCommand{\Z}{ O{} O{} }{\textbf{Z}_{#1}^{#2}}


% lowers
\DeclareDocumentCommand{\e}{ O{} O{} }{\textbf{e}_{#1}^{#2}}
\DeclareDocumentCommand{\n}{ O{} O{} }{\textbf{n}_{#1}^{#2}}
\DeclareDocumentCommand{\t}{ O{} O{} }{\textbf{t}_{#1}^{#2}}
\DeclareDocumentCommand{\p}{ O{} O{} }{\textbf{p}_{#1}^{#2}}
\DeclareDocumentCommand{\q}{ O{} O{} }{\textbf{q}_{#1}^{#2}}
\DeclareDocumentCommand{\u}{ O{} O{} }{\textbf{u}_{#1}^{#2}}
\DeclareDocumentCommand{\v}{ O{} O{} }{\textbf{v}_{#1}^{#2}}
\DeclareDocumentCommand{\x}{ O{} O{} }{\textbf{x}_{#1}^{#2}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Other New commands
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \DeclareDocumentCommand{\CM}{ O{} O{} }{\tilde{\textbf{C}}_{#1}^{#2}}
% \DeclareDocumentCommand{\RM}{ O{} O{} }{\tilde{\textbf{R}}_{#1}^{#2}}
% \DeclareDocumentCommand{\dM}{ O{} O{} }{\tilde{\textbf{d}}_{#1}^{#2}}
% \DeclareDocumentCommand{\params}{ O{} O{} }{\boldsymbol{\theta}_{#1}^{#2}}
% \DeclareDocumentCommand{\paramsE}{ O{} O{} }{\hat{\boldsymbol{\theta}}_{#1}^{#2}}
% \DeclareDocumentCommand{\paramError}{ O{} O{} }{\boldsymbol{\zeta}_{#1}^{#2}}
% \DeclareDocumentCommand{\gyroscopeBias}{ O{} }{\textbf{b}_{#1}^{g}}
% \DeclareDocumentCommand{\gyroscopeBiasE}{ O{} }{\hat{\textbf{b}}_{#1}^{g}}
% \DeclareDocumentCommand{\accelerometerBias}{ O{} }{\textbf{b}_{#1}^{a}}
% \DeclareDocumentCommand{\accelerometerBiasE}{ O{} }{\hat{\textbf{b}}_{#1}^{a}}
% \DeclareDocumentCommand{\position}{ O{} O{} }{{}_\text{#2}\textbf{p}_{\text{#1}}}
% \DeclareDocumentCommand{\positionDot}{ O{} O{} }{{}_\text{#2}\dot{\textbf{p}}_{\text{#1}}}
% \DeclareDocumentCommand{\linearVelocity}{ O{} O{} }{{}_\text{#2}\textbf{v}_{\text{#1}}}
% \DeclareDocumentCommand{\linearVelocityM}{ O{} O{} }{{}_\text{#2}\tilde{\textbf{v}}_{\text{#1}}}
% \DeclareDocumentCommand{\orientation}{ O{} }{\textbf{R}_{\text{#1}}}
% \DeclareDocumentCommand{\orientationDot}{ O{} }{\dot{\textbf{R}}_{\text{#1}}}
% \DeclareDocumentCommand{\homogeneous}{ O{} O{} }{{}_\text{#2}\boldsymbol{\H}_{\text{#1}}}
% \DeclareDocumentCommand{\homogeneousDot}{ O{} }{\dot{\textbf{H}}_{\text{#1}}}
% \DeclareDocumentCommand{\Jacobian}{ O{} O{} }{{}_\text{#2}\boldsymbol{\J}_{\text{#1}}}
% \DeclareDocumentCommand{\inputs}{ O{} O{} }{{}_\text{#2}\boldsymbol{\u}_{\text{#1}}}
% \DeclareDocumentCommand{\inputsM}{ O{} O{} }{{}_\text{#2}\tilde{\boldsymbol{\u}}_{\text{#1}}}
% \DeclareDocumentCommand{\angularVelocity}{ O{} O{} }{{}_\text{#2}\boldsymbol{\omega}_{\text{#1}}}
% \DeclareDocumentCommand{\angularVelocityM}{ O{} O{} }{{}_\text{#2}\tilde{\boldsymbol{\omega}}_{\text{#1}}}
% \DeclareDocumentCommand{\acceleration}{ O{} O{} }{{}_\text{#2}\textbf{a}_{\text{#1}}}
% \DeclareDocumentCommand{\accelerationM}{ O{} O{} }{{}_\text{#2}\tilde{\textbf{a}}_{\text{#1}}}
% \DeclareDocumentCommand{\pE}{ O{} O{} }{\hat{\textbf{p}}_{#1}^{#2}}
% \DeclareDocumentCommand{\pM}{ O{} O{} }{\tilde{\textbf{p}}_{#1}^{#2}}
% \DeclareDocumentCommand{\vE}{ O{} O{} }{\hat{\textbf{v}}_{#1}^{#2}}
% \DeclareDocumentCommand{\wM}{ O{} O{} }{\tilde{\boldsymbol{\omega}}_{#1}^{#2}}
% \DeclareDocumentCommand{\angleTheta}{ O{} O{} }{\boldsymbol{\theta}_{#1}^{#2}}
% \DeclareDocumentCommand{\anglePhi}{ O{} O{} }{\boldsymbol{\phi}_{#1}^{#2}}
% \DeclareDocumentCommand{\encoders}{ O{} O{} }{\boldsymbol{\alpha}_{#1}^{#2}}
% \DeclareDocumentCommand{\encodersM}{ O{} O{} }{\tilde{\boldsymbol{\alpha}}_{#1}^{#2}}
% \DeclareDocumentCommand{\offsets}{ O{} O{} }{\boldsymbol{\epsilon}_{#1}^{#2}}
% \DeclareDocumentCommand{\Cov}{ O{} O{} }{\boldsymbol{\Sigma}_{#1}^{#2}}
% \DeclareDocumentCommand{\Axis}{ O{} O{} }{\textnormal{Axis}_{#1}^{#2}}
% \DeclareDocumentCommand{\using}{ O{} O{} }{\stackrel{\mathmakebox[\widthof{=}]{\text{eq.} (#1)}}{#2} \enspace}
% \DeclareDocumentCommand{\Adjoint}{ O{} }{\mathrm{Ad}_{#1}}
% \DeclareDocumentCommand{\vectorToAlgebra}{ O{} }{\mathscr{L}_\mathfrak{g}\left(#1\right)}
% \DeclareDocumentCommand{\groupError}{ O{} O{} }{\boldsymbol{\eta}_{#1}^{#2}}
% % \DeclareDocumentCommand{\tangentError}{ O{} O{} }{\boldsymbol{\xi}_{#1}^{#2}}
% \DeclareDocumentCommand{\twist}{ O{} O{} }{\boldsymbol{\xi}_{#1}^{#2}}
% \DeclareDocumentCommand{\twistM}{ O{} O{} }{\tilde{\boldsymbol{\xi}}_{#1}^{#2}}

% \DeclareDocumentCommand{\JFK}{ O{} }{\textbf{J}^{\hspace{-0.75mm}\FK}_{#1}}

% \DeclareDocumentCommand{\JFKswitch}{ O{} }{\textbf{J}^{\hspace{-0.75mm}\FKswitch}_{#1}}


% \makeatletter
% \newcommand{\mathleft}{\@fleqntrue\@mathmargin0pt}
% \newcommand{\mathcenter}{\@fleqnfalse}
% \makeatother


==> pre_tex/Conclusion.tex <==
\section{Conclusions}
\label{sec:Conclusions}

We proposed a new method to determine the extrinsic calibration of a LiDAR camera pair. When evaluated against a state-of-the-art baseline, it resulted in, on average, more than a 50\% reduction in LiDAR-to-camera projection error and a 70\% reduction in its variance. These results were established through a round-robin validation study when two targets are used in training, and further buttressed with results for training on four, six, and eight targets. 

Two other benefits of our $L_1$-based method are: (1) it does not require the estimation of a target normal vector from an inherently noisy point cloud; and (2) it also obviates the identification of edge points and their association with specific sides of a target. In combination with lower RMS error and variance, we believe our results may provide an attractive alternative to current target-based methods for extrinsic calibration.  


% We proposed improvements to target-based LiDAR-camera calibration that resulted in, on average,  more than a 50\% reduction in projection error from LiDAR to camera and a 70\% reduction in its variance.We evaluated our proposed method and compared it with a state-of-the-art baseline method in a round-robin validation study when two targets are used in training and presented further data for four, six, and eight targets being used in training. In the validation study, our $L_1$-based method achieved a per corner RMS error, measured in the image plane, on the order of a few pixels, when comparing the projected LiDAR vertices to the image corners. The validation results show our method is repeatable and outperforms the baseline. 

==> pre_tex/ExperimentTables.tex <==
\begin{table*}[]
\caption{Training and validation data. The gray boxes denote the training set and the white boxes contain validation data. The numbers are the RMS errors of the LiDAR vertices projected to the image plane, measured in units of pixels per corner; see \eqref{eq:ErrorMeasure}. For two targets, a complete round-robin study was done. For more targets, the number of combinations became prohibitive. S$_1$ through S$_7$ denote scene (experiment) number. The mean and standard deviation of each row---excluding the training set---are given in the last two columns.}
\label{tab:cross-v1}
\medskip
\centering
\resizebox{2\columnwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\rowcolor[HTML]{EFEFEF} 
Training\textbackslash{}Validation & Method & \# Tag & S1 & S2 & S3 & S4 & S5 & S6 & S7 & mean & std \\ \hline
\cellcolor[HTML]{EFEFEF} & RN & 2 & \cellcolor[HTML]{C0C0C0}{\color[HTML]{333333} 2.6618} & 8.7363 & 4.4712 & 7.3851 & 4.1269 & 7.1884 & 11.9767 & 7.3141 & 2.8991 \\ \cline{2-12} 
\multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}S1} & GL$_1$ & 2 & \cellcolor[HTML]{C0C0C0}0.7728 & \textbf{2.3303} & \textbf{2.3230} & \textbf{1.6318} & \textbf{1.3694} & \textbf{1.9637} & \textbf{2.7427} & \textbf{2.0602} & \textbf{0.5055} \\ \hline
\cellcolor[HTML]{EFEFEF} & RN & 2 & 3.3213 & \cellcolor[HTML]{C0C0C0}7.6645 & 4.9169 & 5.2951 & 4.0811 & 4.4345 & 7.7397 & 4.9648 & 1.5215 \\ \cline{2-12} 
\multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}S2} & GL$_1$ & 2 & \textbf{2.1368} & \cellcolor[HTML]{C0C0C0}1.5181 & \textbf{3.2027} & \textbf{3.2589} & \textbf{2.4480} & \textbf{4.1563} & \textbf{4.4254} & \textbf{3.2713} & \textbf{0.9039} \\ \hline
\cellcolor[HTML]{EFEFEF} & RN & 2 & 4.9909 & 9.5620 & \cellcolor[HTML]{C0C0C0}3.6271 & 8.7533 & 4.6421 & 10.1308 & 15.7764 & 8.9759 & 4.0654 \\ \cline{2-12} 
\multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}S3} & GL$_1$ & 2 & \textbf{4.6720} & \textbf{5.9350} & \cellcolor[HTML]{C0C0C0}1.8469 & \textbf{6.9331} & \textbf{4.4352} & \textbf{8.9493} & \textbf{15.3862} & \textbf{7.7185} & \textbf{4.1029} \\ \hline
\cellcolor[HTML]{EFEFEF} & RN & 2 & 21.2271 & 22.1641 & 17.5779 & \cellcolor[HTML]{C0C0C0}2.9452 & 15.9909 & 8.8797 & 15.3636 & 16.8672 & 4.7833 \\ \cline{2-12} 
\multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}S4} & GL$_1$ & 2 & \textbf{4.3681} & \textbf{4.7176} & \textbf{4.4804} & \cellcolor[HTML]{C0C0C0}0.4986 & \textbf{3.9004} & \textbf{3.3891} & \textbf{3.7440} & \textbf{4.0999} & \textbf{0.5040} \\ \hline
\cellcolor[HTML]{EFEFEF} & RN & 2 & 3.4621 & 8.3131 & 4.8500 & 7.6217 & \cellcolor[HTML]{C0C0C0}3.5197 & 7.4838 & 12.4364 & 7.3612 & 3.1066 \\ \cline{2-12} 
\multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}S5} & GL$_1$ & 2 & \textbf{2.0590} & \textbf{2.9541} & \textbf{3.0224} & \textbf{3.5483} & \cellcolor[HTML]{C0C0C0}0.7392 & \textbf{3.1386} & \textbf{6.0885} & \textbf{3.4685} & \textbf{1.3733} \\ \hline
\cellcolor[HTML]{EFEFEF} & RN & 2 & 29.4400 & 27.5404 & 27.9955 & 9.7005 & 20.6511 & \cellcolor[HTML]{C0C0C0}1.4253 & 9.5050 & 20.8054 & 9.1941 \\ \cline{2-12} 
\multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}S6} & GL$_1$ & 2 & \textbf{5.1207} & \textbf{5.0574} & \textbf{5.3537} & \textbf{2.0539} & \textbf{4.1739} & \cellcolor[HTML]{C0C0C0}1.0012 & \textbf{2.4194} & \textbf{4.0298} & \textbf{1.4503} \\ \hline
\cellcolor[HTML]{EFEFEF} & RN & 2 & 7.7991 & 9.9647 & 7.6857 & 4.1640 & 6.1619 & 2.3398 & \cellcolor[HTML]{C0C0C0}2.3708 & 6.3525 & 2.7512 \\ \cline{2-12} 
\multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}S7} & GL$_1$ & 2 & \textbf{2.1563} & \textbf{2.7837} & \textbf{3.1058} & \textbf{1.3234} & \textbf{2.4537} & \textbf{2.0838} & \cellcolor[HTML]{C0C0C0}1.5389 & \textbf{2.3178} & \textbf{0.6207} \\ \hhline{|=|=|=|=|=|=|=|=|=|=|=|=|}
\cellcolor[HTML]{EFEFEF} & RN & 4 & 6.9426 & 9.6281 & 6.9136 & 3.9650 & 5.6420 & \cellcolor[HTML]{C0C0C0}2.2399 & \cellcolor[HTML]{C0C0C0}2.2399 & 6.6183 & 2.0764 \\ \cline{2-12} 
\multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}S6-S7} & GL$_1$ & 4 & \textbf{2.2409} & \textbf{2.5607} & \textbf{2.9773} & \textbf{1.8215} & \textbf{2.1995} & \cellcolor[HTML]{C0C0C0}0.3417 & \cellcolor[HTML]{C0C0C0}0.3417 & \textbf{2.3600} & \textbf{0.4334} \\ \hline
\cellcolor[HTML]{EFEFEF} & RN & 4 & 4.2476 & 8.5054 & 4.6712 & \cellcolor[HTML]{C0C0C0}2.8686 & 4.3311 & \cellcolor[HTML]{C0C0C0}{\color[HTML]{333333} 2.8686} & 2.8748 & 4.9260 & 2.1153 \\ \cline{2-12} 
\multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}S4-S6} & GL$_1$ & 4 & \textbf{1.0746} & \textbf{1.8871} & \textbf{2.3619} & \cellcolor[HTML]{C0C0C0}0.2341 & \textbf{1.5350} & \cellcolor[HTML]{C0C0C0}{\color[HTML]{333333} 0.2341} & \textbf{2.6191} & \textbf{1.8955} & \textbf{0.6215} \\ \hline
\cellcolor[HTML]{EFEFEF} & RN & 4 & 2.9309 & 8.0801 & 4.1196 & 3.4985 & \cellcolor[HTML]{C0C0C0}3.1519 & \cellcolor[HTML]{C0C0C0}3.1519 & 3.2204 & 4.3699 & 2.1201 \\ \cline{2-12} 
\multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}S5-S6} & GL$_1$ & 4 & \textbf{1.1541} & \textbf{2.1026} & \textbf{2.5017} & \textbf{1.4267} & \cellcolor[HTML]{C0C0C0}0.3291 & \cellcolor[HTML]{C0C0C0}0.3291 & \textbf{2.5693} & \textbf{1.9509} & \textbf{0.6361} \\ \hline
\cellcolor[HTML]{EFEFEF} & RN & 4 & 3.1991 & \cellcolor[HTML]{C0C0C0}{\color[HTML]{333333} 6.0812} & 4.7311 & 5.4558 & \cellcolor[HTML]{C0C0C0}{\color[HTML]{333333} 6.0812} & 4.8344 & 8.6576 & 5.3756 & 2.0139 \\ \cline{2-12} 
\multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}S2-S5} & GL$_1$ & 4 & \textbf{0.9538} & \cellcolor[HTML]{C0C0C0}{\color[HTML]{333333} 0.4803} & \textbf{2.3810} & \textbf{1.4556} & \cellcolor[HTML]{C0C0C0}{\color[HTML]{333333} 0.4803} & \textbf{1.1592} & \textbf{2.5277} & \textbf{1.6955} & \textbf{0.7172} \\ \hline
\cellcolor[HTML]{EFEFEF} & RN & 4 & 2.8820 & \cellcolor[HTML]{C0C0C0}6.2167 & \cellcolor[HTML]{C0C0C0}6.2167 & 4.4672 & 3.9536 & 3.7802 & 6.2324 & 4.2631 & 1.2406 \\ \cline{2-12} 
\multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}S2-S3} & GL$_1$ & 4 & \textbf{1.0896} & \cellcolor[HTML]{C0C0C0}0.4826 & \cellcolor[HTML]{C0C0C0}0.4826 & \textbf{1.5349} & \textbf{1.5938} & \textbf{1.5597} & \textbf{2.7543} & \textbf{1.7065} & \textbf{0.6209} \\ \hline
\cellcolor[HTML]{EFEFEF} & RN & 4 & \cellcolor[HTML]{C0C0C0}2.8595 & 8.2471 & 4.3297 & 3.7712 & 4.1023 & 2.4679 & \cellcolor[HTML]{C0C0C0}2.8595 & 4.5836 & 2.1710 \\ \cline{2-12} 
\multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}S1-S7} & GL$_1$ & 4 & \cellcolor[HTML]{C0C0C0}1.3542 & \textbf{1.9973} & \textbf{2.3987} & \textbf{1.5926} & \textbf{1.4978} & \textbf{1.6130} & \cellcolor[HTML]{C0C0C0}1.3542 & \textbf{1.8199} & \textbf{0.3757} \\ \hline
\cellcolor[HTML]{EFEFEF} & RN & 4 & \cellcolor[HTML]{C0C0C0}2.5633 & 8.0573 & 4.1762 & 3.6859 & 3.8973 & \cellcolor[HTML]{C0C0C0}2.5633 & 3.2569 & 4.6147 & 1.9535 \\ \cline{2-12} 
\multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}S1-S6} & GL$_1$ & 4 & \cellcolor[HTML]{C0C0C0}0.9753 & \textbf{1.9154} & \textbf{2.3361} & \textbf{1.2906} & \textbf{1.2827} & \cellcolor[HTML]{C0C0C0}0.9753 & \textbf{2.3205} & \textbf{1.8291} & \textbf{0.5231} \\ \hhline{|=|=|=|=|=|=|=|=|=|=|=|=|}
\cellcolor[HTML]{EFEFEF} & RN & 6 & 2.9824 & 8.0943 & 4.1273 & \cellcolor[HTML]{C0C0C0}3.2821 & \cellcolor[HTML]{C0C0C0}3.2821 & \cellcolor[HTML]{C0C0C0}3.2821 & 3.0841 & 4.5720 & 2.4045 \\ \cline{2-12} 
\multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}S4-S5-S6} & GL$_1$ & 6 & \textbf{0.9713} & \textbf{1.9887} & \textbf{2.4395} & \cellcolor[HTML]{C0C0C0}0.3288 & \cellcolor[HTML]{C0C0C0}0.3288 & \cellcolor[HTML]{C0C0C0}0.3288 & \textbf{2.4369} & \textbf{1.9591} & \textbf{0.6918} \\ \hline
\cellcolor[HTML]{EFEFEF} & RN & 6 & 2.7816 & \cellcolor[HTML]{C0C0C0}5.5382 & \cellcolor[HTML]{C0C0C0}5.5382 & 4.5817 & \cellcolor[HTML]{C0C0C0}5.5382 & 3.8262 & 6.6229 & 4.4531 & 1.6239 \\ \cline{2-12} 
\multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}S2-S3-S5} & GL$_1$ & 6 & \textbf{1.0022} & \cellcolor[HTML]{C0C0C0}0.4712 & \cellcolor[HTML]{C0C0C0}0.4712 & \textbf{1.4755} & \cellcolor[HTML]{C0C0C0}0.4712 & \textbf{1.1722} & \textbf{2.7791} & \textbf{1.6073} & \textbf{0.8054} \\ \hline
\cellcolor[HTML]{EFEFEF} & RN & 6 & \cellcolor[HTML]{C0C0C0}3.3906 & 8.1677 & \cellcolor[HTML]{C0C0C0}3.3906 & 3.6688 & 3.9558 & 2.2913 & \cellcolor[HTML]{C0C0C0}3.3906 & 4.5209 & 2.5374 \\ \cline{2-12} 
\multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}S1-S3-S7} & GL$_1$ & 6 & \cellcolor[HTML]{C0C0C0}1.7666 & \textbf{1.9994} & \cellcolor[HTML]{C0C0C0}1.7666 & \textbf{1.5854} & \textbf{1.4754} & \textbf{1.5124} & \cellcolor[HTML]{C0C0C0}1.7666 & \textbf{1.6432} & \textbf{0.2419} \\ \hline
\cellcolor[HTML]{EFEFEF} & RN & 6 & 2.9428 & \cellcolor[HTML]{C0C0C0}5.5357 & \cellcolor[HTML]{C0C0C0}5.5357 & \cellcolor[HTML]{C0C0C0}5.5357 & 3.8913 & 2.4828 & 3.7673 & 3.2711 & 0.6733 \\ \cline{2-12} 
\multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}S2-S3-S4} & GL$_1$ & 6 & \textbf{0.9523} & \cellcolor[HTML]{C0C0C0}1.8195 & \cellcolor[HTML]{C0C0C0}1.8195 & \cellcolor[HTML]{C0C0C0}1.8195 & \textbf{1.5275} & \textbf{1.3631} & \textbf{2.4347} & \textbf{1.5694} & \textbf{0.6255} \\ \hline
\cellcolor[HTML]{EFEFEF} & RN & 6 & \cellcolor[HTML]{C0C0C0}5.3281 & \cellcolor[HTML]{C0C0C0}5.3281 & \cellcolor[HTML]{C0C0C0}5.3281 & 4.5086 & 3.8577 & 3.7165 & 6.4413 & 4.6310 & 1.2552 \\ \cline{2-12} 
\multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}S1-S2-S3} & GL$_1$ & 6 & \cellcolor[HTML]{C0C0C0}1.7755 & \cellcolor[HTML]{C0C0C0}1.7755 & \cellcolor[HTML]{C0C0C0}1.7755 & \textbf{1.3698} & \textbf{1.4807} & \textbf{1.3422} & \textbf{2.3156} & \textbf{1.6271} & \textbf{0.4629} \\ \hline
\cellcolor[HTML]{EFEFEF} & RN & 6 & 3.2743 & 8.2067 & 4.2628 & 3.5584 & \cellcolor[HTML]{C0C0C0}3.0628 & \cellcolor[HTML]{C0C0C0}3.0628 & \cellcolor[HTML]{C0C0C0}3.0628 & 4.8256 & 2.2921 \\ \cline{2-12} 
\multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}S5-S6-S7} & GL$_1$ & 6 & \textbf{0.9594} & \textbf{2.0149} & \textbf{2.3877} & \textbf{1.3754} & \cellcolor[HTML]{C0C0C0}1.4905 & \cellcolor[HTML]{C0C0C0}1.4905 & \cellcolor[HTML]{C0C0C0}1.4905 & \textbf{1.6843} & \textbf{0.6390} \\ \hhline{|=|=|=|=|=|=|=|=|=|=|=|=|}
\cellcolor[HTML]{EFEFEF} & RN & 8 & \cellcolor[HTML]{C0C0C0}3.5316 & 8.1362 & \cellcolor[HTML]{C0C0C0}3.5316 & 3.4616 & \cellcolor[HTML]{C0C0C0}3.5316 & 2.2642 & \cellcolor[HTML]{C0C0C0}3.5316 & 4.6207 & 3.1029 \\ \cline{2-12} 
\multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}S1-S3-S5-S7} & GL$_1$ & 8 & \cellcolor[HTML]{C0C0C0}1.6904 & \textbf{1.9886} & \cellcolor[HTML]{C0C0C0}1.6904 & \textbf{1.4743} & \cellcolor[HTML]{C0C0C0}1.6904 & \textbf{1.4136} & \cellcolor[HTML]{C0C0C0}1.6904 & \textbf{1.6255} & \textbf{0.3159} \\ \hline
\cellcolor[HTML]{EFEFEF} & RN & 8 & \cellcolor[HTML]{C0C0C0}4.9240 & \cellcolor[HTML]{C0C0C0}4.9240 & 4.2049 & 3.6159 & \cellcolor[HTML]{C0C0C0}4.9240 & 2.2928 & \cellcolor[HTML]{C0C0C0}4.9240 & 3.3712 & 0.9793 \\ \cline{2-12} 
\multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}S1-S2-S5-S7} & GL$_1$ & 8 & \cellcolor[HTML]{C0C0C0}1.5269 & \cellcolor[HTML]{C0C0C0}1.5269 & \textbf{2.4070} & \textbf{1.4788} & \cellcolor[HTML]{C0C0C0}1.5269 & \textbf{1.4650} & \cellcolor[HTML]{C0C0C0}1.5269 & \textbf{1.7836} & \textbf{0.5399} \\ \hline
\cellcolor[HTML]{EFEFEF} & RN & 8 & \cellcolor[HTML]{C0C0C0}3.6113 & 8.0593 & \cellcolor[HTML]{C0C0C0}3.6113 & \cellcolor[HTML]{C0C0C0}3.6113 & \cellcolor[HTML]{C0C0C0}3.6113 & 2.4532 & 3.8397 & 4.7841 & 2.9199 \\ \cline{2-12} 
\multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}S1-S3-S4-S5} & GL$_1$ & 8 & \cellcolor[HTML]{C0C0C0}1.4986 & \textbf{2.0563} & \cellcolor[HTML]{C0C0C0}1.4986 & \cellcolor[HTML]{C0C0C0}1.4986 & \cellcolor[HTML]{C0C0C0}1.4986 & \textbf{1.2256} & \textbf{2.6797} & \textbf{1.9872} & \textbf{0.7295} \\ \hline
\cellcolor[HTML]{EFEFEF} & RN & 8 & 3.0803 & \cellcolor[HTML]{C0C0C0}5.0057 & 4.1893 & \cellcolor[HTML]{C0C0C0}5.0057 & \cellcolor[HTML]{C0C0C0}5.0057 & 2.3307 & \cellcolor[HTML]{C0C0C0}5.0057 & 3.2001 & 0.9351 \\ \cline{2-12} 
\multirow{-2}{*}{\cellcolor[HTML]{EFEFEF}S2-S4-S5-S7} & GL$_1$ & 8 & \textbf{0.9530} & \cellcolor[HTML]{C0C0C0}1.5921 & \textbf{2.4280} & \cellcolor[HTML]{C0C0C0}1.5921 & \cellcolor[HTML]{C0C0C0}1.5921 & \textbf{1.4865} & \cellcolor[HTML]{C0C0C0}1.5921 & \textbf{1.6225} & \textbf{0.7469} \\ \hline
\end{tabular}
}
\end{table*}

\begin{table}[]
\caption{A summary of validation data in Table \ref{tab:cross-v1}. This table compares mean and standard deviation for baseline and our approach as a function of the number of targets used in training. Units are pixel per corner.}
\label{tab:SummaryTable}
\centering
\resizebox{1\columnwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\rowcolor[HTML]{EFEFEF} 
 & \# Tag & 2 & 4 & 6 & 8 \\ \hline
\cellcolor[HTML]{EFEFEF}RN & mean & 10.3773 & 4.9645 & 4.3789 & 3.9940 \\ \hline
\cellcolor[HTML]{EFEFEF}GL$_1$ & mean & \textbf{3.8523} & \textbf{1.8939} & \textbf{1.6817} & \textbf{1.7547} \\ \hline
\cellcolor[HTML]{EFEFEF}RN & std & 7.0887 & 1.9532 & 1.7771 & 2.0467 \\ \hline
\cellcolor[HTML]{EFEFEF}GL$_1$ & std & \textbf{2.4155} & \textbf{0.5609} & \textbf{0.5516} & \textbf{0.5419} \\ \hline
\end{tabular}
}
\end{table}

% \begin{table*}[]
% \caption{Round-robin validation study. The gray box denotes the training set and the others are used as validation data. The numbers are the RMS errors of the LiDAR vertices projected to the image plane in pixels per corner; see \eqref{eq:ErrorMeasure}.}
% \label{tab:cross-v1}
% \medskip
% \centering
% \resizebox{1.65\columnwidth}{!}{%
% \begin{tabular}{ccccccccclll|l|l|l|l|l|}
% \cline{13-17}
% \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} &  &  &  &  & \multicolumn{2}{l|}{refinement or not} & \multicolumn{2}{l|}{consistency or not} \\ \cline{1-11} \cline{13-17} 
% \multicolumn{1}{|c|}{\cellcolor[HTML]{EFEFEF}Training\textbackslash{}Validation} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}Method} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}S1} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}S2} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}S3} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}S4} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}S5} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}S6} & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}S7} & \multicolumn{1}{l|}{mean} & \multicolumn{1}{l|}{std} &  &  & \begin{tabular}[c]{@{}l@{}}SNR-SR\\ (consistency)\end{tabular} & \begin{tabular}[c]{@{}l@{}}SNRNT-SRNT\\ (non-consistency)\end{tabular} & \begin{tabular}[c]{@{}l@{}}SNR-SNRNT\\ (SNR)\end{tabular} & \begin{tabular}[c]{@{}l@{}}SR-SRNT\\ (SR)\end{tabular} \\ \cline{1-11} \cline{13-17} 
% \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}NSNR-itsOwn} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}{\color[HTML]{333333} 2.6618}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}8.0768} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}4.0389} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}\textbf{5.0324}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}3.7466} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}\textbf{4.5581}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}\textbf{7.8952}} & \multicolumn{1}{l|}{\textbf{5.5580}} & \multicolumn{1}{l|}{\textbf{1.9324}} &  & mean & 0.8300 & 0.5838 & 1.9346 & 1.6822 \\ \cline{2-11} \cline{13-17} 
% \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}GN-itsOwn} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}2.3302} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}\textbf{7.1979}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}\textbf{2.8754}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}7.6470} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}\textbf{3.6220}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}7.8972} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}14.0780} & \multicolumn{1}{l|}{7.2196} & \multicolumn{1}{l|}{3.9873} &  & std & 0.8111 & 0.5187 & -27.1719 & -27.3860 \\ \cline{2-11} \cline{13-17} 
% \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}SNR-Top} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}0.7728} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}2.3303} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}2.3230} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}1.6318} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}1.3694} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}1.9637} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}2.7427} & \multicolumn{1}{l|}{2.0602} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFCCC9}0.5055} &  &  &  &  &  &  \\ \cline{2-11} \cline{13-17} 
% \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}SR-Top-itsOwn} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}0.2977} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}\textbf{2.3242}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}\textbf{2.3060}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}\textbf{1.6039}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}\textbf{1.3652}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}\textbf{1.9476}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}\textbf{2.7119}} & \multicolumn{1}{l|}{\textbf{2.0431}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFCCC9}\textbf{0.5014}} &  &  &  &  &  &  \\ \cline{2-11} \cline{13-17} 
% \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}SNR-nonTop} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}0.8129} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}2.2066} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}2.3726} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}1.3139} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}1.3741} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}1.7232} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}3.1361} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFCCC9}2.0211} & \multicolumn{1}{l|}{0.6941} &  &  &  &  &  &  \\ \cline{2-11} \cline{13-17} 
% \multicolumn{1}{|c|}{\multirow{-6}{*}{\begin{tabular}[c]{@{}c@{}}S1\\ (4)\end{tabular}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}SR-nonTop-itsOwn} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}0.2953} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}\textbf{2.1904}} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}\textbf{2.3715}} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}\textbf{1.2983}} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}\textbf{1.3722}} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}\textbf{1.7098}} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}\textbf{3.1134}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFCCC9}\textbf{2.0093}} & \multicolumn{1}{l|}{\textbf{0.6905}} &  &  &  &  &  &  \\ \cline{1-11} \cline{13-17} 
% \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}NSNR-itsOwn} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}\textbf{3.3213}} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}7.6645} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}\textbf{4.9169}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}\textbf{5.2951}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}\textbf{4.0811}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}\textbf{4.4345}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}\textbf{7.7397}} & \multicolumn{1}{l|}{\textbf{4.9648}} & \multicolumn{1}{l|}{\textbf{1.5215}} &  & mean & 4.9399 & 5.0748 & 0.6740 & 0.8170 \\ \cline{2-11} \cline{13-17} 
% \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}GN-itsOwn} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}8.6213} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}3.7071} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}9.9023} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}15.3850} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}4.8692} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}15.3349} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}23.7915} & \multicolumn{1}{l|}{12.9840} & \multicolumn{1}{l|}{6.6704} &  & std & 7.3902 & 8.0997 & 0.1551 & 0.9284 \\ \cline{2-11} \cline{13-17} 
% \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}SNR-Top} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}2.1368} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}1.5181} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}3.2027} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}3.2589} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}2.4480} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}4.1563} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}4.4254} & \multicolumn{1}{l|}{3.2713} & \multicolumn{1}{l|}{0.9039} &  &  &  &  &  &  \\ \cline{2-11} \cline{13-17} 
% \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}SR-Top-itsOwn} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}\textbf{2.0335}} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}0.5069} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}\textbf{3.0834}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}\textbf{3.0728}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}\textbf{2.3708}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}\textbf{3.9191}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}\textbf{4.1786}} & \multicolumn{1}{l|}{\textbf{3.1097}} & \multicolumn{1}{l|}{\textbf{0.8371}} &  &  &  &  &  &  \\ \cline{2-11} \cline{13-17} 
% \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}SNR-nonTop} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}2.1089} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}1.4482} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}3.1357} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}3.1551} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}2.5363} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}4.0402} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}4.5205} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFCCC9}3.2494} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFCCC9}0.9025} &  &  &  &  &  &  \\ \cline{2-11} \cline{13-17} 
% \multicolumn{1}{|c|}{\multirow{-6}{*}{\begin{tabular}[c]{@{}c@{}}S2\\ (5)\end{tabular}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}SR-nonTop-itsOwn} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}\textbf{1.9949}} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}0.5122} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}\textbf{3.0584}} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}\textbf{2.9646}} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}\textbf{2.4562}} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}\textbf{3.7865}} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}\textbf{4.2464}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFCCC9}\textbf{3.0845}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFCCC9}\textbf{0.8294}} &  &  &  &  &  &  \\ \cline{1-11} \cline{13-17} 
% \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}NSNR-itsOwn} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}4.9909} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}9.5620} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}3.6271} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}8.7533} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}4.6421} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}10.1308} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}\textbf{15.7764}} & \multicolumn{1}{l|}{8.9759} & \multicolumn{1}{l|}{\textbf{4.0654}} &  & mean & 10.8104 & 10.5381 & 2.0817 & 1.7711 \\ \cline{2-11} \cline{13-17} 
% \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}GN-itsOwn} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}\textbf{4.1119}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}\textbf{8.1581}} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}1.6474} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}\textbf{8.2761}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}\textbf{3.6660}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}\textbf{9.7009}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}17.2210} & \multicolumn{1}{l|}{\textbf{8.5223}} & \multicolumn{1}{l|}{4.9048} &  & std & 12.0403 & 13.2644 & 6.5854 & 8.0897 \\ \cline{2-11} \cline{13-17} 
% \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}SNR-Top} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}4.6720} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}5.9350} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}1.8469} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}6.9331} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}4.4352} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}8.9493} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}15.3862} & \multicolumn{1}{l|}{7.7185} & \multicolumn{1}{l|}{4.1029} &  &  &  &  &  &  \\ \cline{2-11} \cline{13-17} 
% \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}SR-Top-itsOwn} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}\textbf{4.2051}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}\textbf{5.4023}} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}0.4530} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}\textbf{6.1449}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}\textbf{3.9981}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}\textbf{7.8992}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}\textbf{13.6549}} & \multicolumn{1}{l|}{\textbf{6.8841}} & \multicolumn{1}{l|}{\textbf{3.6089}} &  &  &  &  &  &  \\ \cline{2-11} \cline{13-17} 
% \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}SNR-nonTop} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}4.7712} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}5.8651} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}1.8748} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}6.5835} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}4.4860} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}8.9523} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}14.7083} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFCCC9}7.5611} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFCCC9}3.8494} &  &  &  &  &  &  \\ \cline{2-11} \cline{13-17} 
% \multicolumn{1}{|c|}{\multirow{-6}{*}{\begin{tabular}[c]{@{}c@{}}S3\\ (6)\end{tabular}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}SR-nonTop-itsOwn} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}\textbf{4.3131}} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}\textbf{5.4749}} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}0.4530} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}\textbf{5.8237}} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}\textbf{4.0666}} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}\textbf{7.9359}} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}\textbf{12.9718}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFCCC9}\textbf{6.7643}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFCCC9}\textbf{3.3388}} &  &  &  &  &  &  \\ \cline{1-11} \cline{13-17} 
% \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}NSNR-itsOwn} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}\textbf{21.2271}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}\textbf{22.1641}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}\textbf{17.5779}} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}2.9452} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}\textbf{15.9909}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}\textbf{8.8797}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}\textbf{15.3636}} & \multicolumn{1}{l|}{\textbf{16.8672}} & \multicolumn{1}{l|}{\textbf{4.7833}} &  & mean & 0.6610 & 0.3646 & 4.5200 & 4.2090 \\ \cline{2-11} \cline{13-17} 
% \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}GN-itsOwn} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}34.4454} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}33.6574} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}28.1258} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}1.2691} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}25.2418} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}12.8025} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}23.7335} & \multicolumn{1}{l|}{26.3344} & \multicolumn{1}{l|}{7.9208} &  & std & -3.4921 & -17.5132 & 6.2171 & -6.4562 \\ \cline{2-11} \cline{13-17} 
% \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}SNR-Top} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}4.3681} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}4.7176} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}\textbf{4.4804}} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}0.4986} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}3.9004} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}3.3891} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}3.7440} & \multicolumn{1}{l|}{4.0999} & \multicolumn{1}{l|}{\textbf{0.5040}} &  &  &  &  &  &  \\ \cline{2-11} \cline{13-17} 
% \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}SR-Top-itsOwn} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}\textbf{4.3110}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}\textbf{4.6949}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}4.5287} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}0.3105} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}\textbf{3.8585}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}\textbf{3.3552}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}\textbf{3.6882}} & \multicolumn{1}{l|}{\textbf{4.0728}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFCCC9}0.5216} &  &  &  &  &  &  \\ \cline{2-11} \cline{13-17} 
% \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}SNR-nonTop} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}4.1023} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}\textbf{4.4895}} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}4.0994} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}0.5306} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}3.7152} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}3.0948} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}4.0345} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFCCC9}3.9226} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFCCC9}\textbf{0.4745}} &  &  &  &  &  &  \\ \cline{2-11} \cline{13-17} 
% \multicolumn{1}{|c|}{\multirow{-6}{*}{\begin{tabular}[c]{@{}c@{}}S4\\ (8)\end{tabular}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}SR-nonTop-itsOwn} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}\textbf{3.9995}} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}4.7599} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}\textbf{4.0345}} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}0.3446} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}\textbf{3.6459}} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}\textbf{3.0518}} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}\textbf{3.9581}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFCCC9}\textbf{3.9083}} & \multicolumn{1}{l|}{0.5576} &  &  &  &  &  &  \\ \cline{1-11} \cline{13-17} 
% \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}NSNR-itsOwn} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}\textbf{3.4621}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}8.3131} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}\textbf{4.8500}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}\textbf{7.6217}} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}3.5197} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}\textbf{7.4838}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}\textbf{12.4364}} & \multicolumn{1}{l|}{\textbf{7.3612}} & \multicolumn{1}{l|}{\textbf{3.1066}} &  & mean & -0.6775 & -0.3371 & -14.0290 & -13.7373 \\ \cline{2-11} \cline{13-17} 
% \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}GN-itsOwn} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}4.9944} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}\textbf{6.1094}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}6.6855} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}11.6415} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}1.6646} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}11.9789} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}22.1886} & \multicolumn{1}{l|}{10.5997} & \multicolumn{1}{l|}{6.3905} &  & std & -1.0194 & -1.5162 & -24.2860 & -24.6565 \\ \cline{2-11} \cline{13-17} 
% \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}SNR-Top} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}\textbf{2.0590}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}\textbf{2.9541}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}\textbf{3.0224}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}\textbf{3.5483}} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}0.7392} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}\textbf{3.1386}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}\textbf{6.0885}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFCCC9}\textbf{3.4685}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFCCC9}\textbf{1.3733}} &  &  &  &  &  &  \\ \cline{2-11} \cline{13-17} 
% \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}SR-Top-itsOwn} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}2.0750} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}2.9553} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}3.0376} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}3.5758} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}0.4453} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}3.1688} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}6.1396} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFCCC9}3.4920} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFCCC9}1.3873} &  &  &  &  &  &  \\ \cline{2-11} \cline{13-17} 
% \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}SNR-nonTop} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}\textbf{2.1928}} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}3.1625} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}\textbf{3.2833}} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}\textbf{4.1153}} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}0.7215} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}\textbf{3.9945}} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}\textbf{7.4586}} & \multicolumn{1}{l|}{\textbf{4.0345}} & \multicolumn{1}{l|}{\textbf{1.8138}} &  &  &  &  &  &  \\ \cline{2-11} \cline{13-17} 
% \multicolumn{1}{|c|}{\multirow{-6}{*}{\begin{tabular}[c]{@{}c@{}}S5\\ (9)\end{tabular}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}SR-nonTop-itsOwn} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}2.2120} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}\textbf{3.0767}} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}3.2870} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}4.1560} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}0.4463} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}4.0383} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}7.5189} & \multicolumn{1}{l|}{4.0481} & \multicolumn{1}{l|}{1.8413} &  &  &  &  &  &  \\ \cline{1-11} \cline{13-17} 
% \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}NSNR-itsOwn} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}\textbf{29.4400}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}\textbf{27.5404}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}\textbf{27.9955}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}\textbf{9.7005}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}\textbf{20.6511}} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}1.4253} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}\textbf{9.5050}} & \multicolumn{1}{l|}{\textbf{20.8054}} & \multicolumn{1}{l|}{\textbf{9.1941}} &  & mean & 24.6439 & 22.2852 & -26.2684 & -28.5062 \\ \cline{2-11} \cline{13-17} 
% \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}GN-itsOwn} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}32.4146} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}29.5532} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}31.6264} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}11.0496} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}23.3259} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}1.1228} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}10.9628} & \multicolumn{1}{l|}{23.1554} & \multicolumn{1}{l|}{9.9364} &  & std & 36.3373 & 28.3887 & -23.6564 & -32.1303 \\ \cline{2-11} \cline{13-17} 
% \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}SNR-Top} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}5.1207} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}5.0574} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}5.3537} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}2.0539} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}4.1739} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}1.0012} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}2.4194} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFCCC9}4.0298} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFCCC9}1.4503} &  &  &  &  &  &  \\ \cline{2-11} \cline{13-17} 
% \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}SR-Top-itsOwn} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}\textbf{3.5224}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}\textbf{3.7322}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}\textbf{3.9811}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}\textbf{1.5804}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}\textbf{3.0932}} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}0.1384} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}\textbf{2.3111}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFCCC9}\textbf{3.0367}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFCCC9}\textbf{0.9233}} &  &  &  &  &  &  \\ \cline{2-11} \cline{13-17} 
% \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}SNR-nonTop} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}7.1933} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}6.7593} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}7.1077} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}2.9520} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}5.4044} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}0.9175} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}3.3760} & \multicolumn{1}{l|}{5.4655} & \multicolumn{1}{l|}{1.8997} &  &  &  &  &  &  \\ \cline{2-11} \cline{13-17} 
% \multicolumn{1}{|c|}{\multirow{-6}{*}{\begin{tabular}[c]{@{}c@{}}S6\\ (10)\end{tabular}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}SR-nonTop-itsOwn} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}\textbf{5.2998}} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}\textbf{5.4520}} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}\textbf{5.3931}} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}\textbf{2.3948}} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}\textbf{4.0854}} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}0.1239} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}\textbf{2.8602}} & \multicolumn{1}{l|}{\textbf{4.2475}} & \multicolumn{1}{l|}{\textbf{1.3604}} &  &  &  &  &  &  \\ \cline{1-11} \cline{13-17} 
% \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}NSNR-itsOwn} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}\textbf{7.7991}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}9.9647} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}\textbf{7.6857}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}4.1640} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}\textbf{6.1619}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}2.3398} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}2.3708} & \multicolumn{1}{l|}{\textbf{6.3525}} & \multicolumn{1}{l|}{\textbf{2.7512}} &  & mean & 2.6706 & -14.7660 & 14.4254 & -2.9595 \\ \cline{2-11} \cline{13-17} 
% \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}GN-itsOwn} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}9.1437} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}\textbf{8.6058}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}8.9375} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}\textbf{2.6230}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}7.1148} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFC7}\textbf{1.7931}} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}4.2007} & \multicolumn{1}{l|}{6.3697} & \multicolumn{1}{l|}{3.3114} &  & std & 4.5271 & -0.9982 & 58.8687 & 50.1774 \\ \cline{2-11} \cline{13-17} 
% \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}SNR-Top} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}\textbf{2.1563}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}2.7837} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}3.1058} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}\textbf{1.3234}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}2.4537} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}2.0838} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}1.5389} & \multicolumn{1}{l|}{2.3178} & \multicolumn{1}{l|}{0.6207} &  &  &  &  &  &  \\ \cline{2-11} \cline{13-17} 
% \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}SR-Top-itsOwn} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}2.1666} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}\textbf{2.6927}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}\textbf{3.0928}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}1.4715} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}\textbf{2.3399}} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFCE93}\textbf{1.7720}} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}0.4578} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFCCC9}\textbf{2.2559}} & \multicolumn{1}{l|}{\textbf{0.5926}} &  &  &  &  &  &  \\ \cline{2-11} \cline{13-17} 
% \multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}SNR-nonTop} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}\textbf{1.5284}} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}\textbf{2.1522}} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}\textbf{2.6341}} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}\textbf{2.1723}} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}\textbf{1.9644}} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}\textbf{1.7023}} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}1.6124} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFCCC9}\textbf{2.0256}} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFCCC9}\textbf{0.3907}} &  &  &  &  &  &  \\ \cline{2-11} \cline{13-17} 
% \multicolumn{1}{|c|}{\multirow{-6}{*}{\begin{tabular}[c]{@{}c@{}}S7\\ (11)\end{tabular}}} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}SR-nonTop-itsOwn} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}1.9127} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}2.3630} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}2.9026} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}2.5708} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}2.3356} & \multicolumn{1}{c|}{\cellcolor[HTML]{9AFF99}1.8636} & \multicolumn{1}{c|}{\cellcolor[HTML]{C0C0C0}0.4642} & \multicolumn{1}{l|}{2.3247} & \multicolumn{1}{l|}{\cellcolor[HTML]{FFCCC9}0.3946} &  &  &  &  &  &  \\ \cline{1-11} \cline{13-17} 
% \end{tabular}
% }
% \end{table*}







% \begin{table*}[]
% \caption{}
% \label{tab:cross-v2}
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
% \hline
% \rowcolor[HTML]{EFEFEF} 
% Training\textbackslash{}Validation &  & S1(lab3) & S2(lab4) & S3(lab5) & S4 (lab6) & S5 (lab7) & S6(lab8) & S7(WF3) & S8(WF5) \\ \hline
% \cellcolor[HTML]{EFEFEF}S1(lab3) & SNR-\textgreater{}SR & \cellcolor[HTML]{C0C0C0}-0.0117 & -0.0413 & -0.0198 & -0.0400 & -0.0444 & -0.0867 & -0.0848 & -0.1679 \\ \hline
% \cellcolor[HTML]{EFEFEF}S2(lab4) & SNR-\textgreater{}SR & -0.0473 & \cellcolor[HTML]{C0C0C0}0.0808 & -0.0131 & -0.0239 & -0.1097 & -0.0691 & -0.0674 & -0.1427 \\ \hline
% \cellcolor[HTML]{EFEFEF}S3(lab5) & SNR-\textgreater{}SR & -0.2234 & -0.1519 & \cellcolor[HTML]{C0C0C0}0.2367 & -0.1851 & -0.1400 & -0.2586 & -0.2459 & -0.2402 \\ \hline
% \cellcolor[HTML]{EFEFEF}S4 (lab6) & SNR-\textgreater{}SR & 0.0120 & -0.0071 & 0.0032 & \cellcolor[HTML]{C0C0C0}0 & 0 & 0 & 0.0024 & 0.0027 \\ \hline
% \cellcolor[HTML]{EFEFEF}S5 (lab7) & SNR-\textgreater{}SR & -0.0332 & -0.0372 & -0.0384 & -0.0332 & \cellcolor[HTML]{C0C0C0}-0.0297 & -0.0608 & -0.0531 & -0.0476 \\ \hline
% \cellcolor[HTML]{EFEFEF}S6(lab8) & SNR-\textgreater{}SR & 0.0417 & 0.0080 & 0.0123 & 0.0242 & 0.0741 & \cellcolor[HTML]{C0C0C0}0.0146 & 0.0354 & -0.0041 \\ \hline
% \cellcolor[HTML]{EFEFEF}S7(WF3) & SNR-\textgreater{}SR & -0.0380 & -0.0406 & -0.0334 & -0.0174 & -0.0199 & -0.0216 & \cellcolor[HTML]{C0C0C0}0.0412 & -0.0262 \\ \hline
% \cellcolor[HTML]{EFEFEF}S8(WF5) & SNR-\textgreater{}SR & -0.0030 & -0.0143 & -0.0077 & -0.0053 & 0.0096 & -0.0112 & 0.0205 & \cellcolor[HTML]{C0C0C0}0.0192 \\ \hline
% \end{tabular}
% \end{table*}




% \begin{table*}[]
% \caption{1 scene with 2 tags and 5 poses }
% \label{tab:cross-v1}
% \resizebox{1.8\columnwidth}{!}{%
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|}
% \hline
% \rowcolor[HTML]{EFEFEF} 
% Training\textbackslash{}Validation & Method & \# Tag & S1 & S2 & S3 & S4 & S5 & S6 & S7 & mean & std \\ \hline
% \cellcolor[HTML]{EFEFEF} & NS & 2 & \cellcolor[HTML]{C0C0C0}{\color[HTML]{333333} 2.6618} & 8.7363 & 4.4712 & 7.3851 & 4.1269 & 7.1884 & 11.9767 & 7.3141 & 2.8991 \\ \cline{2-12} 
% \cellcolor[HTML]{EFEFEF} & GL$_1$ & 2 & \cellcolor[HTML]{C0C0C0}0.7728 & \textbf{2.3303} & \textbf{2.3230} & \textbf{1.6318} & \textbf{1.3694} & \textbf{1.9637} & \textbf{2.7427} & \textbf{2.0602} & \textbf{0.5055} \\ \cline{2-12} 
% \multirow{-3}{*}{\cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}S1\\ (4)\end{tabular}} & IoU & 2 & \cellcolor[HTML]{C0C0C0}-- & 2.4584 & 2.8110 & 2.1117 & 1.8733 & 2.2984 & 3.9435 & 2.5827 & 0.7383 \\ \hline
% \cellcolor[HTML]{EFEFEF} & NS & 2 & 3.3213 & \cellcolor[HTML]{C0C0C0}7.6645 & 4.9169 & 5.2951 & 4.0811 & 4.4345 & 7.7397 & 4.9648 & 1.5215 \\ \cline{2-12} 
% \cellcolor[HTML]{EFEFEF} & GL$_1$ & 2 & \textbf{2.1368} & \cellcolor[HTML]{C0C0C0}1.5181 & \textbf{3.2027} & \textbf{3.2589} & \textbf{2.4480} & \textbf{4.1563} & \textbf{4.4254} & \textbf{3.2713} & \textbf{0.9039} \\ \cline{2-12} 
% \multirow{-3}{*}{\cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}S2\\ (5)\end{tabular}} & IoU & 2 & 2.4965 & \cellcolor[HTML]{C0C0C0}-- & 3.4113 & 3.3785 & 2.7518 & 4.3019 & 3.6594 & 3.3332 & 0.6467 \\ \hline
% \cellcolor[HTML]{EFEFEF} & NS & 2 & 4.9909 & 9.5620 & \cellcolor[HTML]{C0C0C0}3.6271 & 8.7533 & 4.6421 & 10.1308 & 15.7764 & 8.9759 & 4.0654 \\ \cline{2-12} 
% \cellcolor[HTML]{EFEFEF} & GL$_1$ & 2 & \textbf{4.6720} & \textbf{5.9350} & \cellcolor[HTML]{C0C0C0}1.8469 & \textbf{6.9331} & \textbf{4.4352} & \textbf{8.9493} & \textbf{15.3862} & \textbf{7.7185} & \textbf{4.1029} \\ \cline{2-12} 
% \multirow{-3}{*}{\cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}S3\\ (6)\end{tabular}} & IoU & 2 & 5.2199 & 5.1830 & \cellcolor[HTML]{C0C0C0}-- & 7.5932 & 4.4382 & 9.5586 & 14.1518 & 7.6908 & 3.6937 \\ \hline
% \cellcolor[HTML]{EFEFEF} & NS & 2 & 21.2271 & 22.1641 & 17.5779 & \cellcolor[HTML]{C0C0C0}2.9452 & 15.9909 & 8.8797 & 15.3636 & 16.8672 & 4.7833 \\ \cline{2-12} 
% \cellcolor[HTML]{EFEFEF} & GL$_1$ & 2 & \textbf{4.3681} & \textbf{4.7176} & \textbf{4.4804} & \cellcolor[HTML]{C0C0C0}0.4986 & \textbf{3.9004} & \textbf{3.3891} & \textbf{3.7440} & \textbf{4.0999} & \textbf{0.5040} \\ \cline{2-12} 
% \multirow{-3}{*}{\cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}S4\\ (8)\end{tabular}} & IoU & 2 & 6.1193 & 6.3418 & 5.3863 & \cellcolor[HTML]{C0C0C0}-- & 5.2003 & 3.5784 & 5.7562 & 5.3970 & 0.9889 \\ \hline
% \cellcolor[HTML]{EFEFEF} & NS & 2 & 3.4621 & 8.3131 & 4.8500 & 7.6217 & \cellcolor[HTML]{C0C0C0}3.5197 & 7.4838 & 12.4364 & 7.3612 & 3.1066 \\ \cline{2-12} 
% \cellcolor[HTML]{EFEFEF} & GL$_1$ & 2 & \textbf{2.0590} & \textbf{2.9541} & \textbf{3.0224} & \textbf{3.5483} & \cellcolor[HTML]{C0C0C0}0.7392 & \textbf{3.1386} & \textbf{6.0885} & \textbf{3.4685} & \textbf{1.3733} \\ \cline{2-12} 
% \multirow{-3}{*}{\cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}S5\\ (9)\end{tabular}} & IoU & 2 & 1.3295 & 2.4713 & 2.5733 & 1.9232 & \cellcolor[HTML]{C0C0C0}-- & 1.7340 & 3.7268 & 2.2930 & 0.8419 \\ \hline
% \cellcolor[HTML]{EFEFEF} & NS & 2 & 29.4400 & 27.5404 & 27.9955 & 9.7005 & 20.6511 & \cellcolor[HTML]{C0C0C0}1.4253 & 9.5050 & 20.8054 & 9.1941 \\ \cline{2-12} 
% \cellcolor[HTML]{EFEFEF} & GL$_1$ & 2 & \textbf{5.1207} & \textbf{5.0574} & \textbf{5.3537} & \textbf{2.0539} & \textbf{4.1739} & \cellcolor[HTML]{C0C0C0}1.0012 & \textbf{2.4194} & \textbf{4.0298} & \textbf{1.4503} \\ \cline{2-12} 
% \multirow{-3}{*}{\cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}S6\\ (10)\end{tabular}} & IoU & 2 & \cellcolor[HTML]{FFFC9E}53.1274 & \cellcolor[HTML]{FFFC9E}52.7457 & \cellcolor[HTML]{FFFC9E}52.9046 & \cellcolor[HTML]{FFFC9E}61.7489 & \cellcolor[HTML]{FFFC9E}55.5216 & \cellcolor[HTML]{FFFC9E} & \cellcolor[HTML]{FFFC9E}59.7329 & \cellcolor[HTML]{FFFC9E}55.9635 & \cellcolor[HTML]{FFFC9E}3.8892 \\ \hline
% \cellcolor[HTML]{EFEFEF} & NS & 2 & 7.7991 & 9.9647 & 7.6857 & 4.1640 & 6.1619 & 2.3398 & \cellcolor[HTML]{C0C0C0}2.3708 & 6.3525 & 2.7512 \\ \cline{2-12} 
% \cellcolor[HTML]{EFEFEF} & GL$_1$ & 2 & \textbf{2.1563} & \textbf{2.7837} & \textbf{3.1058} & \textbf{1.3234} & \textbf{2.4537} & \textbf{2.0838} & \cellcolor[HTML]{C0C0C0}1.5389 & \textbf{2.3178} & \textbf{0.6207} \\ \cline{2-12} 
% \multirow{-3}{*}{\cellcolor[HTML]{EFEFEF}\begin{tabular}[c]{@{}c@{}}S7\\ (11)\end{tabular}} & IoU & 2 & 6.9715 & 7.5746 & 7.7603 & 6.9527 & 7.6966 & 6.3605 & \cellcolor[HTML]{C0C0C0}-- & 7.2194 & 0.5508 \\ \hline
% \cellcolor[HTML]{EFEFEF} & NS & 4 & 6.9426 & 9.6281 & 6.9136 & 3.9650 & 5.6420 & \cellcolor[HTML]{C0C0C0}2.2399 & \cellcolor[HTML]{C0C0C0}2.2399 & 6.6183 & 2.0764 \\ \cline{2-12} 
% \cellcolor[HTML]{EFEFEF} & GL$_1$ & 4 & \textbf{2.2409} & \textbf{2.5607} & \textbf{2.9773} & \textbf{1.8215} & \textbf{2.1995} & \cellcolor[HTML]{C0C0C0}0.3417 & \cellcolor[HTML]{C0C0C0}0.3417 & \textbf{2.3600} & \textbf{0.4334} \\ \cline{2-12} 
% \multirow{-3}{*}{\cellcolor[HTML]{EFEFEF}(10, 11)} & IoU & 4 & 3.1475 & 3.0735 & 3.5983 & 1.8910 & 2.7451 & \cellcolor[HTML]{C0C0C0}-- & \cellcolor[HTML]{C0C0C0}-- & 2.8911 & 0.6365 \\ \hline
% \cellcolor[HTML]{EFEFEF} & NS & 4 & 4.2476 & 8.5054 & 4.6712 & \cellcolor[HTML]{C0C0C0}2.8686 & 4.3311 & \cellcolor[HTML]{C0C0C0}{\color[HTML]{333333} 2.8686} & 2.8748 & 4.9260 & 2.1153 \\ \cline{2-12} 
% \cellcolor[HTML]{EFEFEF} & GL$_1$ & 4 & \textbf{1.0746} & \textbf{1.8871} & \textbf{2.3619} & \cellcolor[HTML]{C0C0C0}0.2341 & \textbf{1.5350} & \cellcolor[HTML]{C0C0C0}{\color[HTML]{333333} 0.2341} & \textbf{2.6191} & \textbf{1.8955} & \textbf{0.6215} \\ \cline{2-12} 
% \multirow{-3}{*}{\cellcolor[HTML]{EFEFEF}(8, 10)} & IoU & 4 & 1.8631 & 2.5341 & 2.5963 & \cellcolor[HTML]{C0C0C0}-- & 2.0956 & \cellcolor[HTML]{C0C0C0}-- & 3.0065 & 2.4191 & 0.4482 \\ \hline
% \cellcolor[HTML]{EFEFEF} & NS & 4 & 2.9309 & 8.0801 & 4.1196 & 3.4985 & \cellcolor[HTML]{C0C0C0}3.1519 & \cellcolor[HTML]{C0C0C0}3.1519 & 3.2204 & 4.3699 & 2.1201 \\ \cline{2-12} 
% \cellcolor[HTML]{EFEFEF} & GL$_1$ & 4 & \textbf{1.1541} & \textbf{2.1026} & \textbf{2.5017} & \textbf{1.4267} & \cellcolor[HTML]{C0C0C0}0.3291 & \cellcolor[HTML]{C0C0C0}0.3291 & \textbf{2.5693} & \textbf{1.9509} & \textbf{0.6361} \\ \cline{2-12} 
% \multirow{-3}{*}{\cellcolor[HTML]{EFEFEF}(10, 9)} & IoU & 4 & 1.0325 & 2.0526 & 2.3972 & 1.4497 & \cellcolor[HTML]{C0C0C0}-- & \cellcolor[HTML]{C0C0C0}-- & 2.4457 & 1.8755 & 0.6166 \\ \hline
% \cellcolor[HTML]{EFEFEF} & NS & 4 & 3.1991 & \cellcolor[HTML]{C0C0C0}{\color[HTML]{333333} 6.0812} & 4.7311 & 5.4558 & \cellcolor[HTML]{C0C0C0}{\color[HTML]{333333} 6.0812} & 4.8344 & 8.6576 & 5.3756 & 2.0139 \\ \cline{2-12} 
% \cellcolor[HTML]{EFEFEF} & GL$_1$ & 4 & \textbf{0.9538} & \cellcolor[HTML]{C0C0C0}{\color[HTML]{333333} 0.4803} & \textbf{2.3810} & \textbf{1.4556} & \cellcolor[HTML]{C0C0C0}{\color[HTML]{333333} 0.4803} & \textbf{1.1592} & \textbf{2.5277} & \textbf{1.6955} & \textbf{0.7172} \\ \cline{2-12} 
% \multirow{-3}{*}{\cellcolor[HTML]{EFEFEF}(5, 9)} & IoU & 4 & 1.3290 & \cellcolor[HTML]{C0C0C0} & 2.4685 & 2.1663 & \cellcolor[HTML]{C0C0C0} & 1.9265 & 3.8341 & 2.3449 & 0.9317 \\ \hline
% \cellcolor[HTML]{EFEFEF} & NS & 4 & 2.8820 & \cellcolor[HTML]{C0C0C0}6.2167 & \cellcolor[HTML]{C0C0C0}6.2167 & 4.4672 & 3.9536 & 3.7802 & 6.2324 & 4.2631 & 1.2406 \\ \cline{2-12} 
% \cellcolor[HTML]{EFEFEF} & GL$_1$ & 4 & \textbf{1.0896} & \cellcolor[HTML]{C0C0C0}0.4826 & \cellcolor[HTML]{C0C0C0}0.4826 & \textbf{1.5349} & \textbf{1.5938} & \textbf{1.5597} & \textbf{2.7543} & \textbf{1.7065} & \textbf{0.6209} \\ \cline{2-12} 
% \multirow{-3}{*}{\cellcolor[HTML]{EFEFEF}(5, 6)} & IoU & 4 & 1.2629 & \cellcolor[HTML]{C0C0C0} & \cellcolor[HTML]{C0C0C0} & 1.6148 & 1.7171 & 1.7248 & 2.1326 & 1.6905 & 0.3106 \\ \hline
% \cellcolor[HTML]{EFEFEF} & NS & 6 & 2.9824 & 8.0943 & 4.1273 & \cellcolor[HTML]{C0C0C0}3.2821 & \cellcolor[HTML]{C0C0C0}3.2821 & \cellcolor[HTML]{C0C0C0}3.2821 & 3.0841 & 4.5720 & 2.4045 \\ \cline{2-12} 
% \cellcolor[HTML]{EFEFEF} & GL$_1$ & 6 & 0.9713 & 1.9887 & 2.4395 & \cellcolor[HTML]{C0C0C0}0.3288 & \cellcolor[HTML]{C0C0C0}0.3288 & \cellcolor[HTML]{C0C0C0}0.3288 & 2.4369 & 1.9591 & 0.6918 \\ \cline{2-12} 
% \multirow{-3}{*}{\cellcolor[HTML]{EFEFEF}(8,9,10)} & IoU & 6 & 1.0201 & 2.1937 & 2.5195 & \cellcolor[HTML]{C0C0C0}-- & \cellcolor[HTML]{C0C0C0}-- & \cellcolor[HTML]{C0C0C0}-- & 2.4375 & 2.0427 & 0.6956 \\ \hline
% \cellcolor[HTML]{EFEFEF} & NS & 6 & 2.7816 & \cellcolor[HTML]{C0C0C0}5.5382 & \cellcolor[HTML]{C0C0C0}5.5382 & 4.5817 & \cellcolor[HTML]{C0C0C0}5.5382 & 3.8262 & 6.6229 & 4.4531 & 1.6239 \\ \cline{2-12} 
% \cellcolor[HTML]{EFEFEF} & GL$_1$ & 6 & \textbf{1.0022} & \cellcolor[HTML]{C0C0C0}0.4712 & \cellcolor[HTML]{C0C0C0}0.4712 & \textbf{1.4755} & \cellcolor[HTML]{C0C0C0}0.4712 & \textbf{1.1722} & \textbf{2.7791} & \textbf{1.6073} & \textbf{0.8054} \\ \cline{2-12} 
% \multirow{-3}{*}{\cellcolor[HTML]{EFEFEF}(5,6,9)} & IoU & 6 & 1.1076 & \cellcolor[HTML]{C0C0C0}-- & \cellcolor[HTML]{C0C0C0}-- & 1.9277 & \cellcolor[HTML]{C0C0C0}-- & 1.4411 & 2.5627 & 1.7598 & 0.6324 \\ \hline
% \cellcolor[HTML]{EFEFEF} & NS & 8 & 2.8878 & \cellcolor[HTML]{C0C0C0}4.9986 & \cellcolor[HTML]{C0C0C0}4.9986 & 3.7970 & \cellcolor[HTML]{C0C0C0}{\color[HTML]{333333} 4.9986} & \cellcolor[HTML]{C0C0C0}{\color[HTML]{333333} 4.9986} & 3.8550 & 3.5133 & 0.5424 \\ \cline{2-12} 
% \cellcolor[HTML]{EFEFEF} & GL$_1$ & 8 & \textbf{0.9410} & \cellcolor[HTML]{C0C0C0}0.4128 & \cellcolor[HTML]{C0C0C0}0.4128 & \textbf{1.4128} & \cellcolor[HTML]{C0C0C0}{\color[HTML]{333333} 0.4128} & \cellcolor[HTML]{C0C0C0}{\color[HTML]{333333} 0.4128} & \textbf{2.4504} & \textbf{1.6014} & \textbf{0.7721} \\ \cline{2-12} 
% \multirow{-3}{*}{\cellcolor[HTML]{EFEFEF}(5,6,9,10)} & IoU & 8 & 1.0304 & \cellcolor[HTML]{C0C0C0}-- & \cellcolor[HTML]{C0C0C0}-- & 1.7219 & \cellcolor[HTML]{C0C0C0}-- & \cellcolor[HTML]{C0C0C0}-- & 2.2808 & 1.6777 & 0.6264 \\ \hline
% \end{tabular}
% }
% \end{table*}

==> pre_tex/Experiments.tex <==
\section{Experimental Results}
\label{sec:ExperimentsAndResults}
In this section, we extensively evaluate our proposed method on seven different
scenes through a form of ``cross-validation'': in a round-robin fashion, we train on
one or more scenes and then evaluate on the remaining scenes. The quantitative
evaluation consists of computing pixel error per corner, where we take the image
corners as ground truth. We also show qualitative validation results by projecting
the LiDAR scans onto camera images; we include here as many as space allows, with
more scenes and larger images available at \cite{githubFile}. 

\subsection{Data Collection}
\label{sec:DataGathering}
The scenes include both outdoor and indoor settings. Each scene includes two targets,
one approximately 80.5~cm square and the other approximately 15.8~cm square, with the
smaller target placed closer to the camera-LiDAR pair. We use an \textit{Intel
RealSense Depth Camera D435} and a \textit{32-Beam Velodyne ULTRA Puck LiDAR},
mounted on an in-house designed torso for a Cassie-series bipedal robot
\cite{CassieAutonomy2019ExtendedEdition}. From the CAD file, the camera is roughly
20~cm below the LiDAR and 10~cm in front of it. The angle of the camera is
adjustable. Here, its ``pitch'', in the LiDAR frame, is approximately zero. 

A scan consists of the points collected in one revolution of the LiDAR's 32 beams.
The data corresponding to a single beam is also called a ring. For each scene, we
collect approximately 10~s of synchronized data, resulting in approximately 100 pairs
of scans and images. 

For each target, five consecutive pairs of LiDAR scans and camera images are selected
as a data set. For each data set, we apply two methods to estimate the vertices of
the targets, a baseline and the method in Sect.~\ref{sec:NewMethod}. 
% For each
%  \jwg{should have been commented out: target, 25 consecutive pairs of LiDAR scans and camera images are selected and
% divided into 5 data sets.} 
For each data set, we apply two methods to estimate the
vertices of the targets, a baseline and the method in Sect.~\ref{sec:NewMethod}.


\subsection{Baseline Implementation for LiDAR Vertices}
\label{sec:Baseline}
As a baseline, we use the method in \cite{zhou2018automatic}. Because an open-source
implementation was not released, we built our own, attempting to be as faithful as
possible to the described method. 

For each scan, the large and small targets are individually extracted from background
\cite{huang2019lidartag}. For each target and group of five scans, we compute the
extracted point cloud's centroid and center the point cloud about the origin. SVD is
then used to find the target's normal and to orthogonally project the point cloud
onto the plane defined by the normal and the centroid. For each scan, and for each
ring hitting the target, the left and right end points of the ring are selected and
then associated with one of the four edges of the target. Lines are fitted to each
collection of edge points using least-squares and \textit{ransac}. The vertices are
obtained as the intersections of the lines in the plane defined by the target's
normal and centroid. The four vertices are then re-projected to 3D space, as in
Fig.~\ref{fig:payload_LN2D}.



\subsection{Camera Corners and Associations}
\label{sec:CameraCorners}
The process of determining the target corners begins by clicking near them in the
image. This is the only manual intervention required in the paper and even this
process will soon be automated. As shown in Fig.~\ref{fig:Cannyedges},
between any given two clicked points, i.e., an edge of the target, a bounding box is
drawn around the two points. Once we have roughly located the corners of the target,
we process the image using the \textit{edge} command in MATLAB with the `Canny'
option to detect the edge points within the bounding box. A line is then fit through
each edge using \textit{ransac},  and the intersections of the resulting lines define
the target's corners, as shown in Fig.~\ref{fig:CannyLineFitted}. A video and an
implementation of this process is released along with the code.

\begin{figure}[t]%
\centering
\subfloat[]{%
\label{fig:Cannyedges}%
\includegraphics[width=0.48\columnwidth, trim={3.5cm 12.6cm 3cm 10cm},clip]{CannyLineFitted.png}}~
\hspace{2pt}%
\subfloat[]{%
\label{fig:CannyLineFitted}%
\includegraphics[width=0.5\columnwidth, trim={2cm 1.7cm 2cm 0.7cm},clip]{CannyLineFittedEnlarge-eps-converted-to.pdf}}%
\caption[]{\subref{fig:Cannyedges} shows the result of edge detection.
\subref{fig:CannyLineFitted} shows the interior pixels (marked in green) of a
bounding box given two clicked corners. The edge points and the edge line (as found by
\textit{ransac}) are marked in magenta and cyan, respectively. The corners are defined
by the intersections of the resulting lines.}% \label{fig:ImageEdgeDetection}%
\squeezeup
\end{figure}



\subsection{Extrinsic Calibration}
\label{sec:Extrinsic}
On the basis of the associated target vertices and camera-image corners, the PnP
method of \eqref{eq:PnP} is used to find the rigid-body transformation from LiDAR to
camera. We also checked using the IoU (see Sec.~\ref{sec:IoU}), but because the
results are similar, we are not reporting them here. The interested reader can
consult \cite{githubFile}. SVD and \textit{ransac} were computed using corresponding
MATLAB commands, while the optimizations in \eqref{eq:OurNewCost} and \eqref{eq:PnP}
were done with \texttt{fmincon}. 


\subsection{Quantitative Results and Round-robin Analysis}
\label{sec:QuantitativeResultS}

In Table~\ref{tab:cross-v1}, we present the RMS error of the LiDAR vertices projected
into the camera's image plane for the baseline\footnote{SVD to extract the normal and
\textit{ransac} for individual line fitting, with the vertices obtained as the
intersections of the lines.}, labeled \textbf{RN}, and our method in
\eqref{eq:JKHcost} and \eqref{eq:OurNewCost}, labeled \textbf{GL$_1$}. In the case of
two targets, a full round-robin study is performed: the rigid-body transformation
from LiDAR to camera is ``trained'' on the combined set of eight vertices from both
targets and then ``validated'' on the eight vertices of each of the remaining six
scenes. 

A complete round-robin study for four targets from two scenes would require 21
validations, while for six and eight targets, 35 validations each would be required.
For space reasons, we report only a subset of these possibilities. 

To be crystal clear, we are reporting in units pixel per corner
\begin{equation}
\label{eq:ErrorMeasure}
\resizebox{0.4\columnwidth}{!}{%
$\sqrt{\frac{1}{4n}\sum_{i=1}^{4n}\norm{\pre[L]Y_i-\pre[C]Y_i}_2^2},$
}
\end{equation}
where $4n$ is the total number of target corners. In the case of two targets and one
scene, $n=2$. In the case of six targets from three scenes, $n=6$.
Figure~\ref{fig:quantitative_results} illustrates several point clouds projected to
the corresponding camera images. Summary data is presented in Table~\ref{tab:SummaryTable}.

\input{ExperimentTables.tex}


\begin{figure*}[b!]%
\centering
\subfloat{%
% \label{fig:edges}%
\includegraphics[width=0.69\columnwidth, trim={0.5cm 1.0cm 0cm 0.5cm},clip]{v1-2.png}}~
\hspace{2pt}%
\subfloat{%
% \label{fig:edges}%
\includegraphics[width=0.69\columnwidth, trim={0.5cm 1.0cm 0cm 0.5cm},clip]{v3-2.png}}~
\hspace{2pt}%
\subfloat{%
% \label{fig:filled}%
\includegraphics[width=0.69\columnwidth, trim={0.5cm 1.0cm 0cm 0.5cm},clip]{v4-2.png}}\\
\hspace{2pt}%
\subfloat{%
% \label{fig:fiducial_edges}%
\includegraphics[width=0.69\columnwidth, trim={0.5cm 1.0cm 0cm 0.5cm},clip]{v5-2.png}}~
\hspace{2pt}%
\subfloat{%
% \label{fig:fiducial_edges}%
\includegraphics[width=0.69\columnwidth, trim={0.5cm 1.0cm 0cm 0.5cm},clip]{v6-2.png}}~
% \hspace{3pt}%
% \subfloat[]{%
% \label{fig:fiducial_edges}%
% \includegraphics[width=0.5\columnwidth]{v7.png}}~
\hspace{2pt}%
\subfloat{%
% \label{fig:color_points}%
\includegraphics[width=0.68\columnwidth, trim={0.5cm 1.0cm 0cm 0.5cm},clip]{v7-2.png}}%
\caption[]{Visual depiction of the validation data in the last row of
Table~\ref{tab:cross-v1}. For the method \textbf{GL$_1$}, five sets of estimated
LiDAR vertices for each target have been projected into the image plane and marked in
green, while the target's point cloud has been marked in red. Blowing up an image
allows the numbers reported in the table to be visualized. The vertices are key.}%
\label{fig:quantitative_results}%
\end{figure*}


\section{Qualitative Results and Discussion} 
\label{sec:QualitativeResults}

In LiDAR to camera calibration, due to the lack of ground truth, it is traditional to
show projections of LiDAR point clouds onto camera images. Often it is unclear if one
is viewing training data or validation data. In Figure~\ref{fig:TestingDataSet}, we
show a set of projections of LiDAR point clouds onto camera images for validation
data. An additional set of images can be found in~\cite{githubFile}. All of them show
that the key geometric features in the image and point cloud are well aligned. The
quality of the alignment has allowed our laboratory to build a high-quality
(real-time) 3D semantic map with our bipedal robot Cassie Blue \cite{gan2019bayesian}. The
map fuses LiDAR, camera, and IMU data;  with the addition of a simple planner, it led
to autonomous navigation \cite{CassieSemanticMappingYT}.

Tables~\ref{tab:cross-v1} and~\ref{tab:SummaryTable} show that \textbf{GL$_1$}
outperforms the baseline: on average, there is more than a 50\% reduction in projection error and a 70\% reduction in its variance. As for the sources of this improvement, we highlight the following points:
\begin{enumerate}
\renewcommand{\labelenumi}{(\alph{enumi})}
\setlength{\itemsep}{.2cm}
\item  Least-squares-based methods estimate a normal vector for the target's point
    cloud. As shown in Fig.~\ref{fig:FigureLiDARScanExample} and
    Fig.~\ref{fig:FigureLiDARScanExample3Rings}, even though the target is flat and
    has a well-defined normal, the returns in the LiDAR point cloud do not lie on a
    plane. Hence, a global normal vector does not exist. 

\item  Least-squares-based methods extract the target edge points from the point
    cloud for use in line fitting. The line fitting must be done in the plane defined
    by the estimated normal because, in 3D, non-parallel lines do not necessarily
    intersect to define a vertex.  

\item \textbf{GL$_1$} explicitly uses the target geometry in formulating the cost
    function. By assigning zero cost to interior points in the ``ideal target
    volume'' and non-zero otherwise, the optimization problem is focused on orienting
    the boundary of the target volume within the 3D point cloud. This perspective
    seems not to have been used before. 

\item Hence, our approach does not require the (tedious and error-prone)
\textit{explicit} extraction and assignment of points to target edges. The
determination of \textit{boundary points} in 3D is \textit{implicitly} being done
with the cost function. \end{enumerate}


At the present time, our extrinsic calibration method is not ``automatic''. The one manual intervention, namely clicking on the approximate target corners in the camera image, will be automated soon.  

We have not conducted a study on how to place the targets. This is an interesting piece of future work because of the nonlinear operation required when projecting LiDAR points to the camera plane; see \eqref{eq:projection_linear} and \eqref{eq:projection_nonlinear}.

\begin{figure*}[t!]%
\centering
\subfloat{%
% \label{fig:edges}%
\includegraphics[width=0.65\columnwidth, trim={0.5cm 1.0cm 0cm 0.5cm},clip]{test1_3.png}}~
\hspace{3pt}%
\subfloat{%
% \label{fig:edges}%
\includegraphics[width=0.65\columnwidth, trim={0.5cm 1.0cm 0cm 0.5cm},clip]{test2_3.png}}~
\hspace{3pt}%
\subfloat{%
% \label{fig:edges}%
\includegraphics[width=0.65\columnwidth, trim={0.5cm 1.0cm 0cm 0.5cm},clip]{test3_3.png}}\\
% \hspace{3pt}%
% \subfloat[]{%
% \label{fig:filled}%
% \includegraphics[width=0.5\columnwidth]{test4.png}}
\hspace{3pt}%
\subfloat{%
% \label{fig:fiducial_edges}%
\includegraphics[width=0.65\columnwidth, trim={0.5cm 1.0cm 0cm 0.5cm},clip]{test5_3.png}}~
\hspace{3pt}%
\subfloat{%
% \label{fig:fiducial_edges}%
\includegraphics[width=0.65\columnwidth, trim={0.5cm 1.0cm 0cm 0.5cm},clip]{test6_3.png}}~
% \hspace{3pt}%
% \subfloat[]{%
% \label{fig:fiducial_edges}%
% \includegraphics[width=0.5\columnwidth]{test7.png}}~
\hspace{3pt}%
\subfloat{%
% \label{fig:color_points}%
\includegraphics[width=0.65\columnwidth, trim={0.5cm 1.0cm 0cm 0.5cm},clip]{test7_3.png}}%
\caption[]{Qualitative validation results. For the method \textbf{GL$_1$} trained on S$_1$, the LiDAR point cloud has been projected into the image plane for the other data sets and marked in green. The red circles highlight various poles, door edges, desk legs, monitors, and sidewalk curbs where the quality of the alignment can be best judged. The reader may find other areas of interest. Enlarge in your browser for best viewing. }% \label{fig:detector}%
\label{fig:TestingDataSet}
\squeezeup
\end{figure*}





% \begin{figure*}[b!]
%  \centering
%   %trim={<left> <lower> <right> <upper>}
%  \includegraphics[scale=0.4,trim={10.1cm 20cm 1cm 5.2cm},clip]{TargetDistribution}
%  \caption{\jkh{The exp numbers have to be changed!}}
% \end{figure*}


==> pre_tex/ExtrinsicANDRefinement.tex <==
% \section{Extrinsic Optimization and Pose Refinement}
\section{Extrinsic Transformation Optimization}
\label{sec:extrinsic_opt}
This section assumes the vertices of the target in the LiDAR frame and in the
camera's image plane have been determined, along with their correspondences. The
optimization for the extrinsic transformation can be formulated in a standard PnP
problem: minimize Euclidean distance of the corresponding corners. We also propose 
maximizing the intersection over union (IoU) of the corresponding projected polygons.

% This section assumes the vertices of the target in the LiDAR frame and in the
% camera's image plane have been determined, along with their correspondences. The
% optimization for the extrinsic transformation can be formulated in two ways: minimize
% Euclidean distance of the corresponding corners or maximize the
% intersection over union (IoU) of the corresponding polygons. 

\subsection{Euclidean distance}
The standard PnP formulation is

\begin{align}
\label{eq:PnP}
    \left({R_L^C}^*, {T_L^C}^*\right) &:=  \argmin_{R,
    T}\sum_{i=1}^{4n}\norm{\Pi\left(X_i; R, T\right)-\pre[C]Y_i}_2^2\\
                                  &=\argmin_{R,
                                  T}\sum_{i=1}^{4n}\norm{\pre[L]Y_i-\pre[C]Y_i}_2^2,
\end{align}
where $\pre[C]Y_i\in \realnumbers^2$ are the camera corners, $\pre[L]Y_i\in
\realnumbers^2$ are defined in \eqref{eq:Projection}, and $n$ is the number of target
poses.

% The second method requires some geometry background. Assume we have a set of N
% vertices of a polygon $(x_i, y_i)$ in Cartesian coordinates. To sort the vertices in
% counterclockwise (CCW) direction, we apply Graham scan, a method to find the
% convex hull of a finite set of points on a plane \red{cite}. Given a set of sorted
% CCW points of vertices of a polygon $(x_i, y_i)$, the area of the polygon $(\A)$ can be calculated via
% Shoelace algorithm \red{cite}:
% \begin{equation}
%     \label{eq:Shoelace}
%     \A = \frac{1}{2}\left|\sum_{i=1}^{N} \det\begin{bmatrix} x_i & x_{i+1} \\ y_i &
%     y_{i+1}\end{bmatrix}\right|,
% \end{equation}
% where $x_{n+1} = x_1, x_0 = x_n$ as well as $y_{n+1} = y_1, y_0 = y_n$.

\subsection{IoU optimization}
\label{sec:IoU}
To compute the IoU of two projected polygons of the targets in an image plane, we
define the intersection as a polygon with known coordinates\footnote{The vertices of
the polygon consist of the 2D corners and the 2D line intersections and thus can be
computed efficiently.}. We sort the vertices of the polygon counterclockwise using
Graham scan, a method to find the convex hull of a finite set of points on a plane
\cite{graham1972efficient, andrew1979another}. The intersection area of the polygon ($\A$)
can be calculated via the Shoelace algorithm \cite{braden1986surveyor}:
\begin{equation}
    \label{eq:Shoelace}
    \A = \frac{1}{2}\left|\sum_{i=1}^{N} \det\begin{bmatrix} x_i & x_{i+1} \\ y_i &
    y_{i+1}\end{bmatrix}\right|,
\end{equation}
where $x_{n+1} = x_1, x_0 = x_n$ as well as $y_{n+1} = y_1, y_0 = y_n$. 
We use Venn diagram to solve the union of the two projected polygons of the targets
given the intersection calculated above and the area of each projection polygon.


% \subsection{Refinement of the \lidar~Target Vertices}\jkh{it does relate to both LiDAR and camera data}
% \label{sec:refinement}
% The above methods optimize $(R_L^C,T_L^C)$ for given values of $\{X_i\}_{i=1}^{4n}$. Due to the systematic errors mentioned in
% Sec.\ref{sec:lidar_analysis}, we suspect the LiDAR vertices are less accurate than those of the camera's image. We therefore propose a refinement of the vertices conditioned on the current estimate of the projection map, $\Pi$, in \eqref{eq:Projection}, that is, based on the current estimate of the extrinsic parameters $(R_L^C,T_L^C)$. Once the vertices are updated, new estimates for $(R_L^C,T_L^C)$ can be obtained, giving us an alternating two-step process:  

% \noindent \textbf{Step 1: Adjust vertices with current $\pre[][t]R_L^C,  \pre[][t] T_L^C$ held fixed} 
% % \vspace*{-.6cm}
% \begin{equation}
% \label{eq:RefinementAlgorithmStep1}
% \begin{aligned}
%  \delta H:=& \begin{bmatrix} \delta R &  \delta T \\ 0 & 1 \end{bmatrix}  \\
%   \delta H^*:= &  \argmin_{\delta H} \sum_{i=1}^{4n}\norm{\Pi\left( \delta H \circ \pre[][t]X_i;\pre[][t]R_L^C,  \pre[][t]T_L^C\right)-\pre[C]Y_i}_2^2\\ 
%                     ~&~~+ \rho C((H_L^{T}\circ \delta H)^{-1}(\mathcal{PC}));~ \text{and}
% \end{aligned}
% \end{equation}
% \noindent \textbf{Step 2: Refine calibration $R_L^C,  T_L^C$ using updated vertices}
% \begin{equation}
% \label{eq:RefinementAlgorithmStep2}
% \begin{aligned}                \pre[][t+1]X_i:= & \delta H^* \circ \pre[][t] X_i \\
%          \pre[~~L][t+1]Y_i= & \Pi\left( \pre[][t+1]X_i; \pre[][t]R_L^C,  \pre[][t]T_L^C\right),\\
%          \pre[][t+1]\left({R_L^C}^*, {T_L^C}^*\right) =&\argmin_{R,
%              T}\sum_{i=1}^{4n}\norm{\pre[~~L][t+1]Y_i - \pre[C]Y_i}_2^2,
% \end{aligned}
% \end{equation}
% where superscript $t$ denotes iteration number, ${X}_i$ and $\pre[C]Y_i$ are as before, and the weight $\rho$ trades off confidence in the point cloud vs the camera.


==> pre_tex/ImageProjection.tex <==
\section{Image Plane Corners and Correspondences with the LiDAR Vertices}
\label{sec:CameraStuff}

For a given camera image of a LiDAR target, let $\{ \pre[C]Y_i\}_{i=1}^4$ denote the
vertices of the camera image. We assume that these have been obtained through the
user's preferred method, such as corner detection \cite{harris1988combined,
rosten2006machine, rosten2008faster}, edge detection \cite{canny1987computational,
lim1990two, vincent2009descriptive}, or even manual selection. This is not the hard
part of the calibration problem. To achieve simple correspondences $X_i
\leftrightarrow \pre[C]Y_i$, the order of the indices on $\{ X_i\}_{i=1}^4$ may need
to be permuted; we use the vertical and horizontal positions to sort them. 


Once we have the correspondences, the next step is to project the vertices of the
\lidar~target, $\begin{bmatrix} x_i & y_i & z_i & 1 \end{bmatrix}^\transpose = X_i$,
into the image coordinates. The standard relations are \cite{hartley2000multiple,
forsyth2002computer}

\begin{align}
% \begin{equation}
    \label{eq:projection_linear}
    % \left(R_L^C^*, T_L^C^*\right) &=  \argmin_{R_L^C,
    % T_L^C}\sum_{i=1}^{N}\norm{\Pi_K\left(\pre[L]Y_i; R_L^C, T_L^C\right)-\pre[C]Y_i}_2^2\\
    %         &= \argmin_{R_L^C,
    %         T_L^C}\norm{\Pi_K\left(\pre[\textbf{L}]\textbf{Y}; R_L^C, T_L^C\right) - 
    %     \pre[\textbf{C}]\textbf{Y}}_F^2,
    \begin{bmatrix}
        u^\prime\\
        v^\prime\\
        w^\prime
    \end{bmatrix} &=
    \begin{bmatrix}
        f_x & s & c_x \\
        0 & f_y & c_y \\
        0 & 0 & 1
    \end{bmatrix}
    \begin{bmatrix}
    \mathbb{1}_{3\times3} \\ \zeros[1\times3]
    \end{bmatrix}^\transpose
    \begin{bmatrix}
        R_L^C & T_L^C \\
        \zeros[1\times 3] & 1 \\
    \end{bmatrix}
    \begin{bmatrix}
        x_i \\
        y_i \\
        z_i \\
        1
    \end{bmatrix}\\
% \end{equation}
% \begin{align}
% \begin{equation}
    \label{eq:projection_nonlinear}
    \pre[L]Y_i &= \begin{bmatrix}
        u & v & 1
    \end{bmatrix}^{\transpose} = 
    \begin{bmatrix}
        \frac{u^\prime}{w^\prime} & \frac{v^\prime}{w^\prime} & 1
    \end{bmatrix}^{\transpose},
% \end{equation}
\end{align}
where \eqref{eq:projection_linear} includes the camera's intrinsic parameters and the
extrinsic parameters $(R_L^C, T_L^C)$ that we seek. 

For later use, we combine \eqref{eq:projection_linear} and \eqref{eq:projection_nonlinear} to define 
\begin{equation}
\label{eq:Projection}
\Pi\left(X_i; R_L^C, T_L^C \right):=\pre[L]Y_i, 
\end{equation}
the projection map from LiDAR coordinates to image coordinates. Note that it is
a function of both the extrinsic variables and the LiDAR point cloud.


==> pre_tex/Introduction.tex <==
\section{Introduction and Related Work}
\label{sec:intro}
The desire to produce 3D-semantic maps \cite{Lu2020BKI} with our Cassie-series bipedal robot~\cite{gong2019feedback} has motivated us to fuse 3D-LiDAR and RGB-D
monocular camera data for autonomous navigation
\cite{CassieAutonomy2019ExtendedEdition}. Indeed, by mapping spatial LiDAR points
onto a segmented and labeled camera image, one can associate the label of a pixel (or
a region about it) to the LiDAR point as shown in Fig.~\ref{fig:semantic}. An error of a few degrees in rotation or a few percent in translation in the estimated rigid-body transformation between LiDAR and camera can lead to 20 cm reprojection errors at a distance of 5 m when overlaying a LiDAR point cloud on a camera image. Such errors will lead to navigation errors. 

In this paper, we assume that the intrinsic calibration of the two sensors has
already been done~\cite{mirzaei20123d} and focus on obtaining the rigid-body
transformation, i.e. rotation matrix and translation, between a LiDAR and camera.
This is a well studied problem with a rich literature that can be roughly divided
into methods that require targets:
\cite{gong20133d,dhall2017lidar,verma2019automatic,jiao2019novel,kim2019extrinsic,
guindel2017automatic, garcia2013lidar} and those that do not:
\cite{pandey2012automatic,taylor2013automatic,jeong2019road, jiang2018line,
zhen2019joint}. Our modest contributions are applicable to methods that use planar
polygonal targets, such as
checkerboards, triangles, and diamonds.


In target-based methods, one seeks to estimate a set of target features (e.g., edge
lines, normal vectors, vertices) in the LiDAR's point cloud and the camera's image
plane. If ``enough'' independent correspondences can be made, the LiDAR to camera
transformation can be found by Perspective-n-Point (PnP) as in
\cite{lepetit2009epnp}, that is, through an optimization problem of the form
\begin{equation}\label{eq:ConceptualProblem} (R_{C}^{L*}, T_{C}^{L*})= \mathrm{arg}
\min_{(R,T)}{\mathrm{dist}(P(H_{L}^{C}(X_i)),Y_i)}, \end{equation} where $X_i$ are
the (homogeneous) coordinates of the LiDAR features, $Y_i$ are the coordinates of the
camera features, $P$ is the often-called ``projection map'', $H_{L}^{C}$ is the
(homogeneous representation of) the LiDAR-frame to camera-frame transformation with
rotation matrix $R_{C}^{L}$ and translation $T_{C}^{L}$, and $\mathrm{dist}$ is a
distance or error measure.
 
 
 
\subsection{Rough Overview of the Most Common Target-based Approaches}
The works closest to ours are \cite{liao2018extrinsic,zhou2018automatic}. Each of
these works has noted that rotating a square target so that it presents itself as a
diamond can help to remove pose ambiguity due to the spacing of the ring lines; in
particular, see Fig.~2 in \cite{liao2018extrinsic} and Fig.~1 in
\cite{zhou2018automatic}. More generally, we recommend the literature overview in
\cite{liao2018extrinsic} for a recent, succinct survey of LiDAR to camera
calibration.  

 %trim={<left> <lower> <right> <upper>}
\begin{figure}[t]
\centering
\includegraphics[width=1\columnwidth, bb=0 0 1595 618]{graphics/FirstImage.jpg}
\caption{Building a semantic map for autonomous navigation. Once the transformation from LiDAR to camera is known, it is possible to fuse the LiDAR and RGB-camera information to build a 3D-map that is annotated with semantic information. The lower right shows a single camera image; its segmentation with semantic labels is shown in the upper right. Synchronized LiDAR points are mapped onto the camera image, associated to a semantic label, and then re-projected to a local frame \cite{hartley2019contact} along with the semantic labels to create a 3D semantically-labeled  map \cite{Lu2020BKI}, shown in the upper left. The sidewalk is marked in white, the grass in yellow-green, and trees in dark green. In the lower left, Cassie is using the map to plan a path around the North Campus Wave Field, while staying on the sidewalk.}
\label{fig:semantic}
\squeezeup
\end{figure}


The two most common sets of features in the area of target-based calibration are (a)
the 3D-coordinates of the vertices of a rectangular or triangular planar target, and
(b) the normal vector to the plane of the target and the lines connecting the
vertices in the plane of the target. Mathematically, these two sets of data are
equivalent: knowing one of them allows the determination of the other. In practice,
focusing on (b) leads to use of the SVD to find the normal vector and more broadly to
least squares line fitting problems \cite{zhou2018automatic}, while (a) opens up
other perspectives, as highlighted in \cite{liao2018extrinsic}.


% \begin{figure}[t]%
% \centering
% \subfloat{%
% \label{fig:semanticPC}%
% \centering
% \includegraphics[width=0.50\columnwidth, trim={14.1cm 2cm 1cm 8.2cm},clip]{semanticPC3.png}}%
% \hspace{5pt}%
% \subfloat{%
% \label{fig:semanticImg}%
% \centering
% \includegraphics[width=0.45\columnwidth, trim={0.00cm 0cm 0cm 0.cm},clip]{semanticImg.png}}%
% \caption[]{\jwg{Left image needs to be more fun and interesting} Using the obtained transformation, LiDAR points are mapped onto a semantically segmented image. Each point is associated with the label of a pixel. The road is marked as white; static objects such buildings as orange; the grass as yellow-green, and dark green indicates trees. \jwg{Add citation to YouTube video with nice map}}%
% \label{fig:semantic}%
% \squeezeup
% \end{figure}

 %trim={<left> <lower> <right> <upper>}
\begin{figure}[t]%
\centering
\subfloat[]{%
\label{fig:FigureLiDARScanExample}%
\includegraphics[width=0.49\columnwidth, trim={10cm 0cm 8cm 1cm},clip]{FigureLiDARScanExample2.png}}%
\hspace{3pt}%
\subfloat[]{%
\label{fig:FigureLiDARScanExample3Rings}%
\includegraphics[width=0.47\columnwidth, trim={10cm 0cm 10cm 0cm},clip]{payload_3d_selected.png}}\\
\hspace{3pt}%
\subfloat[]{%
    \label{fig:payload2D}%
\includegraphics[width=0.46\columnwidth, trim={1.5cm 0.5cm 3.5cm 1cm},clip]{payload_2d.png}}%
\hspace{3pt}%
\subfloat[]{%
    \label{fig:payload_LN2D}%
\includegraphics[width=0.43\columnwidth, trim={.5cm 0 3cm 0},clip]{payload_LN2D.png}}\\
\hspace{3pt}%
\subfloat[]{%
\label{fig:reference_frame}%
\includegraphics[width=0.45\columnwidth, trim={0.05cm 0cm 0cm 1cm},clip]{reference_frame2.png}}%
\hspace{3pt}%
\subfloat[]{%
\label{fig:reference_frame_side}%
\includegraphics[width=0.45\columnwidth, trim={0.05cm 0cm 0cm 0.77cm},clip]{reference_frame_side.png}}%
\caption[]{\subref{fig:FigureLiDARScanExample} Twenty five LiDAR scans of a planar
    target. The point cloud is roughly 7~cm thick.
    \subref{fig:FigureLiDARScanExample3Rings} The ``noise'' in the point cloud is not
    random. A zoom for four of the rings (13, 15, 17, 19) is typical and shows
    systematic errors in distance. \subref{fig:payload2D} \lidar~points orthogonally
    projected to the plane defined by the normal. \subref{fig:payload_LN2D} Example
    edge points selected to regress a line via \textit{ransac}.
    \subref{fig:reference_frame} Target reference frame and real point cloud data.
    The dotted blue square is the reference target; its vertices are denoted
    $\{\bar{X}_i\}_{i=1}^4$. \subref{fig:reference_frame_side} A side-$(x-z)$-view
highlighting the non-zero thickness of a typical point cloud. These figures and all
others in the paper are of sufficient resolution that they can be blown up to see
detail. }%
\label{}%
\squeezeup
\end{figure}

% \begin{figure}[b]
% 	\centering
% 	\includegraphics[width=\columnwidth]{graphics/FigureLiDARScanExample.png}
% 	\caption{Twenty five LiDAR scans of a planar target. The `noise' in the point cloud is not random.}
% 	\label{fig:FigureLiDARScanExample}
% \end{figure}

Figure~\ref{fig:FigureLiDARScanExample} shows a 3D view of 25 scans from a
factory-calibrated 32-Beam Velodyne ULTRA Puck LiDAR on a diamond shaped planar
target, with a zoom provided in Fig.~\ref{fig:FigureLiDARScanExample3Rings}. There
are clearly systematic errors in the distance (or depth) measurement of the target,
and these errors affect the estimation of the target's ``centroid'', which is
commonly used to determine the translation of the target from the LiDAR and the
target's ``normal vector'', which is used to define the plane of the target as in
Fig.~\ref{fig:payload2D}. Subsequently, the point cloud is orthogonally projected to
this plane and the line boundaries of the target are found by performing
\textit{ransac} on the appropriate set of ring edges; see
Fig.~\ref{fig:payload_LN2D}. The lines along the target's boundaries then define its
vertices in the plane, which for later reference, we note are not constrained to be
compatible with the target's geometry. 

Once the vertices in the plane of the target have been determined, then knowledge of
the target's normal allows the vertices to be lifted back to the coordinates of the
point cloud. This process may be repeated for multiple scans of a target, aggregates
of multiple scans of a target, or several targets, leading to a list of target
vertices $\{ X_i \}_{i=1}^{4n} $, where $n$ is the number of target poses.

The target is typically designed so that the vertices are easily distinguishable in
the camera image. Denoting their corresponding coordinates in the image plane by $\{
Y_i \}_{i=1}^{4n}$ completes the data required for the conceptual fitting problem in
\eqref{eq:ConceptualProblem}. While the problem is nonlinear and non-convex, this is
typically not a problem because CAD data can provide an adequate initial guess for
local solvers, such as Levenberg-Marquardt; see \cite{zhou2018automatic} for example. 



% \begin{figure}[b]
% \vspace{-2mm}
% 	\centering
% 	\includegraphics[width=\columnwidth]{graphics/FigureLiDARScanExample3Rings.png}
% 	\caption{[Should go side by side with previous figure] Zoom in on three of the rings (7, 12, and 17) of Fig.~\fig{fig:FigureLiDARScanExample} }
% 	\label{fig:FigureLiDARScanExample3Rings}
% \squeezeup \squeezeup
% \end{figure}


\subsection{Our Contributions}
\label{sec:Contributions}
Our contributions can be summarized as follows. 
\begin{enumerate}
\setlength{\itemsep}{.15in}
\renewcommand{\labelenumi}{(\alph{enumi})}
% 	\item We make use of the target's geometry when estimating its vertices. In
% particular, if the target is a diamond, vertices form right angles and the
% lengths of the sides are equal. We show that this simple change improves the
% accuracy of estimating the vertices. Essentially, the extra constraints allow
% all of the target's boundary points to be pulled into the regression problem at
% once, instead of parsing them into individual edges of the target, where small
% numbers of points on some of the edges will accentuate the quantization effects due to sparsity
% in a LiDAR point cloud. \jkh{remove edge parsing and line-ransac}

% \item We make use of the target's geometry when estimating its vertices. In
% particular, if the target is a diamond, vertices form right angles and the
% lengths of the sides are equal. 

\item We introduce a novel method for estimating the rigid-body transform from target
    to LiDAR, $H_{T}^{L}$. For the point cloud pulled back to the origin of the LiDAR
    frame via the current estimate of the transformation, the cost is defined as the
    sum of the distance of a point to a 3D-reference target of known
    geometry\footnote{It has been given non-zero volume.} in the LiDAR frame, for
    those points landing outside of the reference target, and zero otherwise. We use
    an $L_1$-inspired norm in this work to define distance. Consistent with
    \cite{liao2018extrinsic}, we find that this is less sensitive to outliers than
    $L_2$-line fitting to edge points\footnote{Defined as the left-right end points
    of each LiDAR ring landing on the target.} using \textit{ransac}
    \cite{zhou2018automatic}.

\item In the above, by using the entire target point cloud when estimating the
    vertices, we avoid all together the delicate task of identifying the edge points
    and parsing them into individual edges of the target, where small numbers of
    points on some of the edges accentuate the quantization effects due to sparsity
    in a LiDAR point cloud.

% 	\item We exploit the fact that the variance of the camera data is
% significantly lower than that of the LiDAR data. Hence, after the LiDAR to
% camera transformation has been estimated by solving the PnP problem, we
% introduce a refinement step to the estimated pose of the LiDAR target given the
% current estimate of the LiDAR to camera transformation. In this process, the
% modified vertices remain consistent with the target geometry and the target's
% point cloud. \jwg{Called Ridiculous in the reviews}

\item We provide a round-robin validation study to compare our approach to a
    state-of-the-art method from 2018, namely  \cite{zhou2018automatic}. A novel
    feature is the use of the camera image as a proxy for ground truth; in the
    context of 3D semantic mapping, this makes sense.  A standard PnP method~\cite{lepetit2009epnp} is
    used to estimate the rigid-body transformation
    from LiDAR to camera. We also validate our algorithm
    on different numbers of targets.

\item Code for our method, our implementation of the baseline, and all the
    data sets used in this paper are released as
    \href{https://github.com/UMich-BipedLab/extrinsic_lidar_camera_calibration}{open
    source}; see \cite{githubFile}.
\end{enumerate}


\begin{comment}

\subsection{More on Related Work}
\label{sec:RelatedWork}

Papers to talk about

\begin{itemize}
    \item Simultaneous intrinsic and extrinsic
    \item When there is a large separation between lidar and camera
    \item SVD prevleance
    \item Ransac
    \item \textbf{Most closely related to our work:} Extrinsic calibration of lidar and camera with polygon
\end{itemize}
\end{comment}

% \subsection{Paper Outline}
% The remainder of the paper is structured....


==> pre_tex/ProblemStatementANDLiDARTagPose.tex <==
\section{Problem Statement and Target Pose}
\label{sec:lidar}
This section describes what elements we need to solve the \lc~calibration problem,
\lidar's point clouds analysis, how to find 3D-2D correspondences and some important
things to keep in mind when doing \lc~calibration as specially \lidar's
irregular returns.


\subsection{Problem Statement}
The core of the problem is to
find a rigid body transform $H_L^C$ between a \lidar~and a camera, which
consists of 6 parameters, including a rotation
60
 matrix $\pre[L]R_L^C$ in $\SO(3)$ and
a translation $\pre[L]T_L^C$ in $\realnumbers^3$, where $\pre[L]R_L^C$ and
$\pre[L]T_L^C$ stands for the rotation and translation from a \lidar~ to a camera
represented in \lidar~frame, respectively. In target-based calibration, we need some
correspondences, features to match between a \lidar~and a camera. There are several
ways to represent features such as plane-line, plane-point, 3D line-line
correspondence or formulate as a Perspective-n-Point (PnP) problem. 

In this paper, we use fiducial tags to find correspondences in both 3D \lidar~point
cloud and in 2D images. Fiducial tags that detected from a \lidar~is called
\lidarts~and the same fiducial tags that detected from a camera is called \atags. A
pose of a \lidart~is provided from \red{cite}; the original method to obtain a
\lidart's pose, a transformation from \lidar~from to \lidart~frame $(H_L^T)$, is
running at realtime at 30 Hz; however, it is not accurate enough for calibration due
to noise level of \lidar~point cloud and thus has to be re-optimized mentioned in
Sec.~\ref{sec:lidartag_opt}. The noise level of \lidar~point cloud is discussed in
Sec.~\ref{sec:lidar_analysis}. Once the pose of the \lidart~is accurately obtained,
we then have 4 corners of the \lidart~in 3D. The same target in an image,  the 4
corners of the \atag~can be detected from \atag~detector in 2D. Therefore, this
allows us to have a set of 3D-2D correspondences on a target. The problem then
becomes a PnP optimization problem to compute a projection matrix mentioned in
Sec.~\ref{sec:extrinsic_opt}. However, this is not the end of the calibration. The
calibration up to this point assumes the corners given from \lidarts~are absolutely
correct. However the noise level of \lidar~point cloud, we still cannot fully trust
the optimization result of the \lidart. We have to do another refinement to the
\lidarts' poses given the projection matrix along with a regularizer mentioned in
Sec.~\ref{sec:refinement}.


\begin{remark}{
    \normalfont
One may argue why not directly using the optimized poses to do calibration, since two
poses from the two different sensors have been given already. It could be done easily
by: 
\begin{equation}H_L^C = H_L^{T_L} H_{T_L}^{T_C}\inv{\left(H_C^{T_{C}}\right)},
\end{equation} 
where $H_{T_L}^{T_C}$ is a
transformation from the \lidart~frame $(T_L)$ to the \atag~frame $(T_C)$. However,
this yet gives us good enough calibration result due to estimating an \atag~pose from
a monocular camera.}
\end{remark}

% In this paper, matrices and vectors are marked in bold. 
% $\prescript{}{L}{P}_A$ stands for a point A represented in \lidar frame. 
% A homogeneous transformation $\H$ consists of a rotation matrix $\pre[L]\R[L][T]$ and a translation vector
% $\pre[L]\T[L][T]$: $$\H[L][T] = \begin{bmatrix}\pre[L]\R[L][T] & \pre[L]\T[L][T] \\
% \zeros &1\end{bmatrix},$$

\subsection{\lidar~Point Cloud Analysis}
\label{sec:lidar_analysis} 
\lidars~have dense region and sparse region on the z-axis as shown in Fig.~\red{dense
region}. We use a 32-beam Velodyne Ultra Puck, the resolution on z-axis is
\red{number} and \red{number} of the dense region and the sparse region respectively.
The points resolution on the y-axis is \red{number}. The quantization error on both
y-axis and z-axis direction could be roughly computed from: As a result, the
quantization error could get quite large if one place the tag at a far distance.
In Fig.~\red{Calibration error} shows if we have 1 degree on each axis and 5\% of
translation error, the calibration result is not good enough for our application.
Thus, it is essential to use geometry constraint to estimate a \lidart~pose as well as
to place a \lidart~at a tilted angle so that the geometry constraint can pick up the
quantization error on y-axis and z-axis. To overcome quantization error on x-axis, we
accumulate a few scans to estimate one \lidrt~pose and condition on the current
estimate of projection matrix to refine the \lidart's poses mentioned in
Sec.~\ref{sec:refinement}.



\subsection{Correspondences and Automatic Detection}
\label{sec:correspondences}
\subsubsection{\lidart~Poses Optimization and Automatic Detection}
\label{sec:lidartag_opt}
To find 3D correspondences in \lidar~point cloud, we use corners of a \lidart~as our
\lidar~target. Patches \lidarts' point clouds are automatically detected from a full
scan of point cloud by \red{cite} and therefore we can assume they are given in this
paper. When estimating a \lidart' pose using its centroid and a normal vector
computed by taking svd of the \lidart's points (more detail, please refer to
\red{cite}), which is fast and suitable for realtime application; however, we notice
there are observable noise of the normal vector and centroid. We further look into
the \lidart~points; we observe the points on the \lidart, a planner object, they
appears as a cube, as shown in Fig.~\red{lidartag cube}. The min/max of the
difference of depth could be 5 cm to 15 cm on x-axis direction; the standard
deviation is also noticeable as shown in Table.~\red{payload point analysis}. The
orientation also has a few degree of variance. As shown in Fig.~\red{calibration
error}, this error is large enough to ruin the calibration. To more accurately
estimate a \lidart~pose, we formulate another optimization problem that does not use
its centroid nor normal vector but take into account its underline noise.

We place an ideal reference target at the center of the \lidar~frame as shown in
Fig.~\red{reference frame}. We want to find the best homogeneous transformation
$H_T^L$ that takes the \lidart~''back'' to the ideal reference target. To do so, we
define a cost function based upon the known geometry (diamond), size (d) and the
noisy level on x-axis (k) of the \lidart. Given a set of \lidart's point cloud
$\pre[L]X_i(x_i, y_i, z_i)$ , 8 corners of the ideal reference frame $\pre[L]Y_i^\prime$,
and the current estimate of $\pre[L]\tilde{R}_T^L$ and $\pre[L]\tilde{T}_T^L$ the
cost for the \lidart's point cloud is defined as: 

% \begin{align}
%     c(X) = \sum_{i=1}^{N} 
%     &\min\left(||x_i- \frac{0.01}{2}||^p, ||x_i-\frac{0.01}{2}||^p\right) + \\
%     &\min\left(||y_i- \frac{d}{2}||^p, ||(y_i- \frac{-d}{2}||^p\right) + \\
%     &\min\left(||z_i- \frac{d}{2}||^p, ||(z_i- \frac{-d}{2}||^p\right).
% \end{align}
% \begin{align}
%     c(X, \widetilde{R_T^L}, \widetilde{T_T^L}) = \sum_{i=1}^{N} &c_x(x_i, \widetilde{R_T^L}_{1,:}, \widetilde{T_L^T}_{1}) + \\
%                                                                 &c_y(y_i, \widetilde{R_T^L}_{2,:}, \widetilde{T_L^T}_2) + \\
%                                                                 &c_z(z_i, \widetilde{R_T^L}_{3,:}, \widetilde{T_L^T}_3),
% \end{align}
\begin{equation}
    \pre[L]\tilde{X_i} = \left(\pre[L]\tilde{R}_T^L\right)\left(\pre[L]X_i\right) + 
    \pre[L]\tilde{T}_T^L
\end{equation}
\begin{equation}
    C(\pre[L]\tilde{X}) = \sum_{i=1}^{N} &c_x(\tilde{x}_i) + \\
                                  &c_y(\tilde{y}_i) + \\
                                  &c_z(\tilde{z}_i),
\end{equation}
% where $\widetilde{R_T^L}, \widetilde{T_T^L}, c_x(x), c_y(y)$ and $c_z(z)$ are:
% \begin{equation}
%     \widetilde{R_T^L} = \begin{bmatrix} \widetilde{R_T^L}_1\\ \widetilde{R_T^L}_2 \\ \widetilde{R_T^L}_3\end{bmatrix}
% \end{equation}
where $c_x(\tilde{x}), c_y(\tilde{y})$ and $c_z(\tilde{z})$ are:
% \scalebox{0.9}{%
 \begin{equation}
% c_x(x_i, \widetilde{R_T^L}_{1,:}, \widetilde{T_L^T}_{1}) =
     c_x(\tilde{x}_i) =
    \begin{cases}
        \min\left(||\tilde{x}_i- \frac{k}{2}||^p, ||(\tilde{x}_i- \frac{-k}{2}||^p\right), & 
        \text{if } \frac{-k}{2}\leq \tilde{x}_i \leq \frac{k}{2}\\\
        0, & \text{otherwise}.
    \end{cases}
\end{equation}
%}
\begin{equation}
    c_y(\tilde{y}_i) = 
    \begin{cases}
        \min\left(||\tilde{y}_i- \frac{d}{2}||^p, ||(\tilde{y}_i- \frac{-d}{2}||^p\right), & 
        \text{if } \frac{-d}{2}\leq \tilde{y}_i \leq \frac{d}{2}\\\
        0, & \text{otherwise}.
    \end{cases}
\end{equation}
\begin{equation}
    c_z(\tilde{z}_i) = 
    \begin{cases}
        \min\left(||\tilde{z}_i- \frac{d}{2}||^p, ||(\tilde{z}_i- \frac{-d}{2}||^p\right), & 
        \text{if } \frac{-d}{2}\leq \tilde{z}_i \leq \frac{d}{2}\\\
        0, & \text{otherwise}.
    \end{cases}
\end{equation}
The optimal $H_T^L^*$ can be determined:
\begin{align}
    H_T^L^* &= \argmin_{\pre[L]\tilde{R}_T^L, \pre[L]\tilde{T}_T^L}
    C(\pre[L]\tilde{X}, \pre[L]\tilde{R}_T^L, \pre[L]\tilde{T}_T^L)\nonumber \\ &=
    \argmin_{\pre[L]\tilde{R}_T^L, \pre[L]\tilde{T}_T^L} \sum_{i=1}^{N} c_x(\tilde{x}_i) +
    c_y(\tilde{y}_i) + c_z(\tilde{z}_i).
\end{align}

Conceptually, if a transformed point is inside the ideal reference frame, the cost is zero;
otherwise, we penalize its each axis with p-norm to a closest boundary of the ideal reference
frame along the same axis. In this work, we choose L1-norm and we find this cost is also robust
to outliers as shown in Fig.\red{robust to outliers}.

We now have an optimized $H_T^L$, a transformation from a \lidart~frame to the ideal
reference frame and we also have the 8 corners of the ideal reference target
$\pre[L]Y_i^\prime$. We can compute the 8 corners \footnote{These 8 corners are two
planes with geometry constraints; we can take the average of the two planes to
find the neutral plane with 4 corners.} of the \lidart~($\pre[L]Y_i$) easily by:
\begin{equation}
    \pre[L]Y_i = \inv{\left(H_T^L\right)} \pre[L]Y_i^\prime,
\end{equation}
where these corners will be refined again after the projection matrix is estimated.

\subsubsection{Image correspondences from \atags}
\label{sec:apriltag_correspondences}
Getting corners correspondence from the same fiducial tag in an image is fairly
easier and straight forward. The corners of the fiducial tag in an image, namely an
\atag, can be automatically detected by the \atag detector. In original
papers\cite{olson2011apriltag}, \cite{wang2016apriltag}, \cite{krogiusflexible}, the corners are defined at the payload corners\footnote{The
detector finds four-sided regions that have darker interior than their exterior in
the whole image.}, shown in Fig.~\red{payload explain}. However, we can use the detected
corners and tag-relative coordinates to backstep to the outer 4 corners $\pre{C}Y_i$.


==> pre_tex/Related.tex <==
\section{Related Work}
\label{sec:related_work}

==> pre_tex/TargetVerticesLiDARframe.tex <==
\section{Finding the LiDAR Target Vertices}
\label{sec:LiDARTargetVertices}

In this conference version of the work, we will assume that each target is planar,
square, and rotated in the frame of the LiDAR by roughly 45$^\circ$ to form a diamond
as in Fig.~\ref{fig:FigureLiDARScanExample}. As indicated in
\cite{liao2018extrinsic,zhou2018automatic}, placing the targets so that the rings of
the LiDAR run parallel to its edges leads to ambiguity in the vertical position due
to the spacing of the rings.  We assume that standard methods have been used to
automatically isolate the target's point cloud \cite{huang2019lidartag} and speak no
further about it. 

We take as a target's features its four vertices, with their coordinates in the LiDAR
frame denoted $\{ X_i \}_{i=1}^{4};$ when useful, we abuse notation and pass from
ordinary coordinates to homogeneous coordinates without noting the distinction. The
vertices  $\{ X_i \}_{i=1}^{4} $ are of course not directly observable in the point
cloud. This section will provide a new method for estimating their coordinates in the
frame of the LiDAR using an $L_1$-like norm. 

%It will also
%provide a simple improvement to existing methods that use least squares fitting.

% \begin{figure}[t]%
% \centering
% \subfloat[]{%
% \label{fig:reference_frame}%
% \includegraphics[width=0.38\columnwidth, trim={0.05cm 0cm 0cm 1cm},clip]{reference_frame.png}}%
% \hspace{1pt}%
% \subfloat[]{%
% \label{fig:reference_frame_side}%
% \includegraphics[width=0.38\columnwidth, trim={0.05cm 0cm 0cm 0.77cm},clip]{reference_frame_side.png}}%
% \caption[]{Target reference frame and real point cloud
% data. \subref{fig:reference_frame}  The dotted blue square is the reference target; its vertices are denoted $\{\bar{X}_i\}_{i=1}^4$. \subref{fig:reference_frame_side} A
% side-$(x-y)$-view highlighting the non-zero thickness of a typical point cloud.}%
% \label{fig:}%
% \squeezeup
% \end{figure}

 %trim={<left> <lower> <right> <upper>}
\begin{figure}[t]%
\centering
\subfloat[]{%
    \label{fig:disturbance}%
    \centering
\includegraphics[width=0.42\columnwidth, trim={3cm 0.56cm 4.5cm 3cm},clip]{disturbance.png}}%
\hspace{10pt}%
\subfloat[]{%
\label{fig:undisturbance}%
\centering
\includegraphics[width=0.41\columnwidth, trim={3cm 0.6cm 4.5cm 3cm},clip]{undisturbance.png}}%
\caption[]{\subref{fig:disturbance} shows that a calibration result is not usable if
it has few degrees of rotation error and a few percent of translation error.
\subref{fig:undisturbance} shows good alignment of a \lidar~point cloud projected
onto a camera image.}% \squeezeup
\vspace{-2mm}
\end{figure}



\subsection{Remarks on LiDAR Point Clouds}
\label{sec:lidar_analysis} 
\lidars have dense regions and sparse regions along the z-axis, as shown in
Fig.~\ref{fig:payload2D}. For a 32-beam Velodyne Ultra Puck, we estimate the
resolution along the z-axis is $0.33^\circ$ and $1.36^\circ$ in the dense and sparse
regions, respectively. A point's distance resolution along the y-axis is roughly
$0.1^\circ$. 
The quantization error could be roughly computed from: $d\sin{\theta}$
when a point is at $d$ meter away. As a result, the quantization error could get
quite large if one place the tag at a far distance. Figure~\ref{fig:disturbance}
shows that a $1^\circ$ of rotation error on each axis and 5\% error in translation
can significantly degrade a calibration result. As noted in
\cite{liao2018extrinsic,zhou2018automatic}, it is essential to place a target at an
appropriate angle so that known geometry can mitigate quantization error in the $y$-
and $z$-axes. 

%% related to refinement
% \jkh{please check}
% To overcome quantization error in the $y$-axis and $z$-axes, we proposed a refinement step in
% \cite{huang2019improvements} to modify the estimated vertices. The refinement step conditions
% on the current estimate of the projection map, image corners as well as a weighted
% loss on \eqref{eq:JKHcost}. However, due to the limited space, we do not apply this step.
% To overcome quantization error in the $x$-axis, we accumulate a few
% scans to estimate a target's pose and ``condition'' on the current estimate of LiDAR
% to image plane projection matrix to refine the target's pose. 

\subsection{New Method for Determining Target Vertices}
\label{sec:NewMethod}

Let ${\cal PC}$ denote the LiDAR target point cloud and let the collection of 3D points be
${\cal X}_i$ so that ${\cal PC} = \{ \chi_i\}_{i=1}^N$. The objective is to fit a
reference target with vertices $\{ \bar{X}_i \}_{i=1}^4$, defined as in
Fig.~\ref{fig:reference_frame}, onto the point cloud with ``minimum error''. It is
actually easier to pull the $\pc$ to the origin of the LiDAR through the current
estimate of the inverse transformation $H_T^L:=(H_L^T)^{-1}$ and measure the error
there. 

\begin{remark}
    \label{remark:Xis}
    To be clear, what we seek is a ``best estimate'' of the target vertices in the LiDAR
    frame and not the transformation itself. Our method is indirect because from the
    point cloud, we estimate a ``best'' LiDAR to target transformation, call it
    $H_L^{T^*}$, and use it to define the vertices 

    \begin{equation}
    \label{eq:vertices}
    X_i^*:=H_L^{T^*}(\bar{X}_i), ~~1 \le i \le 4.
    \end{equation}

    The correspondences of the estimated vertices with the physical top, bottom, and left
    or right sides of the target are not needed at this point.  $\blacksquare$
\end{remark}

For $a \ge 0$ and $\lambda \in \real$, define

\begin{equation}
    \label{eq:L1cost}
    c(\lambda,a):=\begin{cases} 
    \min\{ |\lambda-a|, |\lambda + a| \} & \text{if}~|\lambda| >a \\
    0 & \text{otherwise}
    \end{cases};
\end{equation}

see also the ``soft $L_1$ norm'' in \cite{liao2018extrinsic}. Let
$\{\tilde{\chi}_i\}_{i=1}^N:=H_T^L(\mathcal{PC}):=\{ H_T^L(\chi_i) \}_{i=1}^N$ denote
the pullback of the point cloud by $H_T^L$, and denote a point's $(x,y,z)$-entries by
$(\tilde{x}_i,\tilde{y}_i,\tilde{z}_i)$. The cost is defined as 

\begin{equation}
\label{eq:JKHcost}
    C(H_T^L(\mathcal{PC})):=\sum_{i=1}^{N} c(\tilde{x}_i,\epsilon) +
    c(\tilde{y}_i,d/2) +  c(\tilde{z}_i,d/2),
\end{equation}
where $\epsilon \ge 0$ is a tuning parameter to account for uncertainty in the depth
measurement of the planar target; see Fig.~\ref{fig:reference_frame}. 


We propose to determine the optimal $H_T^L$ by
\begin{equation}
\label{eq:OurNewCost}
    H_T^{L^*} := \argmin_{\pre[L]\tilde{R}_T^L, \pre[L]\tilde{T}_T^L}
   C(H_T^L(\mathcal{PC})).
\end{equation}
Once the transformation is determined, the target vertices are defined by
$X_i := (H_T^{L*})^{-1}(\bar{X}_i), i=1,\cdots,4,$ as in Remark~\ref{remark:Xis}. 

\begin{remark} It is underlined that the target vertices are being determined without
extraction of edge points and their assignment to a side of the target. The cost in
\eqref{eq:JKHcost} treats the target as a rectangular volume.  
\end{remark}


% \subsection{Improvement to Least Squares Approaches for Finding the Target Vertices}
% \jwg{Remove this? }We assume the target's normal vector has been estimated using methods in \cite{liao2018extrinsic,zhou2018automatic} and
% that the point cloud $\pc$ has been orthognally projected to the plane of the target. In
% \cite{liao2018extrinsic,zhou2018automatic}, lines along the four edges of the projected target are regressed
% individually after appropriately parsing the edge points. For ``robustness'',
%  \textit{ransac} is typically used. 

% %using the associated sets of edge points which we denote %$$\{\mathcal{E}^k_j\}_{k=1,j=1}^{k=4,j=n_k}.$$ 

% Instead, we propose to use all of the edge points simultaneously when regressing the
% edges. The basic formulation remains one of fitting four lines to the four sets of
% edge points, as is standard in the area, 
% \begin{equation}
%     \label{eq:lines}
%     z=m_i y + b_i,  1 \le i \le 4
% \end{equation}
% and then adding in the constraints for a square. For opposite sides to be parallel, one needs
% \begin{equation}
%     \label{eq:squareConstraints1}
%     m_1=m_3,~~ m_2=m_4,
% \end{equation}
% and to form right angles,
% %\vspace*{-.5cm}
% \begin{equation}
%   \label{eq:squareConstraints2}
%         m_1 m_2 = -1.
% \end{equation}
% The least squares line-fitting problem with \eqref{eq:squareConstraints1} is a QP and
% already allows edges on opposite sides of the diamond to contribute to finding the
% slopes. While the constraint \eqref{eq:squareConstraints2} links all the edges together, it makes the least
% squares problem non-convex. However, applying Taylor's theorem about ``current
% estimates'' of the slopes at step $t$, denoted ${m}^t_1$,  ${m}^t_2$, along with some
% simple algebra results in the linear (update) constraint \begin{equation}
%     \label{eq:LinearizedSlopeProduct}
%     \begin{bmatrix}m_2^t &m_1^t \end{bmatrix}\begin{bmatrix} m_1^{t+1} \medskip  \\ m_2^{t+1} \end{bmatrix}= -1 + m_1^t  m_2^t .
% \end{equation}
% Starting with the initial estimates of $m_1^0=1, m_2^0=-1$, in our experience, iterating the QP with linear constraints 
% % \resizebox{.45 \textwidth}{!}
% % {
% \begin{equation}
%     \label{eq:LinearizedConstraints}
%     A_{eq}=\left[\begin{array}{rrrr} 1 & 0 & -1 & 0\\ 0 & 1 & 0 & -1 \\ m_2^t &
%         m_1^t & 0 & 0 \end{array}  \right],~ b_{eq}= \left[\begin{array}{c} 0 \\ 0\\
% -1 + m_1^t  m_2^t  \end{array} \right]
% \end{equation}
% % }
% on the slopes, and no constraints on the offsets, converges in two or three steps. In
% principle, one should also impose conditions on the offsets $b_i$ so that the lengths
% of the sides are equal to the physical size of the target, but in our experience, it
% is not necessary to do this. 

% The intersections of the resulting lines define the target's vertices in the plane
% defined by its normal vector. It is then straightforward to lift them to vertices
% $\{X_i \}_{i=1}^{4}$ of the target in $\real^3$. The reader is referred to \cite{githubFile} for the corresponding transformation, $H_L^T$.


==> pre_tex/defines.tex <==
% \usepackage{graphicx}
\usepackage[dvipdfmx]{graphicx} 
\usepackage{bmpsize}

\usepackage{caption}
\captionsetup{size=footnotesize,
    %justification=centering, %% not needed
    skip=5pt, position = bottom}
\let\proof\relax 
\let\endproof\relax
\usepackage{amsthm}
\usepackage{algorithm, algorithmicx, algpseudocode}
\usepackage{mathrsfs}
\usepackage{times}
\usepackage{multicol}
\usepackage[caption=false,font=footnotesize]{subfig}
\usepackage{amsfonts}
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{textcomp}
\usepackage{balance}
%\usepackage[sort,numbers]{natbib}
\usepackage{multirow}
\usepackage{booktabs}
\usepackage{dblfloatfix} 

\usepackage{bbold}
\usepackage{makecell}
\usepackage{hhline} % double-line in a table
% \usepackage[]{hyperref}
\usepackage{hyperref}
\hypersetup{
  colorlinks=true,pdfpagemode=UseNone,citecolor=black,linkcolor=black,urlcolor=BrickRed
}

\usepackage{comment}
%\usepackage{url}
\usepackage{amsmath,amssymb,enumerate}
\let\proof\relax 
\let\endproof\relax
\usepackage{setspace}

\usepackage{xparse}
\usepackage{lipsum}
%\usepackage{subcaption}
\usepackage{soul} 
\usepackage{times}
%\usepackage{cite} % to group references
\usepackage{fixltx2e}
\usepackage[usenames,dvipsnames,svgnames,table, xcdraw]{xcolor}
% \usepackage[sort, numbers]{natbib}
\usepackage{balance}


\newtheorem{problem}{Problem}
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{remark}{Remark}
\newtheorem{fact}{Fact}
\newtheorem{definition}{Definition}
\newtheorem{example}{Example}
\newtheorem{assumption}{Assumption}



\graphicspath{
    {graphics/}
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% $\usepackage{stmaryrd}
% \usepackage{algorithm, algorithmicx, algpseudocode}
% \renewcommand{\algorithmiccomment}[1]{\hfill$\triangleright$~\textcolor{Gray}{#1}}
% \usepackage{xparse}
% \usepackage{soul} 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
% \newtheorem{remark}{Remark}

\def\realnumbers{\mathbb{R}}
\def\real{\mathbb{R}}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
% \DeclareMathOperator*{\minimize}{minimize}
% \newcommand\scalemath[2]{\scalebox{#1}{\mbox{\ensuremath{\displaystyle #2}}}}
% \renewcommand{\thefigure}{\arabic{figure}}


\newcommand{\hilight}[1]{\colorbox{yellow}{#1}} % to use: \hl{this is some highlighted text}
\newcommand{\red}[1]{{\textcolor{red}{#1}}}
\newcommand{\blue}[1]{{\textcolor{blue}{#1}}}
\newcommand{\rha}[1]{[{\textbf{\textcolor{orange}{Ross: #1}}}]}
\newcommand{\jwg}[1]{[{\textbf{\textcolor{red}{JWG: #1}}}]}
\newcommand{\mgj}[1]{[{\textbf{\textcolor{teal}{Maani: #1}}}]}
\newcommand{\jkh}[1]{[{\textbf{\textcolor{blue}{Bruce: #1}}}]}
\newcommand{\bh}[1]{[{\textbf{\textcolor{blue}{Bruce: #1}}}]}
\newcommand{\bht}[1]{[{\textbf{\textcolor{note}{Bruce: (TODO) #1}}}]}
\newcommand{\bhd}[1]{[{\textbf{\textcolor{blue}{Bruce: Done, please check#1}}}]}
\definecolor{note}{rgb}{0.3,0.7,0.25}
\definecolor{rephase}{rgb}{0.15,0.7,0.15}
\definecolor{bag}{rgb}{0.6,0.6,0.2}


\newcommand{\lc}{LiDAR-camera}
\newcommand{\lidar}{LiDAR~}
\newcommand{\lidars}{LiDARs~}
\newcommand{\lidart}{LiDARTag~}
\newcommand{\lidarts}{LiDARTags}
\newcommand{\atag}{AprilTag}
\newcommand{\atags}{AprilTags}
\newcommand{\pc}{\mathcal{PC}}
\newcommand{\GPcal}{\mathcal{GP}}
% \newcommand{\bigO}[1]{\Ocal(#1)} % Big O
% \newcommand{\EV}[1]{\mathbb{E}[#1]} % Expected Value
% \newcommand{\Var}[1]{\mathbb{V}[#1]} % Variance
% \newcommand{\Covariance}[1]{\mathbf{Cov}[#1]} % Covariance
\newcommand{\floor}[1]{\lfloor #1 \rfloor}

% \newcommand{\diag}{\mathop{\mathrm{diag}}}
% \newcommand{\m}{\mathop{\mathrm{m}}}
% \newcommand{\rad}{\mathop{\mathrm{rad}}}
% \newcommand{\dBm}{\mathop{\mathrm{dBm}}}
% \newcommand{\Hz}{\mathop{\mathrm{Hz}}}
% \newcommand{\GHz}{\mathop{\mathrm{GHz}}}
% \newcommand{\MHz}{\mathop{\mathrm{MHz}}}

% \newcommand{\Acal}{\mathcal{A}}
% \newcommand{\Bcal}{\mathcal{B}}
% \newcommand{\Ccal}{\mathcal{C}}
% \newcommand{\Dcal}{\mathcal{D}}
% \newcommand{\dcal}{\text{\calligra d }}
% \newcommand{\ccal}{\text{\calligra c }}
% \newcommand{\Fcal}{\mathcal{F}}

% \newcommand{\Hcal}{\mathcal{H}}
% \newcommand{\Ical}{\mathcal{I}}
% \newcommand{\Kcal}{\mathcal{K}}
% \newcommand{\Lcal}{\mathcal{L}}
% \newcommand{\Mcal}{\mathcal{M}}
\newcommand{\Ncal}{\mathcal{N}}
% \newcommand{\Ocal}{\mathcal{O}}
% \newcommand{\Scal}{\mathcal{S}}
% \newcommand{\Tcal}{\mathcal{T}}
% \newcommand{\Xcal}{\mathcal{X}}
% \newcommand{\Ycal}{\mathcal{Y}}
% \newcommand{\Zcal}{\mathcal{Z}}

% \newcommand{\Exp}{\mathrm{Exp}}
% \newcommand{\Log}{\mathrm{Log}}
% \newcommand{\Jr}{\mathrm{J_r}}
\newcommand{\transpose}{\mathsf{T}}
\newcommand{\SO}{\mathrm{SO}}
\newcommand{\SE}{\mathrm{SE}}


% \newcommand{\GL}{\mathrm{GL}}
\newcommand\inv[1]{#1\raisebox{1.15ex}{$\scriptscriptstyle-\!1$}}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}

% \newcommand{\vecToSkew}{\wedge}
% \newcommand{\skewToVec}{\hat}
% \DeclareDocumentCommand{\vectorToSkew}{ O{} }{\left(#1\right)_\times}

\DeclareDocumentCommand{\vector}{ O{} }{\mathrm{vec}(#1)}
\DeclareDocumentCommand{\zeros}{ O{} }{\textbf{0}_{#1}}
\DeclareDocumentCommand{\X}{ O{} O{} }{\textbf{X}_{#1}^{#2}}
% \DeclareDocumentCommand{\XE}{ O{} O{} }{\hat{\textbf{X}}_{#1}^{#2}}
\DeclareDocumentCommand{\A}{ O{} O{} }{\textbf{A}_{#1}^{#2}}
% \DeclareDocumentCommand{\H}{ O{} O{} }{\textbf{H}_{#1}^{#2}}
\DeclareDocumentCommand{\H}{ O{} O{} }{\textbf{H}_{#1}^{#2}}
\DeclareDocumentCommand{\pre}{ O{} O{} }{{}_{#1}^{#2}}
% \DeclareDocumentCommand{\L}{ O{} O{} }{\textbf{L}_{#1}^{#2}}
% \DeclareDocumentCommand{\M}{ O{} O{} }{\textbf{M}_{#1}^{#2}}
% \DeclareDocumentCommand{\m}{ O{} O{} }{\textbf{m}_{#1}^{#2}}
% \DeclareDocumentCommand{\S}{ O{} O{} }{\textbf{S}_{#1}^{#2}}
\DeclareDocumentCommand{\P}{ O{} O{} }{\textbf{P}_{#1}^{#2}}
% \DeclareDocumentCommand{\Q}{ O{} O{} }{\textbf{Q}_{#1}^{#2}}
% \DeclareDocumentCommand{\J}{ O{} O{} }{\textbf{J}_{#1}^{#2}}
\DeclareDocumentCommand{\R}{ O{} O{} }{\textbf{R}_{#1}^{#2}}
% \DeclareDocumentCommand{\RE}{ O{} O{} }{\hat{\textbf{R}}_{#1}^{#2}}
% \DeclareDocumentCommand{\Q}{ O{} O{} }{\textbf{Q}_{#1}^{#2}}
\DeclareDocumentCommand{\T}{ O{} O{} }{\textbf{T}_{#1}^{#2}}
% \DeclareDocumentCommand{\L}{ O{} O{} }{\textbf{L}_{#1}^{#2}}
% \DeclareDocumentCommand{\K}{ O{} O{} }{\textbf{K}_{#1}^{#2}}
\DeclareDocumentCommand{\V}{ O{} O{} }{\textbf{V}_{#1}^{#2}}
% \DeclareDocumentCommand{\N}{ O{} O{} }{\textbf{N}_{#1}^{#2}}
\DeclareDocumentCommand{\Y}{ O{} O{} }{\textbf{Y}_{#1}^{#2}}
% \DeclareDocumentCommand{\Z}{ O{} O{} }{\textbf{Z}_{#1}^{#2}}
% \DeclareDocumentCommand{\F}{ O{} O{} }{\textbf{F}_{#1}^{#2}}
% \DeclareDocumentCommand{\G}{ O{} O{} }{\textbf{G}_{#1}^{#2}}
% \DeclareDocumentCommand{\A}{ O{} O{} }{\textbf{A}_{#1}^{#2}}
% \DeclareDocumentCommand{\TH}{ O{} O{} }{\boldsymbol{\Theta}_{#1}^{#2}}
% \DeclareDocumentCommand{\w}{ O{} O{} }{\textbf{w}_{#1}^{#2}}
% \DeclareDocumentCommand{\x}{ O{} O{} }{\textbf{x}_{#1}^{#2}}
% \DeclareDocumentCommand{\y}{ O{} O{} }{\textbf{y}_{#1}^{#2}}
% \DeclareDocumentCommand{\e}{ O{} O{} }{\textbf{e}_{#1}^{#2}}
% \DeclareDocumentCommand{\c}{ O{} O{} }{\textbf{c}_{#1}^{#2}}
% \DeclareDocumentCommand{\C}{ O{} O{} }{\textbf{C}_{#1}^{#2}}
% \DeclareDocumentCommand{\CM}{ O{} O{} }{\tilde{\textbf{C}}_{#1}^{#2}}
% \DeclareDocumentCommand{\RM}{ O{} O{} }{\tilde{\textbf{R}}_{#1}^{#2}}
% \DeclareDocumentCommand{\I}{ O{} O{} }{\textbf{I}_{#1}^{#2}}
% \DeclareDocumentCommand{\O}{ O{} O{} }{\textbf{O}_{#1}^{#2}}
% \DeclareDocumentCommand{\r}{ O{} O{} }{\textbf{r}_{#1}^{#2}}
% \DeclareDocumentCommand{\t}{ O{} O{} }{\textbf{t}_{#1}^{#2}}
% \DeclareDocumentCommand{\k}{ O{} O{} }{\textbf{k}_{#1}^{#2}}
% \DeclareDocumentCommand{\u}{ O{} O{} }{\textbf{u}_{#1}^{#2}}
\DeclareDocumentCommand{\U}{ O{} O{} }{\textbf{U}_{#1}^{#2}}
% \DeclareDocumentCommand{\d}{ O{} O{} }{\textbf{d}_{#1}^{#2}}
% \DeclareDocumentCommand{\dE}{ O{} O{} }{\hat{\textbf{d}}_{#1}^{#2}}
% \DeclareDocumentCommand{\b}{ O{} O{} }{\textbf{b}_{#1}^{#2}}
% \DeclareDocumentCommand{\a}{ O{} O{} }{\textbf{a}_{#1}^{#2}}
% \DeclareDocumentCommand{\g}{ O{} O{} }{\textbf{g}_{#1}^{#2}}
% \DeclareDocumentCommand{\f}{ O{} O{} }{\textbf{f}_{#1}^{#2}}
% \DeclareDocumentCommand{\dM}{ O{} O{} }{\tilde{\textbf{d}}_{#1}^{#2}}
% \DeclareDocumentCommand{\params}{ O{} O{} }{\boldsymbol{\theta}_{#1}^{#2}}
% \DeclareDocumentCommand{\paramsE}{ O{} O{} }{\hat{\boldsymbol{\theta}}_{#1}^{#2}}
% \DeclareDocumentCommand{\paramError}{ O{} O{} }{\boldsymbol{\zeta}_{#1}^{#2}}
% \DeclareDocumentCommand{\gyroscopeBias}{ O{} }{\textbf{b}_{#1}^{g}}
% \DeclareDocumentCommand{\gyroscopeBiasE}{ O{} }{\hat{\textbf{b}}_{#1}^{g}}
% \DeclareDocumentCommand{\accelerometerBias}{ O{} }{\textbf{b}_{#1}^{a}}
% \DeclareDocumentCommand{\accelerometerBiasE}{ O{} }{\hat{\textbf{b}}_{#1}^{a}}
% \DeclareDocumentCommand{\position}{ O{} O{} }{{}_\text{#2}\textbf{p}_{\text{#1}}}
% \DeclareDocumentCommand{\positionDot}{ O{} O{} }{{}_\text{#2}\dot{\textbf{p}}_{\text{#1}}}
% \DeclareDocumentCommand{\linearVelocity}{ O{} O{} }{{}_\text{#2}\textbf{v}_{\text{#1}}}
% \DeclareDocumentCommand{\linearVelocityM}{ O{} O{} }{{}_\text{#2}\tilde{\textbf{v}}_{\text{#1}}}
% \DeclareDocumentCommand{\orientation}{ O{} }{\textbf{R}_{\text{#1}}}
% \DeclareDocumentCommand{\orientationDot}{ O{} }{\dot{\textbf{R}}_{\text{#1}}}
% \DeclareDocumentCommand{\homogeneous}{ O{} O{} }{{}_\text{#2}\boldsymbol{\H}_{\text{#1}}}
% \DeclareDocumentCommand{\homogeneousDot}{ O{} }{\dot{\textbf{H}}_{\text{#1}}}
% \DeclareDocumentCommand{\Jacobian}{ O{} O{} }{{}_\text{#2}\boldsymbol{\J}_{\text{#1}}}
% \DeclareDocumentCommand{\inputs}{ O{} O{} }{{}_\text{#2}\boldsymbol{\u}_{\text{#1}}}
% \DeclareDocumentCommand{\inputsM}{ O{} O{} }{{}_\text{#2}\tilde{\boldsymbol{\u}}_{\text{#1}}}
% \DeclareDocumentCommand{\angularVelocity}{ O{} O{} }{{}_\text{#2}\boldsymbol{\omega}_{\text{#1}}}
% \DeclareDocumentCommand{\angularVelocityM}{ O{} O{} }{{}_\text{#2}\tilde{\boldsymbol{\omega}}_{\text{#1}}}
% \DeclareDocumentCommand{\acceleration}{ O{} O{} }{{}_\text{#2}\textbf{a}_{\text{#1}}}
% \DeclareDocumentCommand{\accelerationM}{ O{} O{} }{{}_\text{#2}\tilde{\textbf{a}}_{\text{#1}}}
% \DeclareDocumentCommand{\p}{ O{} O{} }{\textbf{p}_{#1}^{#2}}
% \DeclareDocumentCommand{\pE}{ O{} O{} }{\hat{\textbf{p}}_{#1}^{#2}}
% \DeclareDocumentCommand{\pM}{ O{} O{} }{\tilde{\textbf{p}}_{#1}^{#2}}
% \DeclareDocumentCommand{\v}{ O{} O{} }{\textbf{v}_{#1}^{#2}}
% \DeclareDocumentCommand{\vE}{ O{} O{} }{\hat{\textbf{v}}_{#1}^{#2}}
% \DeclareDocumentCommand{\w}{ O{} O{} }{\boldsymbol{\omega}_{#1}^{#2}}
% \DeclareDocumentCommand{\wM}{ O{} O{} }{\tilde{\boldsymbol{\omega}}_{#1}^{#2}}
% \DeclareDocumentCommand{\angleTheta}{ O{} O{} }{\boldsymbol{\theta}_{#1}^{#2}}
% \DeclareDocumentCommand{\anglePhi}{ O{} O{} }{\boldsymbol{\phi}_{#1}^{#2}}
% \DeclareDocumentCommand{\encoders}{ O{} O{} }{\boldsymbol{\alpha}_{#1}^{#2}}
% \DeclareDocumentCommand{\encodersM}{ O{} O{} }{\tilde{\boldsymbol{\alpha}}_{#1}^{#2}}
% \DeclareDocumentCommand{\offsets}{ O{} O{} }{\boldsymbol{\epsilon}_{#1}^{#2}}
% \DeclareDocumentCommand{\Cov}{ O{} O{} }{\boldsymbol{\Sigma}_{#1}^{#2}}
% \DeclareDocumentCommand{\Axis}{ O{} O{} }{\textnormal{Axis}_{#1}^{#2}}
% \DeclareDocumentCommand{\using}{ O{} O{} }{\stackrel{\mathmakebox[\widthof{=}]{\text{eq.} (#1)}}{#2} \enspace}
% \DeclareDocumentCommand{\Adjoint}{ O{} }{\mathrm{Ad}_{#1}}
% \DeclareDocumentCommand{\vectorToAlgebra}{ O{} }{\mathscr{L}_\mathfrak{g}\left(#1\right)}
% \DeclareDocumentCommand{\groupError}{ O{} O{} }{\boldsymbol{\eta}_{#1}^{#2}}
% % \DeclareDocumentCommand{\tangentError}{ O{} O{} }{\boldsymbol{\xi}_{#1}^{#2}}
% \DeclareDocumentCommand{\twist}{ O{} O{} }{\boldsymbol{\xi}_{#1}^{#2}}
% \DeclareDocumentCommand{\twistM}{ O{} O{} }{\tilde{\boldsymbol{\xi}}_{#1}^{#2}}

% \DeclareDocumentCommand{\JFK}{ O{} }{\textbf{J}^{\hspace{-0.75mm}\FK}_{#1}}

% \DeclareDocumentCommand{\JFKswitch}{ O{} }{\textbf{J}^{\hspace{-0.75mm}\FKswitch}_{#1}}

\newcommand{\squeezeup}{\vspace{-4mm}}

% \makeatletter
% \newcommand{\mathleft}{\@fleqntrue\@mathmargin0pt}
% \newcommand{\mathcenter}{\@fleqnfalse}
% \makeatother


==> table-sim.tex <==
\begin{table*}[]
    \centering
\caption{}
\label{tab:SimNoiseFreeResults}
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
\multicolumn{8}{|c|}{\textbf{Face-on LiDAR}} \\ \hline
Distance & \begin{tabular}[c]{@{}c@{}}Quantization\\ Error\end{tabular} & No. Points & RMSE & RMSE{[}\%{]} & \begin{tabular}[c]{@{}c@{}}Translation\\ Error {[}m{]}\end{tabular} & \begin{tabular}[c]{@{}c@{}}Translation\\ Error {[}\%{]}\end{tabular} & \begin{tabular}[c]{@{}c@{}}Rotation\\ Error {[}deg{]}\end{tabular} \\ \hline
2 & 0.013995 & 2530 & 0.0093564 & 0.46674 & 0.0022678 & 0.11313 & 0.67019 \\ \hline
4 & 0.027941 & 1015 & 0.032971 & 0.8238 & 0.0048189 & 0.1204 & 2.4083 \\ \hline
6.0015 & 0.041899 & 548 & 0.023524 & 0.39196 & 0.0070957 & 0.11823 & 1.6559 \\ \hline
8.0012 & 0.055859 & 338 & 0.020583 & 0.25725 & 0.011582 & 0.14476 & 1.2563 \\ \hline
10.001 & 0.06982 & 228 & 0.013059 & 0.13058 & 0.0085365 & 0.085357 & 0.72964 \\ \hline
12.001 & 0.083781 & 165 & 0.049253 & 0.41041 & 0.024402 & 0.20334 & 3.1591 \\ \hline
14.001 & 0.097743 & 123 & 0.027044 & 0.19316 & 0.026631 & 0.19022 & 0.3473 \\ \hline
16.001 & 0.11171 & 96 & 0.034348 & 0.21466 & 0.033687 & 0.21053 & 0.4951 \\ \hline
18.001 & 0.12567 & 75 & 0.055494 & 0.30829 & 0.029262 & 0.16256 & 3.4818 \\ \hline
20 & 0.13963 & 61 & 0.038591 & 0.19295 & 0.033101 & 0.1655 & 1.4647 \\ \hline
22 & 0.15359 & 52 & 0.035096 & 0.15953 & 0.026134 & 0.11879 & 1.7296 \\ \hline
24 & 0.16755 & 44 & 0.033987 & 0.14161 & 0.024809 & 0.10337 & 1.7151 \\ \hline
26 & 0.18152 & 35 & 0.061431 & 0.23627 & 0.060578 & 0.23299 & 0.75341 \\ \hline
28 & 0.19548 & 31 & 0.051711 & 0.18468 & 0.05161 & 0.18432 & 0.23852 \\ \hline
30 & 0.20944 & 28 & 0.027806 & 0.092685 & 0.025274 & 0.084247 & 0.85583 \\ \hline
32 & 0.2234 & 26 & 0.055234 & 0.1726 & 0.053437 & 0.16699 & 1.0318 \\ \hline
34 & 0.23737 & 20 & 0.068433 & 0.20127 & 0.064893 & 0.19086 & 1.604 \\ \hline
36 & 0.25133 & 19 & 0.060576 & 0.16827 & 0.060433 & 0.16787 & 0.3074 \\ \hline
38 & 0.26529 & 15 & 0.17578 & 0.46259 & 0.084494 & 0.22235 & 11.399 \\ \hline
40 & 0.27925 & 15 & 0.1596 & 0.399 & 0.084398 & 0.21099 & 10.014 \\ \hline
\multicolumn{8}{|c|}{\textbf{Extreme Angle (20, 30, 30)}} \\ \hline
Distance & \begin{tabular}[c]{@{}c@{}}Quantization\\ Error\end{tabular} & No. Points & RMSE & RMSE{[}\%{]} & \begin{tabular}[c]{@{}c@{}}Translation\\ Error {[}m{]}\end{tabular} & \begin{tabular}[c]{@{}c@{}}Translation\\ Error {[}\%{]}\end{tabular} & \begin{tabular}[c]{@{}c@{}}Rotation\\ Error {[}deg{]}\end{tabular} \\ \hline
1.9366 & 0.01352 & 1734 & 0.013065 & 0.67464 & 0.0079154 & 0.40872 & 0.76745 \\ \hline
3.9348 & 0.02747 & 716 & 0.021165 & 0.53789 & 0.01708 & 0.43407 & 0.92286 \\ \hline
5.9342 & 0.041428 & 405 & 0.030579 & 0.5153 & 0.020665 & 0.34823 & 1.6642 \\ \hline
7.9339 & 0.055389 & 258 & 0.035718 & 0.45019 & 0.032373 & 0.40803 & 1.1143 \\ \hline
9.9337 & 0.06935 & 176 & 0.02766 & 0.27845 & 0.02751 & 0.27694 & 0.21241 \\ \hline
11.934 & 0.083312 & 123 & 0.036196 & 0.30331 & 0.035541 & 0.29782 & 0.50617 \\ \hline
13.934 & 0.097274 & 94 & 0.033884 & 0.24318 & 0.031959 & 0.22937 & 0.83119 \\ \hline
15.933 & 0.11124 & 70 & 0.049835 & 0.31277 & 0.046156 & 0.28968 & 1.3875 \\ \hline
17.933 & 0.1252 & 57 & 0.027262 & 0.15202 & 0.023004 & 0.12827 & 1.0801 \\ \hline
19.933 & 0.13916 & 45 & 0.12852 & 0.64473 & 0.030806 & 0.15455 & 9.2217 \\ \hline
21.933 & 0.15312 & 39 & 0.06431 & 0.29321 & 0.046731 & 0.21306 & 3.2624 \\ \hline
23.933 & 0.16709 & 32 & 0.12319 & 0.51471 & 0.016662 & 0.069618 & 9.0208 \\ \hline
25.933 & 0.18105 & 27 & 0.11847 & 0.45683 & 0.042766 & 0.16491 & 8.1638 \\ \hline
27.933 & 0.19501 & 23 & 0.15731 & 0.56316 & 0.013574 & 0.048595 & 11.591 \\ \hline
29.933 & 0.20897 & 21 & 0.11955 & 0.39939 & 0.090078 & 0.30093 & 5.8057 \\ \hline
31.933 & 0.22294 & 17 & 0.47045 & 1.4732 & 0.063707 & 0.1995 & 34.953 \\ \hline
33.933 & 0.2369 & 16 & 0.40669 & 1.1985 & 0.047937 & 0.14127 & 30.164 \\ \hline
35.933 & 0.25086 & 15 & 0.22657 & 0.63053 & 0.04225 & 0.11758 & 16.491 \\ \hline
37.933 & 0.26482 & 14 & 0.29976 & 0.79024 & 0.093693 & 0.24699 & 21.143 \\ \hline
39.933 & 0.27879 & 12 & 0.41025 & 1.0273 & 0.051874 & 0.1299 & 30.401 \\ \hline
\end{tabular}
\end{table*}

